Transfer RL across Observation Feature Spaces via Model-Based Regularization

In many reinforcement learning (RL) applications, the observation space is specified by human developers and restricted by physical realizations, and may thus be subject to dramatic changes over time (e.g. increased number of observable features). However, when the observation space changes, the previous policy will likely fail due to the mismatch of input features, and another policy must be trained from scratch, which is inefficient in terms of computation and sample complexity. Following theoretical insights, we propose a novel algorithm which extracts the latent-space dynamics in the source task, and transfers the dynamics model to the target task to use as a model-based regularizer. Our algorithm works for drastic changes of observation space (e.g. from vector-based observation to image-based observation), without any inter-task mapping or any prior knowledge of the target task. Empirical results show that our algorithm significantly improves the efficiency and stability of learning in the target task.

==> figs/subfig_cart.tex <==
\nextgroupplot[ 
title = {CartPole},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend,}
]
\path [fill=sourcecolor, fill opacity=0.2]
(axis cs:0,24.5336666666667)
--(axis cs:0,18.3666666666667)
--(axis cs:1,18.1398666666667)
--(axis cs:2,17.5650933333333)
--(axis cs:3,17.052008)
--(axis cs:4,16.4016064)
--(axis cs:5,16.0346184533333)
--(axis cs:6,15.4476947626667)
--(axis cs:7,14.9714224768)
--(axis cs:8,14.3236713147733)
--(axis cs:9,13.9189370518187)
--(axis cs:10,13.3550829747883)
--(axis cs:11,12.8839997131639)
--(axis cs:12,12.5004664371978)
--(axis cs:13,12.1537064830916)
--(axis cs:14,11.7895651864733)
--(axis cs:15,11.4249188158453)
--(axis cs:16,11.2065350526762)
--(axis cs:17,10.9518947088076)
--(axis cs:18,10.9347824337128)
--(axis cs:19,10.7611592803036)
--(axis cs:20,10.6355940909095)
--(axis cs:21,10.5484086060609)
--(axis cs:22,10.4520602181821)
--(axis cs:23,10.394981507879)
--(axis cs:24,10.4225852063032)
--(axis cs:25,10.6246681650426)
--(axis cs:26,10.6797345320341)
--(axis cs:27,10.7503876256272)
--(axis cs:28,10.6935767671685)
--(axis cs:29,10.6481947470681)
--(axis cs:30,10.4918891309878)
--(axis cs:31,10.4801779714569)
--(axis cs:32,10.5240757104989)
--(axis cs:33,10.5659272350658)
--(axis cs:34,10.5860084547193)
--(axis cs:35,10.5621400971088)
--(axis cs:36,10.396312077687)
--(axis cs:37,10.3637163288163)
--(axis cs:38,10.3043063963863)
--(axis cs:39,10.3899784504424)
--(axis cs:40,10.3717160936873)
--(axis cs:41,10.2107062082831)
--(axis cs:42,10.0685649666265)
--(axis cs:43,10.1348519733012)
--(axis cs:44,10.227881578641)
--(axis cs:45,10.1556385962461)
--(axis cs:46,10.1978442103302)
--(axis cs:47,10.3182753682642)
--(axis cs:48,10.5943536279447)
--(axis cs:49,10.8351495690224)
--(axis cs:50,11.4678529885513)
--(axis cs:51,11.2075490575077)
--(axis cs:52,11.6987059126728)
--(axis cs:53,14.3581647301382)
--(axis cs:54,17.1729984507773)
--(axis cs:55,19.5449320939551)
--(axis cs:56,21.5426123418308)
--(axis cs:57,23.5673565401313)
--(axis cs:58,25.2128185654384)
--(axis cs:59,26.109388185684)
--(axis cs:60,26.9200438818806)
--(axis cs:61,27.8358351055044)
--(axis cs:62,30.3741347510702)
--(axis cs:63,32.4059078008562)
--(axis cs:64,35.1245929073516)
--(axis cs:65,39.6654743258813)
--(axis cs:66,42.785379460705)
--(axis cs:67,44.6667702352307)
--(axis cs:68,45.8333495215179)
--(axis cs:69,48.846346283881)
--(axis cs:70,50.7627436937714)
--(axis cs:71,54.9543282883505)
--(axis cs:72,58.5367292973471)
--(axis cs:73,64.469316771211)
--(axis cs:74,67.7545200836355)
--(axis cs:75,73.9366160669084)
--(axis cs:76,76.8282928535267)
--(axis cs:77,81.2545676161547)
--(axis cs:78,82.9299874262571)
--(axis cs:79,80.7941899410057)
--(axis cs:80,78.1543519528045)
--(axis cs:81,83.8020148955769)
--(axis cs:82,87.1746785831282)
--(axis cs:83,90.7392761998359)
--(axis cs:84,92.2111542932021)
--(axis cs:85,96.8153234345616)
--(axis cs:86,97.712125414316)
--(axis cs:87,100.909033664786)
--(axis cs:88,99.7869602651622)
--(axis cs:89,100.18076821213)
--(axis cs:90,100.817614569704)
--(axis cs:91,101.75995832243)
--(axis cs:92,101.066766657944)
--(axis cs:93,104.652346659688)
--(axis cs:94,104.008477327751)
--(axis cs:95,102.053248528867)
--(axis cs:96,102.808998823094)
--(axis cs:97,102.993332391808)
--(axis cs:98,104.047332580113)
--(axis cs:99,103.737599397424)
--(axis cs:100,100.082879517939)
--(axis cs:101,104.599503614351)
--(axis cs:102,104.446269558148)
--(axis cs:103,105.896748979852)
--(axis cs:104,104.723132517215)
--(axis cs:105,110.344239347105)
--(axis cs:106,108.581324811017)
--(axis cs:107,108.978193182147)
--(axis cs:108,109.908554545718)
--(axis cs:109,108.280110303241)
--(axis cs:110,105.263888242593)
--(axis cs:111,109.971043927408)
--(axis cs:112,111.623435141926)
--(axis cs:113,114.298414780207)
--(axis cs:114,114.435598490833)
--(axis cs:115,113.988012125999)
--(axis cs:116,112.6636097008)
--(axis cs:117,110.097354427306)
--(axis cs:118,110.582550208512)
--(axis cs:119,110.659040166809)
--(axis cs:120,108.111165466781)
--(axis cs:121,110.321999040091)
--(axis cs:122,113.250132565406)
--(axis cs:123,116.326639385658)
--(axis cs:124,114.539111508527)
--(axis cs:125,111.223422540155)
--(axis cs:126,110.537738032124)
--(axis cs:127,113.836790425699)
--(axis cs:128,114.982699007226)
--(axis cs:129,109.744559205781)
--(axis cs:130,109.561914031291)
--(axis cs:131,107.968331225033)
--(axis cs:132,106.654464980026)
--(axis cs:133,110.863305317354)
--(axis cs:134,113.603644253884)
--(axis cs:135,113.602915403107)
--(axis cs:136,115.122065655819)
--(axis cs:137,113.037519191322)
--(axis cs:138,111.636615353057)
--(axis cs:139,109.249092282446)
--(axis cs:140,111.91120715929)
--(axis cs:141,115.074699060765)
--(axis cs:142,113.945759248612)
--(axis cs:143,112.53500739889)
--(axis cs:144,113.001205919112)
--(axis cs:145,111.520564735289)
--(axis cs:146,114.382651788232)
--(axis cs:147,114.678521430585)
--(axis cs:148,112.761950477802)
--(axis cs:149,111.142827048908)
--(axis cs:150,106.870928305793)
--(axis cs:151,105.976409311301)
--(axis cs:152,105.060860782374)
--(axis cs:153,107.114821959233)
--(axis cs:154,108.318124234053)
--(axis cs:155,108.459899387242)
--(axis cs:156,109.28098617646)
--(axis cs:157,111.437522274502)
--(axis cs:158,112.342817819601)
--(axis cs:159,110.000187589014)
--(axis cs:160,109.739483404545)
--(axis cs:161,111.617653390303)
--(axis cs:162,110.867389378909)
--(axis cs:163,108.093578169794)
--(axis cs:164,105.901329202502)
--(axis cs:165,109.940730028668)
--(axis cs:166,110.692450689601)
--(axis cs:167,112.780427218347)
--(axis cs:168,113.030408441345)
--(axis cs:169,112.150260086409)
--(axis cs:170,112.565608069127)
--(axis cs:171,110.572286455302)
--(axis cs:172,110.357229164241)
--(axis cs:173,111.75104999806)
--(axis cs:174,112.319573331781)
--(axis cs:175,113.728725332092)
--(axis cs:176,117.289180265673)
--(axis cs:177,114.964277545872)
--(axis cs:178,116.457955370031)
--(axis cs:179,115.545030962691)
--(axis cs:180,117.609224770153)
--(axis cs:181,118.573913149456)
--(axis cs:182,119.052063852898)
--(axis cs:183,117.961117748985)
--(axis cs:184,117.060494199188)
--(axis cs:185,117.02739535935)
--(axis cs:186,116.421782954147)
--(axis cs:187,112.863359696651)
--(axis cs:188,109.097087757321)
--(axis cs:189,108.070136872523)
--(axis cs:190,110.248842831352)
--(axis cs:191,112.678207598415)
--(axis cs:192,114.635632745399)
--(axis cs:193,119.240639529652)
--(axis cs:194,117.525244957055)
--(axis cs:195,117.078929298977)
--(axis cs:196,118.916143439182)
--(axis cs:197,113.284781418012)
--(axis cs:198,115.307491801076)
--(axis cs:199,110.018193440861)
--(axis cs:199,156.065428547299)
--(axis cs:199,156.065428547299)
--(axis cs:198,159.90570235079)
--(axis cs:197,158.046961271821)
--(axis cs:196,161.16453492311)
--(axis cs:195,159.963168653887)
--(axis cs:194,159.937044150692)
--(axis cs:193,161.420805188365)
--(axis cs:192,158.708673152123)
--(axis cs:191,157.842508106821)
--(axis cs:190,155.910968466859)
--(axis cs:189,154.877543916908)
--(axis cs:188,155.621096562801)
--(axis cs:187,156.942537370168)
--(axis cs:186,159.16092171271)
--(axis cs:185,161.242485474221)
--(axis cs:184,161.035940176109)
--(axis cs:183,159.333091886803)
--(axis cs:182,159.124698191837)
--(axis cs:181,159.430622739797)
--(axis cs:180,156.836695091413)
--(axis cs:179,157.404035530932)
--(axis cs:178,157.554544413665)
--(axis cs:177,157.342430517082)
--(axis cs:176,159.318954813019)
--(axis cs:175,156.606776849607)
--(axis cs:174,156.483221062009)
--(axis cs:173,156.519276327511)
--(axis cs:172,154.922678742722)
--(axis cs:171,153.777265095069)
--(axis cs:170,154.679081368837)
--(axis cs:169,153.889768377713)
--(axis cs:168,154.170127138807)
--(axis cs:167,154.135408923509)
--(axis cs:166,153.085177821053)
--(axis cs:165,152.711888942983)
--(axis cs:164,149.656527845396)
--(axis cs:163,151.845576473411)
--(axis cs:162,152.555053925097)
--(axis cs:161,153.625400739705)
--(axis cs:160,151.914584257965)
--(axis cs:159,151.567063655789)
--(axis cs:158,152.763996236403)
--(axis cs:157,152.687911962171)
--(axis cs:156,152.43480661938)
--(axis cs:155,150.617924940892)
--(axis cs:154,150.921906176115)
--(axis cs:153,148.434799386811)
--(axis cs:152,145.88441590018)
--(axis cs:151,147.802269875225)
--(axis cs:150,148.502254010698)
--(axis cs:149,151.694400846706)
--(axis cs:148,153.574834391715)
--(axis cs:147,154.714459656311)
--(axis cs:146,153.167991237055)
--(axis cs:145,150.926405712986)
--(axis cs:144,151.582590474566)
--(axis cs:143,151.21082142654)
--(axis cs:142,152.003110116509)
--(axis cs:141,153.961554312303)
--(axis cs:140,151.459859557045)
--(axis cs:139,150.024491112973)
--(axis cs:138,152.712863891216)
--(axis cs:137,153.33982986402)
--(axis cs:136,155.005287330025)
--(axis cs:135,152.889692495864)
--(axis cs:134,152.810532286497)
--(axis cs:133,150.010582024788)
--(axis cs:132,147.271310864319)
--(axis cs:131,148.397138580398)
--(axis cs:130,147.220589892165)
--(axis cs:129,147.874904031872)
--(axis cs:128,151.23338003984)
--(axis cs:127,151.141641716467)
--(axis cs:126,149.617468812251)
--(axis cs:125,151.10375268198)
--(axis cs:124,152.412440852475)
--(axis cs:123,153.013967732261)
--(axis cs:122,149.564959665326)
--(axis cs:121,145.797782914991)
--(axis cs:120,143.987811977072)
--(axis cs:119,146.159681638006)
--(axis cs:118,146.507768714174)
--(axis cs:117,145.226044226051)
--(axis cs:116,148.682138615897)
--(axis cs:115,151.018923269872)
--(axis cs:114,152.015320754006)
--(axis cs:113,151.244150942508)
--(axis cs:112,149.387522011468)
--(axis cs:111,147.749902514335)
--(axis cs:110,144.211794809586)
--(axis cs:109,147.763326845315)
--(axis cs:108,147.945075223311)
--(axis cs:107,148.156010695805)
--(axis cs:106,147.386513369757)
--(axis cs:105,148.023558378863)
--(axis cs:104,144.978781306912)
--(axis cs:103,145.873059966973)
--(axis cs:102,145.499574958716)
--(axis cs:101,144.998635365062)
--(axis cs:100,140.714294206327)
--(axis cs:99,144.640617757909)
--(axis cs:98,145.542272197386)
--(axis cs:97,145.185840246733)
--(axis cs:96,146.472966975083)
--(axis cs:95,144.705708718853)
--(axis cs:94,146.115385898567)
--(axis cs:93,147.927399039875)
--(axis cs:92,146.050832133177)
--(axis cs:91,146.595623499805)
--(axis cs:90,144.819279374756)
--(axis cs:89,143.547099218445)
--(axis cs:88,144.389540689723)
--(axis cs:87,146.402759195487)
--(axis cs:86,143.786698994358)
--(axis cs:85,144.466123742948)
--(axis cs:84,139.864821345351)
--(axis cs:83,139.064193348356)
--(axis cs:82,135.803658352112)
--(axis cs:81,132.678156273473)
--(axis cs:80,127.379945341841)
--(axis cs:79,131.224015010635)
--(axis cs:78,132.45368542996)
--(axis cs:77,131.956273454117)
--(axis cs:76,127.978508484313)
--(axis cs:75,125.414802272058)
--(axis cs:74,119.576336173406)
--(axis cs:73,116.459670216757)
--(axis cs:72,111.73992110428)
--(axis cs:71,106.799318047016)
--(axis cs:70,101.489730892104)
--(axis cs:69,100.928746948463)
--(axis cs:68,97.9268503522453)
--(axis cs:67,96.4075629403066)
--(axis cs:66,92.3835370087165)
--(axis cs:65,87.5348379275623)
--(axis cs:64,82.1101307427863)
--(axis cs:63,78.1287467618161)
--(axis cs:62,74.0271834522702)
--(axis cs:61,69.4919793153377)
--(axis cs:60,67.2223908108388)
--(axis cs:59,67.1275718468818)
--(axis cs:58,64.1087981419357)
--(axis cs:57,60.3443310107529)
--(axis cs:56,54.5719137634411)
--(axis cs:55,50.3854755376348)
--(axis cs:54,45.1292610887101)
--(axis cs:53,37.609909694221)
--(axis cs:52,26.9863037844429)
--(axis cs:51,24.1073797305536)
--(axis cs:50,25.6508079965254)
--(axis cs:49,21.17184332899)
--(axis cs:48,21.1730541612375)
--(axis cs:47,20.4991510348803)
--(axis cs:46,18.540355460267)
--(axis cs:45,19.0420276586671)
--(axis cs:44,18.4521179066672)
--(axis cs:43,18.7728140500007)
--(axis cs:42,18.8489342291675)
--(axis cs:41,20.3945011197927)
--(axis cs:40,22.8681263997409)
--(axis cs:39,21.0015746663428)
--(axis cs:38,19.0851349995951)
--(axis cs:37,18.4396687494939)
--(axis cs:36,17.7156692702007)
--(axis cs:35,15.3612532544175)
--(axis cs:34,14.2931499013552)
--(axis cs:33,14.3412707100274)
--(axis cs:32,14.2848383875342)
--(axis cs:31,13.9642146510845)
--(axis cs:30,14.0051016471889)
--(axis cs:29,13.4730437256528)
--(axis cs:28,13.457804657066)
--(axis cs:27,13.6555891546658)
--(axis cs:26,13.0360697766656)
--(axis cs:25,12.861587220832)
--(axis cs:24,12.7019006927067)
--(axis cs:23,12.6189591992167)
--(axis cs:22,12.8986156656875)
--(axis cs:21,13.0065195821094)
--(axis cs:20,13.1497328109701)
--(axis cs:19,13.3536660137127)
--(axis cs:18,13.7254158504741)
--(axis cs:17,13.506603146426)
--(axis cs:16,13.9749205996992)
--(axis cs:15,14.393650749624)
--(axis cs:14,15.1753967703633)
--(axis cs:13,15.7191626296208)
--(axis cs:12,16.0072866203593)
--(axis cs:11,16.6339416087825)
--(axis cs:10,17.3340103443115)
--(axis cs:9,18.3340129303893)
--(axis cs:8,19.0506828296533)
--(axis cs:7,20.1382702037333)
--(axis cs:6,20.680921088)
--(axis cs:5,21.7924846933333)
--(axis cs:4,22.0486058666667)
--(axis cs:3,23.177424)
--(axis cs:2,23.68828)
--(axis cs:1,23.9602666666667)
--(axis cs:0,24.5336666666667)
--cycle;

\path [fill=ourcolor, fill opacity=0.2]
(axis cs:0,24.0003333333333)
--(axis cs:0,16.1993333333333)
--(axis cs:1,16.1994)
--(axis cs:2,15.1060533333333)
--(axis cs:3,15.0181093333333)
--(axis cs:4,14.8211541333333)
--(axis cs:5,14.33685664)
--(axis cs:6,14.256085312)
--(axis cs:7,14.0981349162667)
--(axis cs:8,13.6984412663467)
--(axis cs:9,13.525419679744)
--(axis cs:10,12.8736024104619)
--(axis cs:11,12.8188819283695)
--(axis cs:12,12.5217722093623)
--(axis cs:13,11.9639511008231)
--(axis cs:14,12.0044942139918)
--(axis cs:15,11.4702620378601)
--(axis cs:16,11.4761429636214)
--(axis cs:17,11.3942477042305)
--(axis cs:18,11.0953981633844)
--(axis cs:19,11.1496518640408)
--(axis cs:20,10.9063881578993)
--(axis cs:21,10.8184438596528)
--(axis cs:22,10.6680884210556)
--(axis cs:23,10.5944707368445)
--(axis cs:24,10.4955765894756)
--(axis cs:25,10.2431279382471)
--(axis cs:26,10.4611690172644)
--(axis cs:27,10.6022685471448)
--(axis cs:28,10.4950815043825)
--(axis cs:29,10.7493318701727)
--(axis cs:30,11.0727988294715)
--(axis cs:31,11.3648390635772)
--(axis cs:32,11.2918712508617)
--(axis cs:33,11.1267636673561)
--(axis cs:34,10.9947442672182)
--(axis cs:35,10.8889954137745)
--(axis cs:36,11.0377963310196)
--(axis cs:37,10.9502370648157)
--(axis cs:38,11.0401896518526)
--(axis cs:39,11.0921517214821)
--(axis cs:40,11.2469880438523)
--(axis cs:41,11.2708571017485)
--(axis cs:42,11.1100190147321)
--(axis cs:43,11.0545485451191)
--(axis cs:44,11.1500388360952)
--(axis cs:45,11.4664310688762)
--(axis cs:46,11.6464781884343)
--(axis cs:47,11.7568492174141)
--(axis cs:48,12.0980127072646)
--(axis cs:49,12.8446768324784)
--(axis cs:50,13.4421414659827)
--(axis cs:51,12.8936465061195)
--(axis cs:52,12.4215838715623)
--(axis cs:53,12.2905337639165)
--(axis cs:54,12.4390270111332)
--(axis cs:55,13.6575549422399)
--(axis cs:56,13.7390439537919)
--(axis cs:57,13.2178351630335)
--(axis cs:58,13.0940681304268)
--(axis cs:59,12.9617878376748)
--(axis cs:60,14.2089636034732)
--(axis cs:61,13.2804375494452)
--(axis cs:62,12.6976833728895)
--(axis cs:63,12.5778800316449)
--(axis cs:64,14.2620373586493)
--(axis cs:65,16.4424298869194)
--(axis cs:66,17.3738772428689)
--(axis cs:67,19.7321017942951)
--(axis cs:68,20.3513481021027)
--(axis cs:69,19.5403451483489)
--(axis cs:70,18.8982761186791)
--(axis cs:71,18.9832875616099)
--(axis cs:72,18.7197633826213)
--(axis cs:73,18.722210706097)
--(axis cs:74,18.570901898211)
--(axis cs:75,19.1299881852354)
--(axis cs:76,19.9303905481883)
--(axis cs:77,21.809045771884)
--(axis cs:78,21.3671032841739)
--(axis cs:79,21.4999492940058)
--(axis cs:80,21.7866261018713)
--(axis cs:81,20.0492342148304)
--(axis cs:82,22.185054038531)
--(axis cs:83,25.3880432308248)
--(axis cs:84,29.4965012513265)
--(axis cs:85,33.1170010010612)
--(axis cs:86,34.8602008008489)
--(axis cs:87,38.0680939740125)
--(axis cs:88,41.1276085125433)
--(axis cs:89,40.9085534767013)
--(axis cs:90,42.3195761146944)
--(axis cs:91,43.9817275584222)
--(axis cs:92,46.0186487134044)
--(axis cs:93,51.1875189707235)
--(axis cs:94,54.0492818432455)
--(axis cs:95,56.7701588079297)
--(axis cs:96,58.9749937130104)
--(axis cs:97,60.4261949704084)
--(axis cs:98,59.96048930966)
--(axis cs:99,60.1937247810613)
--(axis cs:100,60.1481798248491)
--(axis cs:101,61.8679438598793)
--(axis cs:102,66.6076217545701)
--(axis cs:103,67.7726307369894)
--(axis cs:104,69.0913045895915)
--(axis cs:105,69.1260436716732)
--(axis cs:106,70.9801682706719)
--(axis cs:107,70.5638679498709)
--(axis cs:108,69.53102769323)
--(axis cs:109,71.764622154584)
--(axis cs:110,70.5908977236672)
--(axis cs:111,70.9451181789338)
--(axis cs:112,75.5354278764803)
--(axis cs:113,78.5540756345176)
--(axis cs:114,81.7283271742807)
--(axis cs:115,85.6953950727579)
--(axis cs:116,85.0488493915397)
--(axis cs:117,85.1986128465651)
--(axis cs:118,86.6310236105854)
--(axis cs:119,87.6231522218016)
--(axis cs:120,86.5293217774413)
--(axis cs:121,86.4897907552864)
--(axis cs:122,87.1044326042291)
--(axis cs:123,88.9634794167166)
--(axis cs:124,90.29705020004)
--(axis cs:125,88.2629734933653)
--(axis cs:126,90.0690454613589)
--(axis cs:127,92.5950363690871)
--(axis cs:128,90.2666290952697)
--(axis cs:129,86.8198366095491)
--(axis cs:130,89.1085359543059)
--(axis cs:131,87.6664287634448)
--(axis cs:132,88.7320096774225)
--(axis cs:133,89.504407741938)
--(axis cs:134,92.4362595268837)
--(axis cs:135,92.4688742881737)
--(axis cs:136,90.2350327638722)
--(axis cs:137,89.4000262110978)
--(axis cs:138,90.4662209688782)
--(axis cs:139,88.7249101084359)
--(axis cs:140,87.3579280867487)
--(axis cs:141,85.9248091360656)
--(axis cs:142,87.7921139755192)
--(axis cs:143,88.013557847082)
--(axis cs:144,88.0822462776656)
--(axis cs:145,90.3256636887991)
--(axis cs:146,89.871997617706)
--(axis cs:147,89.8374647608314)
--(axis cs:148,87.9687051419985)
--(axis cs:149,84.9478307802654)
--(axis cs:150,83.2714646242124)
--(axis cs:151,88.7233716993699)
--(axis cs:152,88.2448306928292)
--(axis cs:153,89.6803978875967)
--(axis cs:154,92.4223183100774)
--(axis cs:155,95.8111213147286)
--(axis cs:156,97.5324970517829)
--(axis cs:157,97.1251976414263)
--(axis cs:158,96.8864914464744)
--(axis cs:159,94.8491264905128)
--(axis cs:160,92.9591011924103)
--(axis cs:161,92.4136809539282)
--(axis cs:162,95.1108114298092)
--(axis cs:163,95.3284491438474)
--(axis cs:164,95.1009593150779)
--(axis cs:165,96.366634118729)
--(axis cs:166,98.0725739616499)
--(axis cs:167,94.4907258359866)
--(axis cs:168,92.6056473354559)
--(axis cs:169,90.1242512016981)
--(axis cs:170,89.2641342946918)
--(axis cs:171,89.1776407690868)
--(axis cs:172,88.5211126152694)
--(axis cs:173,89.2762900922155)
--(axis cs:174,87.9408987404391)
--(axis cs:175,88.5446523256846)
--(axis cs:176,86.846655193881)
--(axis cs:177,84.9303908217715)
--(axis cs:178,84.4429793240838)
--(axis cs:179,84.4071167926004)
--(axis cs:180,83.5108934340803)
--(axis cs:181,84.6953147472643)
--(axis cs:182,89.0355851311447)
--(axis cs:183,87.0081347715825)
--(axis cs:184,90.658507817266)
--(axis cs:185,92.8528729204794)
--(axis cs:186,92.2864983363836)
--(axis cs:187,93.8417986691068)
--(axis cs:188,98.3601056019521)
--(axis cs:189,97.3342844815617)
--(axis cs:190,95.6462275852494)
--(axis cs:191,93.0609154015328)
--(axis cs:192,91.1276656545596)
--(axis cs:193,93.161265856981)
--(axis cs:194,92.3679460189181)
--(axis cs:195,98.0674901484678)
--(axis cs:196,100.513192118774)
--(axis cs:197,102.737087028353)
--(axis cs:198,101.201802956016)
--(axis cs:199,103.134642364812)
--(axis cs:199,144.144148202483)
--(axis cs:199,144.144148202483)
--(axis cs:198,140.629518586438)
--(axis cs:197,142.911648233047)
--(axis cs:196,141.172560291309)
--(axis cs:195,138.714783697469)
--(axis cs:194,132.99981295517)
--(axis cs:193,133.924432860629)
--(axis cs:192,131.38812440912)
--(axis cs:191,134.1149055114)
--(axis cs:190,134.226298555916)
--(axis cs:189,135.332623194895)
--(axis cs:188,135.940695660286)
--(axis cs:187,131.133452908691)
--(axis cs:186,131.625066135863)
--(axis cs:185,130.838499336496)
--(axis cs:184,130.023124170619)
--(axis cs:183,126.253655213274)
--(axis cs:182,126.483402349926)
--(axis cs:181,123.053919604075)
--(axis cs:180,121.875399505093)
--(axis cs:179,122.3108327147)
--(axis cs:178,122.738207560041)
--(axis cs:177,122.506009450052)
--(axis cs:176,126.099095145898)
--(axis cs:175,127.681452265706)
--(axis cs:174,127.251065332132)
--(axis cs:173,129.463831665165)
--(axis cs:172,126.837289581457)
--(axis cs:171,129.078361976821)
--(axis cs:170,128.53803580436)
--(axis cs:169,130.105711422116)
--(axis cs:168,131.957055944312)
--(axis cs:167,134.754236597057)
--(axis cs:166,139.292045746321)
--(axis cs:165,138.481640516234)
--(axis cs:164,139.417967311959)
--(axis cs:163,140.680709139949)
--(axis cs:162,141.898136424937)
--(axis cs:161,141.546670531171)
--(axis cs:160,142.741588163963)
--(axis cs:159,144.343235204954)
--(axis cs:158,144.227294006193)
--(axis cs:157,144.449784174408)
--(axis cs:156,145.135896884676)
--(axis cs:155,143.236454439179)
--(axis cs:154,141.086318048973)
--(axis cs:153,137.140314227883)
--(axis cs:152,136.066142784854)
--(axis cs:151,137.881761814401)
--(axis cs:150,132.585035601335)
--(axis cs:149,134.738711168335)
--(axis cs:148,139.429305627085)
--(axis cs:147,140.62771536719)
--(axis cs:146,140.792560875654)
--(axis cs:145,139.781784427901)
--(axis cs:144,138.051980534876)
--(axis cs:143,138.847725668595)
--(axis cs:142,137.201157085744)
--(axis cs:141,136.32619635718)
--(axis cs:140,136.864912113142)
--(axis cs:139,138.56347347476)
--(axis cs:138,140.687675176784)
--(axis cs:137,140.20809397098)
--(axis cs:136,141.418367463725)
--(axis cs:135,144.579459329656)
--(axis cs:134,146.59857416207)
--(axis cs:133,143.856467702587)
--(axis cs:132,144.127917961567)
--(axis cs:131,143.900730785293)
--(axis cs:130,144.799580148283)
--(axis cs:129,142.62339185202)
--(axis cs:128,144.904073148358)
--(axis cs:127,147.676674768781)
--(axis cs:126,144.527760127643)
--(axis cs:125,142.268033492887)
--(axis cs:124,144.459208532775)
--(axis cs:123,143.023593999302)
--(axis cs:122,140.494659165795)
--(axis cs:121,139.791573957243)
--(axis cs:120,139.055800779887)
--(axis cs:119,141.252834308193)
--(axis cs:118,140.665376218574)
--(axis cs:117,139.281386939884)
--(axis cs:116,139.343317008189)
--(axis cs:115,140.878729593569)
--(axis cs:114,138.188911991961)
--(axis cs:113,135.991889989952)
--(axis cs:112,133.889695820773)
--(axis cs:111,130.403369775966)
--(axis cs:110,129.059128886624)
--(axis cs:109,130.204994441614)
--(axis cs:108,126.663993052017)
--(axis cs:107,126.245324648355)
--(axis cs:106,125.971405810443)
--(axis cs:105,123.805590596387)
--(axis cs:104,123.773321578818)
--(axis cs:103,122.183068640189)
--(axis cs:102,120.307835800236)
--(axis cs:101,116.559211416961)
--(axis cs:100,113.423514271202)
--(axis cs:99,115.812559505669)
--(axis cs:98,114.873366048753)
--(axis cs:97,115.258290894274)
--(axis cs:96,112.722780284509)
--(axis cs:95,111.151392022303)
--(axis cs:94,107.738906694546)
--(axis cs:93,104.731050034849)
--(axis cs:92,99.3959792102279)
--(axis cs:91,94.8353073461183)
--(axis cs:90,91.6504675159811)
--(axis cs:89,90.3625843949764)
--(axis cs:88,89.5278971603872)
--(axis cs:87,86.0260381171507)
--(axis cs:86,82.3820476464383)
--(axis cs:85,82.1357262247146)
--(axis cs:84,77.9102411142266)
--(axis cs:83,68.8873847261165)
--(axis cs:82,60.8073975743123)
--(axis cs:81,53.8834136345571)
--(axis cs:80,55.544433709863)
--(axis cs:79,56.2712088039954)
--(axis cs:78,57.5052610049943)
--(axis cs:77,57.1474095895762)
--(axis cs:76,53.3919286536369)
--(axis cs:75,52.1313274837128)
--(axis cs:74,50.7808260213077)
--(axis cs:73,54.0916991933013)
--(axis cs:72,55.4793739916266)
--(axis cs:71,54.5643841561999)
--(axis cs:70,53.1288135285832)
--(axis cs:69,54.8523502440623)
--(axis cs:68,56.3902711384112)
--(axis cs:67,55.8201722563474)
--(axis cs:66,50.4747986537675)
--(axis cs:65,46.7844149838761)
--(axis cs:64,39.5022687298451)
--(axis cs:63,31.8512525789731)
--(axis cs:62,30.996482390383)
--(axis cs:61,34.8782696546454)
--(axis cs:60,39.7978370683067)
--(axis cs:59,34.2605463353834)
--(axis cs:58,36.6921829192293)
--(axis cs:57,35.8816453157033)
--(axis cs:56,36.3018066446291)
--(axis cs:55,34.9771749724531)
--(axis cs:54,30.7463020488997)
--(axis cs:53,30.3995442277912)
--(axis cs:52,31.8650969514057)
--(axis cs:51,31.3809545225905)
--(axis cs:50,34.7174431532381)
--(axis cs:49,29.8968039415476)
--(axis cs:48,26.5456715936012)
--(axis cs:47,24.5564228253349)
--(axis cs:46,22.5449451983352)
--(axis cs:45,22.2310148312524)
--(axis cs:44,19.3797685390655)
--(axis cs:43,19.8412106738319)
--(axis cs:42,19.1175133422898)
--(axis cs:41,20.646808344529)
--(axis cs:40,21.7167604306612)
--(axis cs:39,18.4453672049932)
--(axis cs:38,18.2317090062415)
--(axis cs:37,19.2144695911352)
--(axis cs:36,19.4096703222523)
--(axis cs:35,17.9703379028153)
--(axis cs:34,15.9030890451859)
--(axis cs:33,15.4698613064823)
--(axis cs:32,15.7952432997696)
--(axis cs:31,16.5439707913786)
--(axis cs:30,16.2382134892233)
--(axis cs:29,15.1144335281958)
--(axis cs:28,13.9595419102447)
--(axis cs:27,12.2825940544726)
--(axis cs:26,12.1699092347574)
--(axis cs:25,11.7790532101134)
--(axis cs:24,12.1570665126417)
--(axis cs:23,12.1963331408021)
--(axis cs:22,12.4870830926693)
--(axis cs:21,12.7505205325033)
--(axis cs:20,12.9130673322958)
--(axis cs:19,13.2663341653698)
--(axis cs:18,13.4995843733789)
--(axis cs:17,13.9993971333903)
--(axis cs:16,14.4074964167379)
--(axis cs:15,14.459287187589)
--(axis cs:14,15.3907756511529)
--(axis cs:13,15.3384695639411)
--(axis cs:12,15.9313369549264)
--(axis cs:11,16.6725045269914)
--(axis cs:10,17.1072139920725)
--(axis cs:9,18.025350823424)
--(axis cs:8,18.71493852928)
--(axis cs:7,19.1095898282667)
--(axis cs:6,19.753653952)
--(axis cs:5,20.5336507733333)
--(axis cs:4,20.8420634666667)
--(axis cs:3,21.3108293333333)
--(axis cs:2,21.75512)
--(axis cs:1,23.7604)
--(axis cs:0,24.0003333333333)
--cycle;

\path [fill=singlecolor, fill opacity=0.2]
(axis cs:0,28.2333333333333)
--(axis cs:0,18.3663333333333)
--(axis cs:1,18.1864)
--(axis cs:2,17.6824533333333)
--(axis cs:3,16.9659626666667)
--(axis cs:4,16.5326368)
--(axis cs:5,15.73270944)
--(axis cs:6,15.166167552)
--(axis cs:7,14.5328673749333)
--(axis cs:8,14.1061605666133)
--(axis cs:9,13.9449284532907)
--(axis cs:10,13.0959427626325)
--(axis cs:11,13.1100208767727)
--(axis cs:12,12.7546833680848)
--(axis cs:13,12.2903466944679)
--(axis cs:14,12.158944022241)
--(axis cs:15,11.7004218844594)
--(axis cs:16,11.6270041742342)
--(axis cs:17,11.4549366727207)
--(axis cs:18,10.9972826715099)
--(axis cs:19,11.2111594705412)
--(axis cs:20,10.935527576433)
--(axis cs:21,10.8617553944797)
--(axis cs:22,10.5694043155838)
--(axis cs:23,10.535523452467)
--(axis cs:24,10.321752095307)
--(axis cs:25,10.1374016762456)
--(axis cs:26,10.2032546743298)
--(axis cs:27,10.3092704061305)
--(axis cs:28,10.2806829915711)
--(axis cs:29,10.7776797265902)
--(axis cs:30,10.9954771146055)
--(axis cs:31,11.083048358351)
--(axis cs:32,10.9664386866808)
--(axis cs:33,10.8331509493447)
--(axis cs:34,10.5798540928091)
--(axis cs:35,10.4638832742473)
--(axis cs:36,10.3844399527311)
--(axis cs:37,10.4274852955182)
--(axis cs:38,10.6619215697479)
--(axis cs:39,11.076203922465)
--(axis cs:40,11.580763137972)
--(axis cs:41,12.2379438437109)
--(axis cs:42,11.6836217416354)
--(axis cs:43,11.3468973933083)
--(axis cs:44,11.1107845813133)
--(axis cs:45,11.0352943317173)
--(axis cs:46,11.0615687987072)
--(axis cs:47,10.6759217056324)
--(axis cs:48,10.8074040311726)
--(axis cs:49,10.8258565582714)
--(axis cs:50,10.9006852466171)
--(axis cs:51,10.9272148639604)
--(axis cs:52,10.7951052245016)
--(axis cs:53,10.6894175129346)
--(axis cs:54,10.5582006770144)
--(axis cs:55,10.2665605416115)
--(axis cs:56,9.85991509995587)
--(axis cs:57,9.9945320799647)
--(axis cs:58,9.87562566397176)
--(axis cs:59,9.74716719784407)
--(axis cs:60,9.83773375827526)
--(axis cs:61,9.68352033995354)
--(axis cs:62,9.58014960529616)
--(axis cs:63,9.2907863509036)
--(axis cs:64,9.46596241405621)
--(axis cs:65,9.6061032645783)
--(axis cs:66,10.1781492783293)
--(axis cs:67,10.2491194226634)
--(axis cs:68,10.3858955381308)
--(axis cs:69,9.96204976383794)
--(axis cs:70,9.83623981107035)
--(axis cs:71,9.90232518218962)
--(axis cs:72,9.92186014575169)
--(axis cs:73,10.1508214499347)
--(axis cs:74,10.0006571599477)
--(axis cs:75,9.8005257279582)
--(axis cs:76,9.70042058236656)
--(axis cs:77,9.84026979922658)
--(axis cs:78,9.83881583938127)
--(axis cs:79,9.69771933817168)
--(axis cs:80,9.87150880387068)
--(axis cs:81,9.71720704309654)
--(axis cs:82,9.40036563447723)
--(axis cs:83,9.41362584091512)
--(axis cs:84,9.34423400606543)
--(axis cs:85,9.19498720485234)
--(axis cs:86,9.05592309721521)
--(axis cs:87,9.8046718111055)
--(axis cs:88,10.0436707822177)
--(axis cs:89,9.90160329244085)
--(axis cs:90,9.88794930061935)
--(axis cs:91,9.94369277382881)
--(axis cs:92,9.78162088572972)
--(axis cs:93,9.67863004191711)
--(axis cs:94,10.016237366867)
--(axis cs:95,10.3129232268269)
--(axis cs:96,11.8500719147949)
--(axis cs:97,11.9797241985026)
--(axis cs:98,12.4501126921354)
--(axis cs:99,12.793356820375)
--(axis cs:100,12.7613521229667)
--(axis cs:101,12.8290816983733)
--(axis cs:102,12.6498653586987)
--(axis cs:103,12.5598256202923)
--(axis cs:104,12.7411271629005)
--(axis cs:105,12.5995017303204)
--(axis cs:106,12.399468050923)
--(axis cs:107,13.3059744407384)
--(axis cs:108,13.0712462192574)
--(axis cs:109,12.9501969754059)
--(axis cs:110,13.0198242469914)
--(axis cs:111,13.6022593975931)
--(axis cs:112,14.0684075180745)
--(axis cs:113,14.9405260144596)
--(axis cs:114,16.6256208115677)
--(axis cs:115,19.2192966492541)
--(axis cs:116,19.98110398607)
--(axis cs:117,22.377883188856)
--(axis cs:118,24.6285065510848)
--(axis cs:119,25.7024719075345)
--(axis cs:120,25.4553108593609)
--(axis cs:121,24.2907153541554)
--(axis cs:122,26.8719722833243)
--(axis cs:123,27.2155778266595)
--(axis cs:124,26.3041289279942)
--(axis cs:125,26.3895031423954)
--(axis cs:126,26.658069180583)
--(axis cs:127,27.6318553444664)
--(axis cs:128,28.7837509422398)
--(axis cs:129,30.7068674204585)
--(axis cs:130,31.1844939363668)
--(axis cs:131,29.4933284824268)
--(axis cs:132,28.4679294526081)
--(axis cs:133,28.9872102287531)
--(axis cs:134,28.3155015163358)
--(axis cs:135,30.6454678797353)
--(axis cs:136,32.2229743037883)
--(axis cs:137,33.5561127763639)
--(axis cs:138,33.3902902210912)
--(axis cs:139,33.5984321768729)
--(axis cs:140,34.7576790748317)
--(axis cs:141,34.9254765931987)
--(axis cs:142,33.4601146078923)
--(axis cs:143,33.9872916863138)
--(axis cs:144,32.5491000157177)
--(axis cs:145,33.0524800125742)
--(axis cs:146,31.8485173433927)
--(axis cs:147,32.5314805413808)
--(axis cs:148,33.318317766438)
--(axis cs:149,32.2207875464837)
--(axis cs:150,30.8765633705203)
--(axis cs:151,31.0985173630829)
--(axis cs:152,32.898680557133)
--(axis cs:153,33.0117444457064)
--(axis cs:154,34.9287955565651)
--(axis cs:155,36.3829697785854)
--(axis cs:156,38.493042489535)
--(axis cs:157,39.1075006582947)
--(axis cs:158,39.6324671933024)
--(axis cs:159,39.5321737546419)
--(axis cs:160,39.4789390037135)
--(axis cs:161,40.0021512029708)
--(axis cs:162,42.0205876290433)
--(axis cs:163,43.2819367699013)
--(axis cs:164,45.8453494159211)
--(axis cs:165,46.3561461994035)
--(axis cs:166,46.3511836261895)
--(axis cs:167,47.7408802342849)
--(axis cs:168,47.6975041874279)
--(axis cs:169,47.3244033499423)
--(axis cs:170,44.5457893466205)
--(axis cs:171,44.2614314772964)
--(axis cs:172,44.4345451818371)
--(axis cs:173,46.740769478803)
--(axis cs:174,48.6059489163758)
--(axis cs:175,51.3774924664339)
--(axis cs:176,50.2552606398138)
--(axis cs:177,51.7302751785177)
--(axis cs:178,55.2906868094808)
--(axis cs:179,55.592282780918)
--(axis cs:180,57.5326928914011)
--(axis cs:181,53.4126876464542)
--(axis cs:182,52.3089501171633)
--(axis cs:183,50.1392267603973)
--(axis cs:184,51.6633814083179)
--(axis cs:185,52.4566384599876)
--(axis cs:186,52.5315107679901)
--(axis cs:187,53.6380086143921)
--(axis cs:188,54.7230735581803)
--(axis cs:189,53.6315921798776)
--(axis cs:190,52.7051404105688)
--(axis cs:191,51.3771789951217)
--(axis cs:192,48.9550765294307)
--(axis cs:193,50.9838612235445)
--(axis cs:194,51.7258889788356)
--(axis cs:195,53.9537111830685)
--(axis cs:196,50.8961022797881)
--(axis cs:197,50.1961484904972)
--(axis cs:198,50.7695854590644)
--(axis cs:199,49.9622017005849)
--(axis cs:200,49.5622946938012)
--(axis cs:201,49.029635755041)
--(axis cs:202,49.2302419373661)
--(axis cs:203,49.2839268832262)
--(axis cs:204,49.306941506581)
--(axis cs:205,48.8313532052648)
--(axis cs:206,46.8450825642118)
--(axis cs:207,48.3822660513695)
--(axis cs:208,46.4121461744289)
--(axis cs:209,47.5735836062098)
--(axis cs:210,47.8720668849678)
--(axis cs:211,48.3907201746409)
--(axis cs:212,45.9317094730461)
--(axis cs:213,42.6987009117702)
--(axis cs:214,44.4984940627495)
--(axis cs:215,45.4777952501996)
--(axis cs:216,45.426569533493)
--(axis cs:217,44.8863889601277)
--(axis cs:218,42.7089778347689)
--(axis cs:219,42.2865822678151)
--(axis cs:220,40.9489991475854)
--(axis cs:221,39.5387993180683)
--(axis cs:222,40.1306394544547)
--(axis cs:223,40.9237782302304)
--(axis cs:224,42.2856225841843)
--(axis cs:225,41.5934980673475)
--(axis cs:226,44.3877317872113)
--(axis cs:227,43.3763187631024)
--(axis cs:228,43.2537216771486)
--(axis cs:229,44.5684440083855)
--(axis cs:230,44.9476885400417)
--(axis cs:231,44.2377508320334)
--(axis cs:232,42.7624006656267)
--(axis cs:233,45.0155205325014)
--(axis cs:234,45.2456164260011)
--(axis cs:235,44.7426264741342)
--(axis cs:236,46.833767845974)
--(axis cs:237,47.4531476101125)
--(axis cs:238,45.14231808809)
--(axis cs:239,45.3001878038054)
--(axis cs:240,45.1661502430443)
--(axis cs:241,46.5118535277688)
--(axis cs:242,46.7210161555483)
--(axis cs:243,48.7360129244387)
--(axis cs:244,50.8418103395509)
--(axis cs:245,54.3649149383074)
--(axis cs:246,54.6441319506459)
--(axis cs:247,58.2351722271834)
--(axis cs:248,58.9546711150801)
--(axis cs:249,57.0164702253974)
--(axis cs:250,56.1860428469846)
--(axis cs:251,53.0544342775877)
--(axis cs:252,52.2164807554035)
--(axis cs:253,50.6187179376561)
--(axis cs:254,55.1545743501249)
--(axis cs:255,55.2029928134332)
--(axis cs:256,55.2089942507466)
--(axis cs:257,54.7871287339306)
--(axis cs:258,55.6555029871445)
--(axis cs:259,54.4903357230489)
--(axis cs:260,53.4320685784391)
--(axis cs:261,52.1981881960846)
--(axis cs:262,50.9382172235344)
--(axis cs:263,49.3234404454942)
--(axis cs:264,49.9435523563953)
--(axis cs:265,50.0546418851163)
--(axis cs:266,48.036913508093)
--(axis cs:267,48.3424641398077)
--(axis cs:268,49.9339046451795)
--(axis cs:269,51.559657049477)
--(axis cs:270,51.2273256395816)
--(axis cs:271,48.1947938449986)
--(axis cs:272,45.9289017426655)
--(axis cs:273,44.6892547274658)
--(axis cs:274,43.3839371153059)
--(axis cs:275,48.0001496922448)
--(axis cs:276,46.1584530871291)
--(axis cs:277,44.3323624697033)
--(axis cs:278,44.7655566424293)
--(axis cs:279,42.7456453139435)
--(axis cs:280,45.4497829178214)
--(axis cs:281,42.9460263342571)
--(axis cs:282,44.3960210674057)
--(axis cs:283,43.0834835205912)
--(axis cs:284,43.7727201498063)
--(axis cs:285,45.7309761198451)
--(axis cs:286,44.984780895876)
--(axis cs:287,45.8078247167008)
--(axis cs:288,44.072793106694)
--(axis cs:289,44.7773011520219)
--(axis cs:290,43.8013075882842)
--(axis cs:291,44.4406460706273)
--(axis cs:292,45.6925168565019)
--(axis cs:293,46.6204134852015)
--(axis cs:294,46.5294641214945)
--(axis cs:295,46.929904630529)
--(axis cs:296,46.0099903710898)
--(axis cs:297,45.0475922968719)
--(axis cs:298,44.3179405041642)
--(axis cs:299,44.2675524033313)
--(axis cs:299,81.2352021845754)
--(axis cs:299,81.2352021845754)
--(axis cs:298,83.0766693973859)
--(axis cs:297,84.587503413399)
--(axis cs:296,83.7837959334155)
--(axis cs:295,86.0795782501027)
--(axis cs:294,86.607389479295)
--(axis cs:293,86.1919868491188)
--(axis cs:292,84.2554002280652)
--(axis cs:291,83.2272502850815)
--(axis cs:290,81.3002295230185)
--(axis cs:289,81.6992035704398)
--(axis cs:288,81.0567544630497)
--(axis cs:287,83.6026930788122)
--(axis cs:286,81.1612830151819)
--(axis cs:285,82.851520435644)
--(axis cs:284,78.613150544555)
--(axis cs:283,78.5909381806937)
--(axis cs:282,80.3874227258672)
--(axis cs:281,77.5811117406673)
--(axis cs:280,81.2427230091674)
--(axis cs:279,77.711070428126)
--(axis cs:278,81.2054213684908)
--(axis cs:277,81.5649433772802)
--(axis cs:276,83.1556792216002)
--(axis cs:275,84.6520990270003)
--(axis cs:274,81.256540450417)
--(axis cs:273,83.1117588963546)
--(axis cs:272,84.7456152871099)
--(axis cs:271,88.1901857755541)
--(axis cs:270,91.0705655527759)
--(axis cs:269,92.6374569409699)
--(axis cs:268,89.9797378428791)
--(axis cs:267,87.4243389702655)
--(axis cs:266,85.4617570461652)
--(axis cs:265,85.7682796410399)
--(axis cs:264,86.8922662179665)
--(axis cs:263,86.8394161057915)
--(axis cs:262,88.9987701322393)
--(axis cs:261,92.2984626652992)
--(axis cs:260,94.347828331624)
--(axis cs:259,95.0431187478633)
--(axis cs:258,94.9108984348291)
--(axis cs:257,93.6051230435364)
--(axis cs:256,93.5794038044205)
--(axis cs:255,93.6150047555256)
--(axis cs:254,94.2753392777403)
--(axis cs:253,89.1766740971754)
--(axis cs:252,89.8283426214692)
--(axis cs:251,90.2180116101699)
--(axis cs:250,95.1640145127123)
--(axis cs:249,97.0704348075571)
--(axis cs:248,101.521043509446)
--(axis cs:247,100.600387720141)
--(axis cs:246,97.2662346501766)
--(axis cs:245,96.8142933127208)
--(axis cs:244,91.5675333075677)
--(axis cs:243,89.2758333011262)
--(axis cs:242,86.9441249597411)
--(axis cs:241,87.5875728663431)
--(axis cs:240,85.0341327495955)
--(axis cs:239,84.8502492703277)
--(axis cs:238,86.903894921243)
--(axis cs:237,90.0537019848871)
--(axis cs:236,87.5585441477755)
--(axis cs:235,87.197846851386)
--(axis cs:234,88.4539752308992)
--(axis cs:233,85.648219038624)
--(axis cs:232,83.6181904649467)
--(axis cs:231,85.7295714145167)
--(axis cs:230,86.1616309348126)
--(axis cs:229,85.5427886685157)
--(axis cs:228,82.5281525023113)
--(axis cs:227,82.8084406278892)
--(axis cs:226,84.2517174515282)
--(axis cs:225,81.5719801477435)
--(axis cs:224,82.4226418513461)
--(axis cs:223,81.4445523141826)
--(axis cs:222,79.7214403927283)
--(axis cs:221,80.0093004909103)
--(axis cs:220,82.5613756136379)
--(axis cs:219,84.9590528503807)
--(axis cs:218,86.3486493963092)
--(axis cs:217,88.5523117453865)
--(axis cs:216,89.2467230150665)
--(axis cs:215,89.7060704354998)
--(axis cs:214,88.5070047110414)
--(axis cs:213,86.5251725554684)
--(axis cs:212,91.9714656943355)
--(axis cs:211,94.5890821179194)
--(axis cs:210,94.1190193140659)
--(axis cs:209,94.7644408092491)
--(axis cs:208,92.4881343448947)
--(axis cs:207,95.326334597785)
--(axis cs:206,93.457834913898)
--(axis cs:205,95.0635436423724)
--(axis cs:204,96.8877628862989)
--(axis cs:203,96.3012036078736)
--(axis cs:202,98.0086711765086)
--(axis cs:201,97.1940889706358)
--(axis cs:200,97.5923612132947)
--(axis cs:199,98.0227848499517)
--(axis cs:198,99.2521477291063)
--(axis cs:197,99.8066013280496)
--(axis cs:196,101.249834993395)
--(axis cs:195,104.811127075077)
--(axis cs:194,102.095325510513)
--(axis cs:193,101.343740221475)
--(axis cs:192,97.279425276844)
--(axis cs:191,98.3231982627217)
--(axis cs:190,99.9196644950687)
--(axis cs:189,102.257080618836)
--(axis cs:188,105.419934106878)
--(axis cs:187,104.699000966931)
--(axis cs:186,105.013167875331)
--(axis cs:185,104.89937651083)
--(axis cs:184,103.706803971871)
--(axis cs:183,100.898671631505)
--(axis cs:182,101.081589539381)
--(axis cs:181,100.530986924227)
--(axis cs:180,105.196233655283)
--(axis cs:179,102.745042069104)
--(axis cs:178,103.05605258638)
--(axis cs:177,97.6531490663084)
--(axis cs:176,95.1959363328855)
--(axis cs:175,95.7446704161069)
--(axis cs:174,95.1888380201336)
--(axis cs:173,93.252297525167)
--(axis cs:172,90.1648719064588)
--(axis cs:171,92.7803398830735)
--(axis cs:170,91.4833415205085)
--(axis cs:169,98.2104269006356)
--(axis cs:168,97.8544502924612)
--(axis cs:167,98.9001461989098)
--(axis cs:166,97.7463494153039)
--(axis cs:165,95.9132701024632)
--(axis cs:164,94.8071709614124)
--(axis cs:163,92.6831303684321)
--(axis cs:162,90.5869129605402)
--(axis cs:161,88.5085578673419)
--(axis cs:160,88.7580306675107)
--(axis cs:159,87.5613716677217)
--(axis cs:158,87.9082979179854)
--(axis cs:157,88.5847057308151)
--(axis cs:156,86.7637988301855)
--(axis cs:155,83.4295818710652)
--(axis cs:154,80.7191440054982)
--(axis cs:153,77.3560133402061)
--(axis cs:152,76.902100008591)
--(axis cs:151,72.9913750107387)
--(axis cs:150,72.3558854300901)
--(axis cs:149,75.4615234542792)
--(axis cs:148,78.1159876511824)
--(axis cs:147,78.9113178973113)
--(axis cs:146,77.6637307049725)
--(axis cs:145,79.2864133812156)
--(axis cs:144,77.9990167265196)
--(axis cs:143,82.8063542414828)
--(axis cs:142,83.0495261351868)
--(axis cs:141,87.0864910023168)
--(axis cs:140,87.1306970862294)
--(axis cs:139,85.2962046911201)
--(axis cs:138,84.1009225305668)
--(axis cs:137,86.9749864965418)
--(axis cs:136,84.0566497873439)
--(axis cs:135,81.5694789008465)
--(axis cs:134,80.5027652927249)
--(axis cs:133,81.3422066159061)
--(axis cs:132,80.7759249365493)
--(axis cs:131,82.5944061706866)
--(axis cs:130,86.0092577133582)
--(axis cs:129,84.9361554750311)
--(axis cs:128,80.9607776771222)
--(axis cs:127,80.1165554297361)
--(axis cs:126,77.2448609538368)
--(axis cs:125,78.2060761922961)
--(axis cs:124,80.9735119070368)
--(axis cs:123,83.2325565504626)
--(axis cs:122,81.8405290214116)
--(axis cs:121,77.9164946100978)
--(axis cs:120,80.9870349292889)
--(axis cs:119,80.5001269949445)
--(axis cs:118,77.6581587436806)
--(axis cs:117,73.9202817629341)
--(axis cs:116,70.458685537001)
--(axis cs:115,67.6798569212512)
--(axis cs:114,64.108071151564)
--(axis cs:113,60.4079222727884)
--(axis cs:112,57.3596528409855)
--(axis cs:111,55.2324827178985)
--(axis cs:110,56.4550200640398)
--(axis cs:109,55.1620250800497)
--(axis cs:108,55.9088646833955)
--(axis cs:107,55.1350808542444)
--(axis cs:106,51.6848510678055)
--(axis cs:105,51.8973138347569)
--(axis cs:104,52.4214756267794)
--(axis cs:103,49.7675945334743)
--(axis cs:102,48.0242431668429)
--(axis cs:101,48.4633872918869)
--(axis cs:100,45.412567448192)
--(axis cs:99,44.71420931024)
--(axis cs:98,44.8006783044666)
--(axis cs:97,44.8663478805833)
--(axis cs:96,44.6068515173958)
--(axis cs:95,41.9662310634114)
--(axis cs:94,39.0807888292643)
--(axis cs:93,36.4505693699137)
--(axis cs:92,35.1964617123921)
--(axis cs:91,35.5704938071568)
--(axis cs:90,33.838117258946)
--(axis cs:89,32.9642299070158)
--(axis cs:88,33.0469540504365)
--(axis cs:87,32.7484425630456)
--(axis cs:86,30.352053203807)
--(axis cs:85,30.9150665047587)
--(axis cs:84,31.385499797615)
--(axis cs:83,32.5902080803521)
--(axis cs:82,30.3375934337735)
--(axis cs:81,30.5969084588835)
--(axis cs:80,27.8961355736044)
--(axis cs:79,31.0447528003389)
--(axis cs:78,29.8391910004236)
--(axis cs:77,28.1148220838628)
--(axis cs:76,29.2681942714952)
--(axis cs:75,29.900992839369)
--(axis cs:74,26.8095743825445)
--(axis cs:73,25.7667179781807)
--(axis cs:72,22.7333974727259)
--(axis cs:71,22.0415801742407)
--(axis cs:70,20.0018085511342)
--(axis cs:69,20.018844022251)
--(axis cs:68,19.1984716944805)
--(axis cs:67,16.6064229514339)
--(axis cs:66,16.6579453559591)
--(axis cs:65,12.2553483616155)
--(axis cs:64,11.3271854520194)
--(axis cs:63,11.4423151483575)
--(axis cs:62,12.1278939354469)
--(axis cs:61,12.7015340859753)
--(axis cs:60,13.2685009408025)
--(axis cs:59,13.5188761760031)
--(axis cs:58,14.0734285533372)
--(axis cs:57,14.7667856916715)
--(axis cs:56,13.8083987812561)
--(axis cs:55,12.4187484765701)
--(axis cs:54,12.7566855957126)
--(axis cs:53,13.2956903279741)
--(axis cs:52,13.3945295766343)
--(axis cs:51,13.9764953041262)
--(axis cs:50,13.3372024634911)
--(axis cs:49,13.3797530793639)
--(axis cs:48,13.4330246825382)
--(axis cs:47,13.6829475198394)
--(axis cs:46,14.670351066466)
--(axis cs:45,14.5543554997491)
--(axis cs:44,14.8261110413531)
--(axis cs:43,15.1823888016914)
--(axis cs:42,15.8362360021142)
--(axis cs:41,17.2202950026428)
--(axis cs:40,16.9087020866368)
--(axis cs:39,15.7020442749626)
--(axis cs:38,14.1016386770366)
--(axis cs:37,13.6517150129625)
--(axis cs:36,13.6395604328697)
--(axis cs:35,13.7827838744205)
--(axis cs:34,13.9199798430256)
--(axis cs:33,14.1583081371154)
--(axis cs:32,14.9645518380609)
--(axis cs:31,15.8473564642428)
--(axis cs:30,16.6174455803035)
--(axis cs:29,15.846223642046)
--(axis cs:28,12.3237795525575)
--(axis cs:27,11.8295577740302)
--(axis cs:26,11.7536138842044)
--(axis cs:25,11.8502673552555)
--(axis cs:24,12.1045008607361)
--(axis cs:23,12.3472927425867)
--(axis cs:22,12.5756992615668)
--(axis cs:21,13.0529574102918)
--(axis cs:20,13.3828634295314)
--(axis cs:19,13.4283292869143)
--(axis cs:18,13.3687449419762)
--(axis cs:17,14.2609311774702)
--(axis cs:16,14.2178306385044)
--(axis cs:15,14.3972882981305)
--(axis cs:14,15.1632770393298)
--(axis cs:13,15.4790962991623)
--(axis cs:12,16.1653703739529)
--(axis cs:11,16.9817129674411)
--(axis cs:10,17.3103912093013)
--(axis cs:9,18.8629890116267)
--(axis cs:8,19.2870695978667)
--(axis cs:7,20.0754203306667)
--(axis cs:6,21.1942754133333)
--(axis cs:5,22.5761776)
--(axis cs:4,24.253472)
--(axis cs:3,25.4335066666667)
--(axis cs:2,26.8001333333333)
--(axis cs:1,27.3)
--(axis cs:0,28.2333333333333)
--cycle;

\path [fill=auxcolor, fill opacity=0.2]
(axis cs:0,27.3333333333333)
--(axis cs:0,17.199)
--(axis cs:1,17.2124)
--(axis cs:2,15.9831866666667)
--(axis cs:3,15.6931493333333)
--(axis cs:4,15.0677861333333)
--(axis cs:5,14.6208955733333)
--(axis cs:6,14.330049792)
--(axis cs:7,14.1373065002667)
--(axis cs:8,14.09651186688)
--(axis cs:9,13.837209493504)
--(axis cs:10,13.0697009281365)
--(axis cs:11,13.2624274091759)
--(axis cs:12,13.0632085940074)
--(axis cs:13,12.4705668752059)
--(axis cs:14,12.3497201668314)
--(axis cs:15,11.9331094667984)
--(axis cs:16,11.9198209067721)
--(axis cs:17,11.7425233920843)
--(axis cs:18,11.3540187136675)
--(axis cs:19,11.4098816376006)
--(axis cs:20,11.1345719767472)
--(axis cs:21,11.0876575813977)
--(axis cs:22,10.7634593984515)
--(axis cs:23,10.7040341854279)
--(axis cs:24,10.5831606816756)
--(axis cs:25,10.4465285453405)
--(axis cs:26,10.7035561696057)
--(axis cs:27,10.8894449356846)
--(axis cs:28,10.9315559485477)
--(axis cs:29,10.9985780921715)
--(axis cs:30,11.4655291404038)
--(axis cs:31,11.6990233123231)
--(axis cs:32,11.4258853165251)
--(axis cs:33,11.1740415865534)
--(axis cs:34,10.9390999359094)
--(axis cs:35,11.1046132820609)
--(axis cs:36,11.3369572923154)
--(axis cs:37,11.676232500519)
--(axis cs:38,12.0942526670818)
--(axis cs:39,12.8220688003321)
--(axis cs:40,12.8843217069324)
--(axis cs:41,12.8207240322126)
--(axis cs:42,12.2699125591034)
--(axis cs:43,11.6625967139494)
--(axis cs:44,11.2834107044928)
--(axis cs:45,11.3264618969276)
--(axis cs:46,11.8410361842087)
--(axis cs:47,11.5660956140337)
--(axis cs:48,11.9394764912269)
--(axis cs:49,12.2581811929815)
--(axis cs:50,12.2930782877186)
--(axis cs:51,12.1677959635082)
--(axis cs:52,11.6942367708065)
--(axis cs:53,11.4153894166452)
--(axis cs:54,11.6789115333162)
--(axis cs:55,11.6697958933196)
--(axis cs:56,11.435770047989)
--(axis cs:57,11.5685493717246)
--(axis cs:58,11.2477061640463)
--(axis cs:59,11.137964931237)
--(axis cs:60,11.350305278323)
--(axis cs:61,11.1602442226584)
--(axis cs:62,10.78152871146)
--(axis cs:63,10.3118896358347)
--(axis cs:64,10.5094450420011)
--(axis cs:65,10.8939560336009)
--(axis cs:66,11.3951648268807)
--(axis cs:67,11.6092651948379)
--(axis cs:68,11.6140121558703)
--(axis cs:69,11.3445430580296)
--(axis cs:70,11.3019011130903)
--(axis cs:71,11.2881875571389)
--(axis cs:72,11.0705500457111)
--(axis cs:73,11.0964400365689)
--(axis cs:74,11.3303520292551)
--(axis cs:75,11.7442816234041)
--(axis cs:76,11.6553586320566)
--(axis cs:77,11.597553572312)
--(axis cs:78,11.6176428578496)
--(axis cs:79,11.8807809529463)
--(axis cs:80,12.4444247623571)
--(axis cs:81,12.2288064765523)
--(axis cs:82,11.5096451812419)
--(axis cs:83,11.5143161449935)
--(axis cs:84,11.4576529159948)
--(axis cs:85,12.6190556661292)
--(axis cs:86,12.6151778662367)
--(axis cs:87,13.318608959656)
--(axis cs:88,13.2677538343915)
--(axis cs:89,14.0596697341798)
--(axis cs:90,15.3608691206772)
--(axis cs:91,14.6018952965418)
--(axis cs:92,14.2612495705667)
--(axis cs:93,14.3288663231201)
--(axis cs:94,14.808693058496)
--(axis cs:95,15.4196211134635)
--(axis cs:96,15.8354968907708)
--(axis cs:97,16.4546641792833)
--(axis cs:98,16.8233980100933)
--(axis cs:99,18.3979850747413)
--(axis cs:100,19.1773213931264)
--(axis cs:101,18.4485237811678)
--(axis cs:102,18.8052190249342)
--(axis cs:103,19.0507752199474)
--(axis cs:104,21.4872868426246)
--(axis cs:105,22.6020294740997)
--(axis cs:106,24.1399569126131)
--(axis cs:107,25.3044988634238)
--(axis cs:108,26.6486657574057)
--(axis cs:109,26.7322659392579)
--(axis cs:110,27.445679418073)
--(axis cs:111,25.683010201125)
--(axis cs:112,26.4395414942334)
--(axis cs:113,27.87056652872)
--(axis cs:114,28.675653222976)
--(axis cs:115,32.5468559117142)
--(axis cs:116,35.5834180627047)
--(axis cs:117,38.3932011168304)
--(axis cs:118,41.0869608934643)
--(axis cs:119,42.9626353814381)
--(axis cs:120,44.9966416384838)
--(axis cs:121,46.2569799774537)
--(axis cs:122,47.845383981963)
--(axis cs:123,50.222773852237)
--(axis cs:124,49.2888857484563)
--(axis cs:125,49.8238419320984)
--(axis cs:126,49.819006879012)
--(axis cs:127,51.4884721698763)
--(axis cs:128,51.010177735901)
--(axis cs:129,52.4007421887208)
--(axis cs:130,54.68692708431)
--(axis cs:131,55.5688083341147)
--(axis cs:132,55.6801133339584)
--(axis cs:133,56.4030240005001)
--(axis cs:134,57.1343525337334)
--(axis cs:135,60.6923486936534)
--(axis cs:136,63.1385456215894)
--(axis cs:137,64.0499698306048)
--(axis cs:138,67.1387758644839)
--(axis cs:139,68.4642206915871)
--(axis cs:140,72.1633765532697)
--(axis cs:141,69.3295679092824)
--(axis cs:142,71.4299209940926)
--(axis cs:143,72.9958701286074)
--(axis cs:144,73.1231627695526)
--(axis cs:145,71.8626635489754)
--(axis cs:146,70.0832641725137)
--(axis cs:147,71.2784780046776)
--(axis cs:148,74.1161157370754)
--(axis cs:149,73.5924259229937)
--(axis cs:150,77.0400074050616)
--(axis cs:151,72.7042725907159)
--(axis cs:152,72.7283514059061)
--(axis cs:153,72.8148144580582)
--(axis cs:154,73.3029182331132)
--(axis cs:155,72.5952679198239)
--(axis cs:156,76.5960810025258)
--(axis cs:157,74.403398135354)
--(axis cs:158,72.9947851749498)
--(axis cs:159,75.5690948066265)
--(axis cs:160,75.9469425119679)
--(axis cs:161,74.9903540095743)
--(axis cs:162,79.4522165409928)
--(axis cs:163,79.7151065661276)
--(axis cs:164,80.3915519195687)
--(axis cs:165,79.4321082023216)
--(axis cs:166,77.671553228524)
--(axis cs:167,78.2231092494858)
--(axis cs:168,79.4583540662553)
--(axis cs:169,78.1794832530043)
--(axis cs:170,78.5820532690701)
--(axis cs:171,79.0189759485894)
--(axis cs:172,76.9345807588715)
--(axis cs:173,78.3540646070972)
--(axis cs:174,79.4344516856778)
--(axis cs:175,78.5538280152089)
--(axis cs:176,76.6961290788338)
--(axis cs:177,75.636903263067)
--(axis cs:178,75.0021226104536)
--(axis cs:179,77.3540314216962)
--(axis cs:180,78.256225137357)
--(axis cs:181,78.3037801098856)
--(axis cs:182,78.2358240879085)
--(axis cs:183,79.3549259369934)
--(axis cs:184,81.8704074162614)
--(axis cs:185,80.8087259330091)
--(axis cs:186,82.2067140797406)
--(axis cs:187,81.2520379304592)
--(axis cs:188,78.513697011034)
--(axis cs:189,79.9901576088272)
--(axis cs:190,78.6454594203951)
--(axis cs:191,78.5284342029827)
--(axis cs:192,78.6092140290529)
--(axis cs:193,76.180637889909)
--(axis cs:194,77.8511769785938)
--(axis cs:195,74.6204082495417)
--(axis cs:196,72.4353932663)
--(axis cs:197,73.7080479463734)
--(axis cs:198,72.9195050237654)
--(axis cs:199,69.4821373523456)
--(axis cs:200,69.4923098818765)
--(axis cs:201,69.3182479055012)
--(axis cs:202,70.419998324401)
--(axis cs:203,70.3150653261874)
--(axis cs:204,70.1447855942833)
--(axis cs:205,75.2272951420933)
--(axis cs:206,71.2010361136746)
--(axis cs:207,69.147362224273)
--(axis cs:208,72.8372231127518)
--(axis cs:209,72.9897118235347)
--(axis cs:210,73.3983694588278)
--(axis cs:211,65.5449622337289)
--(axis cs:212,67.3290364536498)
--(axis cs:213,68.0293624962532)
--(axis cs:214,64.7300899970025)
--(axis cs:215,63.623271997602)
--(axis cs:216,61.170750931415)
--(axis cs:217,59.635800745132)
--(axis cs:218,60.1946405961056)
--(axis cs:219,58.2355124768845)
--(axis cs:220,57.9549433148409)
--(axis cs:221,57.390287985206)
--(axis cs:222,57.6586970548315)
--(axis cs:223,57.5735576438652)
--(axis cs:224,58.2383794484255)
--(axis cs:225,59.6106368920737)
--(axis cs:226,57.4541761803256)
--(axis cs:227,56.7558076109272)
--(axis cs:228,58.3905127554084)
--(axis cs:229,61.4852102043267)
--(axis cs:230,58.6747681634614)
--(axis cs:231,57.7327478641024)
--(axis cs:232,60.810798291282)
--(axis cs:233,61.7886386330256)
--(axis cs:234,60.8768442397538)
--(axis cs:235,60.9663420584697)
--(axis cs:236,59.1394736467758)
--(axis cs:237,59.4647789174206)
--(axis cs:238,60.2105564672698)
--(axis cs:239,57.7261785071492)
--(axis cs:240,58.186609472386)
--(axis cs:241,55.5622875779088)
--(axis cs:242,57.1895633956604)
--(axis cs:243,54.831317383195)
--(axis cs:244,55.5313872398893)
--(axis cs:245,56.7312431252448)
--(axis cs:246,60.1109278335292)
--(axis cs:247,62.05900893349)
--(axis cs:248,60.9592738134587)
--(axis cs:249,59.3004857174336)
--(axis cs:250,59.6064552406135)
--(axis cs:251,59.5316308591575)
--(axis cs:252,59.3869713539927)
--(axis cs:253,57.6095104165275)
--(axis cs:254,61.567208333222)
--(axis cs:255,60.9469666665776)
--(axis cs:256,60.3439733332621)
--(axis cs:257,60.7347786666097)
--(axis cs:258,61.6337562666211)
--(axis cs:259,63.3052050132968)
--(axis cs:260,62.5370306773041)
--(axis cs:261,59.2627578751766)
--(axis cs:262,57.5827396334746)
--(axis cs:263,58.6323917067797)
--(axis cs:264,58.8580466987571)
--(axis cs:265,56.378970692339)
--(axis cs:266,59.1939098872045)
--(axis cs:267,58.7077279097636)
--(axis cs:268,56.9589156611442)
--(axis cs:269,55.2267325289154)
--(axis cs:270,56.5743193564657)
--(axis cs:271,58.0789888185059)
--(axis cs:272,58.4088577214714)
--(axis cs:273,59.1594195105104)
--(axis cs:274,55.646202275075)
--(axis cs:275,58.3286951533933)
--(axis cs:276,56.1959561227147)
--(axis cs:277,53.4833648981717)
--(axis cs:278,53.2460252518707)
--(axis cs:279,54.1500868681632)
--(axis cs:280,56.0799361611973)
--(axis cs:281,55.2572155956245)
--(axis cs:282,55.1789724764996)
--(axis cs:283,52.680911314533)
--(axis cs:284,51.2777957182931)
--(axis cs:285,50.7610365746345)
--(axis cs:286,51.3410292597076)
--(axis cs:287,51.5589567410994)
--(axis cs:288,51.1603653928795)
--(axis cs:289,48.4416256476369)
--(axis cs:290,46.4132338514429)
--(axis cs:291,44.8637204144876)
--(axis cs:292,46.1769096649234)
--(axis cs:293,49.0014610652721)
--(axis cs:294,50.1468355188843)
--(axis cs:295,50.4972684151075)
--(axis cs:296,49.4110813987526)
--(axis cs:297,51.3943984523355)
--(axis cs:298,49.2354520952017)
--(axis cs:299,49.0202950094947)
--(axis cs:299,92.5419487137283)
--(axis cs:299,92.5419487137283)
--(axis cs:298,93.6836025588271)
--(axis cs:297,97.3758365318672)
--(axis cs:296,94.2442123315007)
--(axis cs:295,97.2796820810425)
--(axis cs:294,97.1079359346364)
--(axis cs:293,92.5012532516289)
--(axis cs:292,87.8423998978695)
--(axis cs:291,85.8349998723368)
--(axis cs:290,88.4100831737544)
--(axis cs:289,91.6538539671929)
--(axis cs:288,92.9641507923245)
--(axis cs:287,94.8951051570723)
--(axis cs:286,94.1838814463404)
--(axis cs:285,92.6297684745922)
--(axis cs:284,93.7704605932402)
--(axis cs:283,97.3709090748836)
--(axis cs:282,100.244886343604)
--(axis cs:281,99.7806079295056)
--(axis cs:280,101.367093245215)
--(axis cs:279,99.2169498898525)
--(axis cs:278,100.794937362316)
--(axis cs:277,98.5517550362279)
--(axis cs:276,101.472777128618)
--(axis cs:275,102.124221410773)
--(axis cs:274,99.9466100967993)
--(axis cs:273,103.799929287666)
--(axis cs:272,102.891494942915)
--(axis cs:271,103.179868678644)
--(axis cs:270,101.638669181639)
--(axis cs:269,100.360503143715)
--(axis cs:268,102.775378929644)
--(axis cs:267,105.425473662055)
--(axis cs:266,106.122092077569)
--(axis cs:265,105.352115096961)
--(axis cs:264,108.931560537868)
--(axis cs:263,105.172200672335)
--(axis cs:262,103.756584173751)
--(axis cs:261,106.787230217189)
--(axis cs:260,109.566954438153)
--(axis cs:259,111.007693047692)
--(axis cs:258,110.142282976281)
--(axis cs:257,108.759270387018)
--(axis cs:256,107.180587983773)
--(axis cs:255,110.792318313049)
--(axis cs:254,111.060481224645)
--(axis cs:253,105.066768197473)
--(axis cs:252,107.591043580175)
--(axis cs:251,108.421637808552)
--(axis cs:250,108.34329726069)
--(axis cs:249,106.512371575862)
--(axis cs:248,109.023464469828)
--(axis cs:247,109.945330587284)
--(axis cs:246,106.854079900772)
--(axis cs:245,102.075183209299)
--(axis cs:244,98.9184790116233)
--(axis cs:243,98.1370987645291)
--(axis cs:242,100.304123455661)
--(axis cs:241,98.2710709862434)
--(axis cs:240,102.146922066138)
--(axis cs:239,101.141319249339)
--(axis cs:238,106.56756572834)
--(axis cs:237,105.200373827092)
--(axis cs:236,104.031467283865)
--(axis cs:235,105.880917438164)
--(axis cs:234,105.175896797705)
--(axis cs:233,107.018620997131)
--(axis cs:232,106.347359579747)
--(axis cs:231,101.639199474684)
--(axis cs:230,101.948666010022)
--(axis cs:229,106.109999179194)
--(axis cs:228,102.57041564066)
--(axis cs:227,99.6786028841578)
--(axis cs:226,101.189420271864)
--(axis cs:225,103.559608673163)
--(axis cs:224,101.790094174787)
--(axis cs:223,101.078201051818)
--(axis cs:222,99.4297513147719)
--(axis cs:221,99.7033558101316)
--(axis cs:220,99.4038614293311)
--(axis cs:219,98.6285767866639)
--(axis cs:218,100.759887649997)
--(axis cs:217,100.549692895829)
--(axis cs:216,100.97594945312)
--(axis cs:215,104.044520149733)
--(axis cs:214,104.838400187166)
--(axis cs:213,108.130583567291)
--(axis cs:212,107.446562792447)
--(axis cs:211,106.541536823892)
--(axis cs:210,115.909754363199)
--(axis cs:209,115.419609620665)
--(axis cs:208,115.022428692498)
--(axis cs:207,111.169452532289)
--(axis cs:206,111.976648998695)
--(axis cs:205,116.778727915035)
--(axis cs:204,112.039409893794)
--(axis cs:203,114.414929033909)
--(axis cs:202,116.776911292386)
--(axis cs:201,113.870889115482)
--(axis cs:200,112.779111394353)
--(axis cs:199,113.671555909608)
--(axis cs:198,116.446778220343)
--(axis cs:197,118.423472775429)
--(axis cs:196,118.428257635953)
--(axis cs:195,122.608405378275)
--(axis cs:194,127.377006722843)
--(axis cs:193,126.237758403554)
--(axis cs:192,127.663281337776)
--(axis cs:191,126.744935005554)
--(axis cs:190,126.197168756942)
--(axis cs:189,126.537210946178)
--(axis cs:188,123.420347016055)
--(axis cs:187,126.583350436736)
--(axis cs:186,128.775854712586)
--(axis cs:185,128.2077350574)
--(axis cs:184,128.059585488416)
--(axis cs:183,127.215648527187)
--(axis cs:182,126.11747732565)
--(axis cs:181,124.49676332373)
--(axis cs:180,124.211704154662)
--(axis cs:179,125.288880193327)
--(axis cs:178,122.701850241659)
--(axis cs:177,123.576729468741)
--(axis cs:176,123.711995169259)
--(axis cs:175,124.988910628241)
--(axis cs:174,126.744471618634)
--(axis cs:173,125.194922856626)
--(axis cs:172,123.142736904116)
--(axis cs:171,125.161504463478)
--(axis cs:170,124.193297246014)
--(axis cs:169,123.399538224185)
--(axis cs:168,125.998672780231)
--(axis cs:167,125.814840975288)
--(axis cs:166,125.860134552444)
--(axis cs:165,129.305584857222)
--(axis cs:164,129.53906440486)
--(axis cs:163,128.265330506075)
--(axis cs:162,126.880913132594)
--(axis cs:161,123.334308082409)
--(axis cs:160,125.350051769678)
--(axis cs:159,124.536398045431)
--(axis cs:158,122.711914223456)
--(axis cs:157,123.881226112653)
--(axis cs:156,126.047615974149)
--(axis cs:155,123.208936634353)
--(axis cs:154,124.776754126275)
--(axis cs:153,124.511525991177)
--(axis cs:152,124.987240822305)
--(axis cs:151,125.550384361214)
--(axis cs:150,128.621063784851)
--(axis cs:149,124.96749639773)
--(axis cs:148,125.19253716383)
--(axis cs:147,123.520088121454)
--(axis cs:146,123.023526818484)
--(axis cs:145,126.277325189772)
--(axis cs:144,129.279823153881)
--(axis cs:143,129.516028942351)
--(axis cs:142,128.752786177939)
--(axis cs:141,127.182399389091)
--(axis cs:140,129.777832569697)
--(axis cs:139,125.797207378788)
--(axis cs:138,126.969759223485)
--(axis cs:137,125.245115696022)
--(axis cs:136,124.139477953361)
--(axis cs:135,122.131597441702)
--(axis cs:134,118.154246802127)
--(axis cs:133,117.267391835992)
--(axis cs:132,115.034156461657)
--(axis cs:131,112.442362243738)
--(axis cs:130,109.877786138006)
--(axis cs:129,109.055482672507)
--(axis cs:128,107.751770007301)
--(axis cs:127,109.597295842459)
--(axis cs:126,108.277703136407)
--(axis cs:125,107.788378920509)
--(axis cs:124,108.91605698397)
--(axis cs:123,109.235987896629)
--(axis cs:122,104.769651537452)
--(axis cs:121,104.826064421815)
--(axis cs:120,103.940580527269)
--(axis cs:119,99.9661423257534)
--(axis cs:118,98.9070945738584)
--(axis cs:117,94.7502015506563)
--(axis cs:116,89.2792519383204)
--(axis cs:115,84.4315649229005)
--(axis cs:114,78.8142061536256)
--(axis cs:113,77.4663410253653)
--(axis cs:112,75.29850961504)
--(axis cs:111,70.8723036854667)
--(axis cs:110,73.5642962735)
--(axis cs:109,72.9799536752083)
--(axis cs:108,75.2666087606771)
--(axis cs:107,72.498427617513)
--(axis cs:106,69.9725345218913)
--(axis cs:105,67.6062514856975)
--(axis cs:104,66.4143976904552)
--(axis cs:103,63.2423304464023)
--(axis cs:102,60.9915797246696)
--(axis cs:101,59.5723913225036)
--(axis cs:100,62.7320724864628)
--(axis cs:99,61.3142572747452)
--(axis cs:98,57.0987382600982)
--(axis cs:97,57.0556728251227)
--(axis cs:96,56.3275910314034)
--(axis cs:95,55.1674054559209)
--(axis cs:94,54.7650068199012)
--(axis cs:93,55.6287585248765)
--(axis cs:92,54.7098648227622)
--(axis cs:91,55.1701643617861)
--(axis cs:90,56.2706221188994)
--(axis cs:89,52.5292776486242)
--(axis cs:88,50.3695970607802)
--(axis cs:87,49.3117463259753)
--(axis cs:86,47.4772662408025)
--(axis cs:85,47.9959994676697)
--(axis cs:84,41.7189160012538)
--(axis cs:83,40.665061668234)
--(axis cs:82,38.8634104186258)
--(axis cs:81,38.0292630232822)
--(axis cs:80,36.8346621124361)
--(axis cs:79,33.7260776405452)
--(axis cs:78,31.0575137173481)
--(axis cs:77,28.9802254800185)
--(axis cs:76,27.2975318500231)
--(axis cs:75,28.6884148125289)
--(axis cs:74,26.4519351823278)
--(axis cs:73,25.5313356445764)
--(axis cs:72,25.7641695557205)
--(axis cs:71,25.013295277984)
--(axis cs:70,27.96661909748)
--(axis cs:69,24.54102387185)
--(axis cs:68,22.9087798398125)
--(axis cs:67,24.252558133099)
--(axis cs:66,24.631780999707)
--(axis cs:65,22.4645595829671)
--(axis cs:64,23.1056161453756)
--(axis cs:63,19.7403535150528)
--(axis cs:62,18.182691893816)
--(axis cs:61,19.3699482006034)
--(axis cs:60,20.8456852507542)
--(axis cs:59,21.0151065634428)
--(axis cs:58,21.8437165376368)
--(axis cs:57,22.2459790053793)
--(axis cs:56,21.4322237567242)
--(axis cs:55,20.0402796959052)
--(axis cs:54,20.9250162865482)
--(axis cs:53,17.6885203581852)
--(axis cs:52,17.2689004477316)
--(axis cs:51,18.8277922263311)
--(axis cs:50,19.8097402829139)
--(axis cs:49,19.095342020309)
--(axis cs:48,19.5857608587196)
--(axis cs:47,18.9238677400662)
--(axis cs:46,17.8130846750828)
--(axis cs:45,16.9162725105201)
--(axis cs:44,16.0452573048168)
--(axis cs:43,16.281321631021)
--(axis cs:42,17.5766520387763)
--(axis cs:41,18.987481715137)
--(axis cs:40,19.8509354772546)
--(axis cs:39,20.0468360132349)
--(axis cs:38,18.2084616832103)
--(axis cs:37,17.7351604373462)
--(axis cs:36,16.577283880016)
--(axis cs:35,16.0465215166867)
--(axis cs:34,15.2496518958584)
--(axis cs:33,15.4786482031563)
--(axis cs:32,15.7648102539454)
--(axis cs:31,16.8810128174317)
--(axis cs:30,17.1095160217897)
--(axis cs:29,17.1618116939038)
--(axis cs:28,15.0105146173797)
--(axis cs:27,15.2963099383913)
--(axis cs:26,13.4453874229891)
--(axis cs:25,12.5479842787364)
--(axis cs:24,12.8266470150872)
--(axis cs:23,12.8499754355256)
--(axis cs:22,13.1291359610737)
--(axis cs:21,13.8196699513421)
--(axis cs:20,14.1495874391776)
--(axis cs:19,14.6369842989721)
--(axis cs:18,14.6294803737151)
--(axis cs:17,14.2198504671438)
--(axis cs:16,14.6248130839298)
--(axis cs:15,14.7725996882456)
--(axis cs:14,15.240749610307)
--(axis cs:13,15.6842703462171)
--(axis cs:12,16.5386712661047)
--(axis cs:11,17.0565890826308)
--(axis cs:10,17.1206530199552)
--(axis cs:9,18.3424829416107)
--(axis cs:8,19.0279370103467)
--(axis cs:7,19.2849212629333)
--(axis cs:6,20.0060682453333)
--(axis cs:5,20.57416864)
--(axis cs:4,21.5257941333333)
--(axis cs:3,23.0072426666667)
--(axis cs:2,23.95072)
--(axis cs:1,26.1800666666667)
--(axis cs:0,27.3333333333333)
--cycle;

\path [fill=tunecolor, fill opacity=0.2]
(axis cs:0,29.7676666666667)
--(axis cs:0,19.1996666666667)
--(axis cs:1,18.6263333333333)
--(axis cs:2,18.6476666666667)
--(axis cs:3,18.1046666666667)
--(axis cs:4,18.1503333333333)
--(axis cs:5,17.5869333333333)
--(axis cs:6,18.36948)
--(axis cs:7,17.7822506666667)
--(axis cs:8,17.6656672)
--(axis cs:9,17.4792004266667)
--(axis cs:10,17.3431603413333)
--(axis cs:11,17.0877949397333)
--(axis cs:12,17.2368359517867)
--(axis cs:13,16.6560687614293)
--(axis cs:14,16.7648550091435)
--(axis cs:15,16.9052173406481)
--(axis cs:16,16.6708405391851)
--(axis cs:17,16.3497390980148)
--(axis cs:18,15.8930579450785)
--(axis cs:19,16.5476463560628)
--(axis cs:20,16.6511170848502)
--(axis cs:21,17.0336270012135)
--(axis cs:22,16.9799016009708)
--(axis cs:23,17.5171879474433)
--(axis cs:24,17.707083691288)
--(axis cs:25,17.6386669530304)
--(axis cs:26,18.5374668957576)
--(axis cs:27,18.5099735166061)
--(axis cs:28,18.4943121466182)
--(axis cs:29,18.1421163839612)
--(axis cs:30,18.4270264405023)
--(axis cs:31,17.8749544857352)
--(axis cs:32,19.1398302552548)
--(axis cs:33,18.8385308708705)
--(axis cs:34,20.1504913633631)
--(axis cs:35,20.0601930906905)
--(axis cs:36,20.4944878058857)
--(axis cs:37,20.8355235780419)
--(axis cs:38,22.0281521957669)
--(axis cs:39,21.7555884232802)
--(axis cs:40,21.8044040719575)
--(axis cs:41,22.536723257566)
--(axis cs:42,22.7157786060528)
--(axis cs:43,22.0592895515089)
--(axis cs:44,22.6207649745404)
--(axis cs:45,23.176478646299)
--(axis cs:46,22.8877829170392)
--(axis cs:47,22.5832263336314)
--(axis cs:48,22.6528477335718)
--(axis cs:49,23.1955448535241)
--(axis cs:50,22.8964358828193)
--(axis cs:51,22.7503487062554)
--(axis cs:52,24.099945631671)
--(axis cs:53,25.1466231720035)
--(axis cs:54,25.8635652042694)
--(axis cs:55,25.4573188300822)
--(axis cs:56,27.0647217307324)
--(axis cs:57,27.704977384586)
--(axis cs:58,27.4437819076688)
--(axis cs:59,27.3211588594683)
--(axis cs:60,28.3699937542413)
--(axis cs:61,29.1691283367264)
--(axis cs:62,30.1680360027145)
--(axis cs:63,32.4143621355049)
--(axis cs:64,35.5180230417373)
--(axis cs:65,35.7872851000565)
--(axis cs:66,35.1756280800452)
--(axis cs:67,37.9466357973695)
--(axis cs:68,38.2372419712289)
--(axis cs:69,38.1891269103165)
--(axis cs:70,39.0635681949198)
--(axis cs:71,36.9173212226025)
--(axis cs:72,36.0931236447487)
--(axis cs:73,36.0411655824656)
--(axis cs:74,37.6047324659725)
--(axis cs:75,37.4558526394447)
--(axis cs:76,40.2912821115557)
--(axis cs:77,40.6461590225779)
--(axis cs:78,42.8891272180623)
--(axis cs:79,42.1234351077832)
--(axis cs:80,40.9450147528932)
--(axis cs:81,39.2277451356479)
--(axis cs:82,39.208262775185)
--(axis cs:83,41.3332768868147)
--(axis cs:84,41.6456215094517)
--(axis cs:85,41.1228305408947)
--(axis cs:86,41.7179310993824)
--(axis cs:87,42.1076782128393)
--(axis cs:88,41.4125425702714)
--(axis cs:89,40.3963673895505)
--(axis cs:90,40.1837605783071)
--(axis cs:91,38.4802084626456)
--(axis cs:92,40.4494334367832)
--(axis cs:93,42.6253467494265)
--(axis cs:94,43.9666107328746)
--(axis cs:95,42.6788885862997)
--(axis cs:96,44.0363775357064)
--(axis cs:97,47.1355686952318)
--(axis cs:98,48.4147882895188)
--(axis cs:99,46.378430631615)
--(axis cs:100,46.7022111719587)
--(axis cs:101,44.0814356042336)
--(axis cs:102,45.6370818167202)
--(axis cs:103,47.3558654533762)
--(axis cs:104,47.5839590293676)
--(axis cs:105,46.4869005568274)
--(axis cs:106,47.9361204454619)
--(axis cs:107,49.1755630230362)
--(axis cs:108,48.492850418429)
--(axis cs:109,48.4539470014099)
--(axis cs:110,47.8830242677946)
--(axis cs:111,48.1526194142356)
--(axis cs:112,48.1753621980552)
--(axis cs:113,48.1397564251108)
--(axis cs:114,48.5374051400887)
--(axis cs:115,46.8157241120709)
--(axis cs:116,45.6654459563234)
--(axis cs:117,44.2720900983921)
--(axis cs:118,45.004205412047)
--(axis cs:119,45.4964309963042)
--(axis cs:120,44.9752781303767)
--(axis cs:121,43.705889170968)
--(axis cs:122,44.6965780034411)
--(axis cs:123,46.3894624027529)
--(axis cs:124,46.2513699222023)
--(axis cs:125,48.2872292710952)
--(axis cs:126,48.3363834168761)
--(axis cs:127,45.9087067335009)
--(axis cs:128,44.6392320534674)
--(axis cs:129,44.8845189761073)
--(axis cs:130,42.4809485142191)
--(axis cs:131,39.411425478042)
--(axis cs:132,42.3424737157669)
--(axis cs:133,44.8126456392802)
--(axis cs:134,43.9821831780908)
--(axis cs:135,47.112279875806)
--(axis cs:136,45.4430905673115)
--(axis cs:137,47.2342724538492)
--(axis cs:138,48.000284629746)
--(axis cs:139,45.7397610371301)
--(axis cs:140,46.5984088297041)
--(axis cs:141,46.9519937304299)
--(axis cs:142,47.4411283176773)
--(axis cs:143,46.9719026541418)
--(axis cs:144,45.4971221233135)
--(axis cs:145,45.7305643653174)
--(axis cs:146,45.3171181589206)
--(axis cs:147,47.2727611938032)
--(axis cs:148,44.7044089550425)
--(axis cs:149,41.5159938307007)
--(axis cs:150,41.2727283978939)
--(axis cs:151,37.8981160516484)
--(axis cs:152,37.5182928413188)
--(axis cs:153,39.9529009397217)
--(axis cs:154,41.0420540851107)
--(axis cs:155,43.2125766014219)
--(axis cs:156,44.5091279478042)
--(axis cs:157,42.9339023582433)
--(axis cs:158,43.4931218865947)
--(axis cs:159,42.1870975092757)
--(axis cs:160,40.6494113407539)
--(axis cs:161,39.0193957392698)
--(axis cs:162,37.9351832580825)
--(axis cs:163,38.4468132731327)
--(axis cs:164,39.0236506185061)
--(axis cs:165,40.0375871614716)
--(axis cs:166,42.0695363958439)
--(axis cs:167,42.4488291166751)
--(axis cs:168,39.9849299600068)
--(axis cs:169,39.1412773013388)
--(axis cs:170,38.919621841071)
--(axis cs:171,39.0422974728568)
--(axis cs:172,41.5465046449521)
--(axis cs:173,40.6172037159617)
--(axis cs:174,43.2667629727693)
--(axis cs:175,43.9660770448821)
--(axis cs:176,46.8389949692391)
--(axis cs:177,44.5303293087246)
--(axis cs:178,43.2973301136463)
--(axis cs:179,40.3841974242504)
--(axis cs:180,40.906624606067)
--(axis cs:181,41.4572996848536)
--(axis cs:182,43.0524397478829)
--(axis cs:183,42.660818464973)
--(axis cs:184,43.747321438645)
--(axis cs:185,44.4557238175827)
--(axis cs:186,45.2106457207328)
--(axis cs:187,44.7016499099196)
--(axis cs:188,45.1545199279357)
--(axis cs:189,44.4562159423485)
--(axis cs:190,43.9031727538788)
--(axis cs:191,42.1817382031031)
--(axis cs:192,42.6585238958158)
--(axis cs:193,41.7532857833193)
--(axis cs:194,45.4092952933221)
--(axis cs:195,45.6706362346577)
--(axis cs:196,45.2563756543928)
--(axis cs:197,46.9445005235143)
--(axis cs:198,45.8216670854781)
--(axis cs:199,42.4035336683825)
--(axis cs:200,42.0225602680393)
--(axis cs:201,40.7513148810981)
--(axis cs:202,42.5542519048785)
--(axis cs:203,44.0232015239028)
--(axis cs:204,44.5772945524556)
--(axis cs:205,43.5482356419645)
--(axis cs:206,43.4383218469049)
--(axis cs:207,43.6499241441906)
--(axis cs:208,43.9662726486858)
--(axis cs:209,43.2124181189486)
--(axis cs:210,43.5497344951589)
--(axis cs:211,42.4394542627938)
--(axis cs:212,44.2442967435684)
--(axis cs:213,44.515370728188)
--(axis cs:214,43.9182965825504)
--(axis cs:215,42.807903932707)
--(axis cs:216,40.6727898128323)
--(axis cs:217,41.2176318502658)
--(axis cs:218,42.6335054802127)
--(axis cs:219,42.9533377175035)
--(axis cs:220,42.6689368406694)
--(axis cs:221,40.0144161392022)
--(axis cs:222,39.4907995780284)
--(axis cs:223,38.6319063290894)
--(axis cs:224,38.8453917299382)
--(axis cs:225,39.1225133839506)
--(axis cs:226,39.0846773738271)
--(axis cs:227,39.7667418990617)
--(axis cs:228,40.246660185916)
--(axis cs:229,38.3572614820661)
--(axis cs:230,38.1443425189863)
--(axis cs:231,36.842074015189)
--(axis cs:232,34.8864592121512)
--(axis cs:233,33.3819007030543)
--(axis cs:234,33.0517872291101)
--(axis cs:235,31.8878964499548)
--(axis cs:236,30.9902504932971)
--(axis cs:237,31.8446003946377)
--(axis cs:238,33.0737469823768)
--(axis cs:239,35.4184642525681)
--(axis cs:240,35.3543714020545)
--(axis cs:241,34.8688971216436)
--(axis cs:242,33.7879843639816)
--(axis cs:243,33.6835874911852)
--(axis cs:244,34.3198033262815)
--(axis cs:245,32.6409093276919)
--(axis cs:246,31.7983941288202)
--(axis cs:247,31.8048486363895)
--(axis cs:248,32.4350789091116)
--(axis cs:249,33.7806631272893)
--(axis cs:250,34.5711305018314)
--(axis cs:251,33.7368377347985)
--(axis cs:252,34.2286701878388)
--(axis cs:253,33.1422028169377)
--(axis cs:254,32.1136955868835)
--(axis cs:255,33.4642231361735)
--(axis cs:256,33.7646451756054)
--(axis cs:257,36.2913161404843)
--(axis cs:258,34.8192529123875)
--(axis cs:259,32.7220689965766)
--(axis cs:260,31.6842551972613)
--(axis cs:261,31.6863374911424)
--(axis cs:262,32.2289366595806)
--(axis cs:263,32.5352826609978)
--(axis cs:264,33.3148261287982)
--(axis cs:265,36.5916609030386)
--(axis cs:266,37.5331287224309)
--(axis cs:267,37.1327029779447)
--(axis cs:268,36.6982957156891)
--(axis cs:269,36.7251032392179)
--(axis cs:270,36.2000159247077)
--(axis cs:271,36.0650127397661)
--(axis cs:272,37.5712768584796)
--(axis cs:273,38.1768214867837)
--(axis cs:274,35.5547238560936)
--(axis cs:275,33.4370457515415)
--(axis cs:276,32.8295032678999)
--(axis cs:277,32.2888692809866)
--(axis cs:278,31.4776287581226)
--(axis cs:279,32.5415696731648)
--(axis cs:280,31.6596557385318)
--(axis cs:281,30.6409912574921)
--(axis cs:282,30.9120596726604)
--(axis cs:283,31.5425810714616)
--(axis cs:284,35.1472648571693)
--(axis cs:285,35.3431452190688)
--(axis cs:286,35.2538495085884)
--(axis cs:287,36.228812940204)
--(axis cs:288,36.4944503521632)
--(axis cs:289,35.9953602817306)
--(axis cs:290,34.0028882253845)
--(axis cs:291,33.1420439136409)
--(axis cs:292,32.666768464246)
--(axis cs:293,31.9600814380635)
--(axis cs:294,31.4344651504508)
--(axis cs:295,31.060905453694)
--(axis cs:296,32.3214576962885)
--(axis cs:297,32.5902994903641)
--(axis cs:298,31.3321729256247)
--(axis cs:299,30.9920716738331)
--(axis cs:299,61.493479162958)
--(axis cs:299,61.493479162958)
--(axis cs:298,61.6747656203642)
--(axis cs:297,64.0096236921219)
--(axis cs:296,63.711946281819)
--(axis cs:295,61.9230995189405)
--(axis cs:294,62.9032077320089)
--(axis cs:293,64.7700929983445)
--(axis cs:292,67.3691995812639)
--(axis cs:291,66.6174161432466)
--(axis cs:290,68.2717701790583)
--(axis cs:289,72.7890460571561)
--(axis cs:288,72.4774742381119)
--(axis cs:287,70.9285094643065)
--(axis cs:286,71.3016368303831)
--(axis cs:285,71.6927960379789)
--(axis cs:284,70.1802450474736)
--(axis cs:283,63.421556309342)
--(axis cs:282,62.9016120533441)
--(axis cs:281,62.9932650666802)
--(axis cs:280,66.1830813333502)
--(axis cs:279,65.6775183333544)
--(axis cs:278,64.904647916693)
--(axis cs:277,66.3050598958663)
--(axis cs:276,67.1253248698329)
--(axis cs:275,70.0896560872911)
--(axis cs:274,75.2854034424472)
--(axis cs:273,77.6226709697257)
--(axis cs:272,77.4856720454904)
--(axis cs:271,73.9149233901964)
--(axis cs:270,75.1269042377455)
--(axis cs:269,74.3082136305152)
--(axis cs:268,74.533517038144)
--(axis cs:267,75.10839629768)
--(axis cs:266,76.6154120387666)
--(axis cs:265,75.6105150484583)
--(axis cs:264,69.2044771439062)
--(axis cs:263,66.7720130965494)
--(axis cs:262,65.8051830373534)
--(axis cs:261,63.538562130025)
--(axis cs:260,63.5897026625313)
--(axis cs:259,65.8193783281641)
--(axis cs:258,69.4490562435385)
--(axis cs:257,71.6695703044231)
--(axis cs:256,69.2282128805289)
--(axis cs:255,67.6350994339944)
--(axis cs:254,66.842874292493)
--(axis cs:253,71.1781761989496)
--(axis cs:252,70.9723035820203)
--(axis cs:251,69.3897961441921)
--(axis cs:250,68.3611618469068)
--(axis cs:249,67.8847023086334)
--(axis cs:248,66.6541278857918)
--(axis cs:247,65.0425765239064)
--(axis cs:246,65.961470654883)
--(axis cs:245,66.8093383186038)
--(axis cs:244,67.7525895649214)
--(axis cs:243,66.4738202894851)
--(axis cs:242,68.6835253618564)
--(axis cs:241,69.4932400356538)
--(axis cs:240,69.3653833779006)
--(axis cs:239,68.8553958890424)
--(axis cs:238,67.4854115279696)
--(axis cs:237,64.9056810766287)
--(axis cs:236,64.3231013457859)
--(axis cs:235,67.7952100155657)
--(axis cs:234,70.1021791861238)
--(axis cs:233,71.3776406493214)
--(axis cs:232,75.1384674783185)
--(axis cs:231,77.5805010145648)
--(axis cs:230,77.958876268206)
--(axis cs:229,74.9964286685908)
--(axis cs:228,78.0782025024052)
--(axis cs:227,79.0310031280064)
--(axis cs:226,79.0785039100081)
--(axis cs:225,78.6053798875101)
--(axis cs:224,76.9397248593876)
--(axis cs:223,77.4904894075678)
--(axis cs:222,78.4202784261265)
--(axis cs:221,80.5154313659914)
--(axis cs:220,84.0019558741559)
--(axis cs:219,84.5357781760283)
--(axis cs:218,82.7358060533687)
--(axis cs:217,78.0263409000442)
--(axis cs:216,76.9654261250552)
--(axis cs:215,83.1063659896523)
--(axis cs:214,85.7243741537321)
--(axis cs:213,86.3963843588318)
--(axis cs:212,85.4863137818731)
--(axis cs:211,82.749058894008)
--(axis cs:210,84.6854902841767)
--(axis cs:209,81.3144461885542)
--(axis cs:208,83.4834744023594)
--(axis cs:207,83.8036763362826)
--(axis cs:206,82.8289287536866)
--(axis cs:205,80.2184942754415)
--(axis cs:204,84.1057845109686)
--(axis cs:203,83.6819806387108)
--(axis cs:202,80.2023091317218)
--(axis cs:201,77.1519697479856)
--(axis cs:200,78.097462184982)
--(axis cs:199,78.9966610645608)
--(axis cs:198,83.0622429973677)
--(axis cs:197,84.7275537467096)
--(axis cs:196,81.6253588500537)
--(axis cs:195,81.9983652292338)
--(axis cs:194,81.5562898698756)
--(axis cs:193,76.5612790040111)
--(axis cs:192,77.7930987550139)
--(axis cs:191,73.1163734437674)
--(axis cs:190,75.1113834713759)
--(axis cs:189,76.2134793392199)
--(axis cs:188,77.5500158406916)
--(axis cs:187,78.0625198008645)
--(axis cs:186,81.5606497510806)
--(axis cs:185,79.6588121888507)
--(axis cs:184,79.6066819027301)
--(axis cs:183,78.3164357117459)
--(axis cs:182,79.4604613063491)
--(axis cs:181,76.1165766329363)
--(axis cs:180,74.9611374578371)
--(axis cs:179,75.2260051556297)
--(axis cs:178,80.1890897778704)
--(axis cs:177,82.2104455556714)
--(axis cs:176,85.8121402779225)
--(axis cs:175,81.8395920140698)
--(axis cs:174,82.6907400175873)
--(axis cs:173,79.3695083553174)
--(axis cs:172,81.3780521108135)
--(axis cs:171,79.2386484718502)
--(axis cs:170,78.4147272564794)
--(axis cs:169,80.6767424039326)
--(axis cs:168,81.5539280049157)
--(axis cs:167,83.7245766728113)
--(axis cs:166,84.0772208410141)
--(axis cs:165,82.304609384601)
--(axis cs:164,80.0720117307513)
--(axis cs:163,79.9395979967724)
--(axis cs:162,77.9814141626322)
--(axis cs:161,77.0338510366236)
--(axis cs:160,78.1502304624462)
--(axis cs:159,79.3791214113911)
--(axis cs:158,83.8485684309055)
--(axis cs:157,83.8432105386319)
--(axis cs:156,84.1532631732898)
--(axis cs:155,81.649745633279)
--(axis cs:154,80.3036820415987)
--(axis cs:153,78.421019218665)
--(axis cs:152,73.441690689998)
--(axis cs:151,75.9916966958308)
--(axis cs:150,82.2477042031218)
--(axis cs:149,82.2095469205689)
--(axis cs:148,85.1023503173778)
--(axis cs:147,89.368854563389)
--(axis cs:146,86.0661515375695)
--(axis cs:145,86.7231060886286)
--(axis cs:144,86.3868826107857)
--(axis cs:143,90.2831032634822)
--(axis cs:142,89.4871290793527)
--(axis cs:141,90.5655780158576)
--(axis cs:140,89.0803891864887)
--(axis cs:139,88.8751531497775)
--(axis cs:138,90.3483581038885)
--(axis cs:137,88.818530963194)
--(axis cs:136,87.5719970373259)
--(axis cs:135,89.297162963324)
--(axis cs:134,84.877953704155)
--(axis cs:133,84.8304421301937)
--(axis cs:132,82.5040526627422)
--(axis cs:131,79.6793991617611)
--(axis cs:130,84.0227489522013)
--(axis cs:129,87.028019523585)
--(axis cs:128,86.2667744044812)
--(axis cs:127,89.3735513389349)
--(axis cs:126,93.2658558403353)
--(axis cs:125,92.6903198004191)
--(axis cs:124,92.4208164171906)
--(axis cs:123,93.0090205214882)
--(axis cs:122,90.4861923185269)
--(axis cs:121,87.6064903981586)
--(axis cs:120,86.0643629976983)
--(axis cs:119,85.2613704137895)
--(axis cs:118,88.0932963505703)
--(axis cs:117,87.0077871048795)
--(axis cs:116,87.959150547766)
--(axis cs:115,90.0141881847075)
--(axis cs:114,92.207901897551)
--(axis cs:113,93.5732107052721)
--(axis cs:112,94.1825967149235)
--(axis cs:111,93.9863292269877)
--(axis cs:110,93.7908282004013)
--(axis cs:109,96.045368583835)
--(axis cs:108,97.0296273964604)
--(axis cs:107,97.8784509122422)
--(axis cs:106,95.1209803069694)
--(axis cs:105,91.7639753837117)
--(axis cs:104,95.504302562973)
--(axis cs:103,96.5044615370496)
--(axis cs:102,93.3128269213119)
--(axis cs:101,92.8557003183066)
--(axis cs:100,94.3259587312166)
--(axis cs:99,92.8451150806874)
--(axis cs:98,94.4138938508593)
--(axis cs:97,93.4577006469074)
--(axis cs:96,89.2872924753009)
--(axis cs:95,87.6476989274595)
--(axis cs:94,88.4076236593244)
--(axis cs:93,86.9501129074888)
--(axis cs:92,83.6934744676944)
--(axis cs:91,80.3784264179513)
--(axis cs:90,81.1478663557724)
--(axis cs:89,81.7762496113822)
--(axis cs:88,82.1951453475611)
--(axis cs:87,85.654598351118)
--(axis cs:86,86.4919979388976)
--(axis cs:85,85.3564974236219)
--(axis cs:84,85.0601217795274)
--(axis cs:83,85.3664855577426)
--(axis cs:82,82.265773613845)
--(axis cs:81,81.4317170173062)
--(axis cs:80,80.4228962716327)
--(axis cs:79,79.3868703395409)
--(axis cs:78,80.5154212577595)
--(axis cs:77,78.1026099055327)
--(axis cs:76,77.4027623819158)
--(axis cs:75,72.3191196440615)
--(axis cs:74,72.4320662217435)
--(axis cs:73,70.4978327771794)
--(axis cs:72,66.8551243048076)
--(axis cs:71,67.6934053810094)
--(axis cs:70,71.0331733929285)
--(axis cs:69,70.7656334078273)
--(axis cs:68,72.4902917597841)
--(axis cs:67,72.5294480330634)
--(axis cs:66,68.8368100413293)
--(axis cs:65,69.0374292183282)
--(axis cs:64,69.8631198562436)
--(axis cs:63,64.8452331536379)
--(axis cs:62,60.472208108714)
--(axis cs:61,59.3394268025592)
--(axis cs:60,57.340783503199)
--(axis cs:59,56.2507293789988)
--(axis cs:58,57.3297450570818)
--(axis cs:57,57.3444313213522)
--(axis cs:56,54.4629558183569)
--(axis cs:55,52.4701947729462)
--(axis cs:54,50.6209934661827)
--(axis cs:53,48.225908499395)
--(axis cs:52,45.7903022909105)
--(axis cs:51,41.6791278636381)
--(axis cs:50,40.8154098295476)
--(axis cs:49,41.1849289536012)
--(axis cs:48,40.8393278586682)
--(axis cs:47,40.8982431566686)
--(axis cs:46,41.0637206125024)
--(axis cs:45,41.9294840989613)
--(axis cs:44,40.7945217903683)
--(axis cs:43,41.2514022379603)
--(axis cs:42,43.5889194641171)
--(axis cs:41,42.0942326634797)
--(axis cs:40,41.375624162683)
--(axis cs:39,42.6437802033537)
--(axis cs:38,43.1126419208588)
--(axis cs:37,39.8569690677402)
--(axis cs:36,38.3376280013419)
--(axis cs:35,35.9712850016774)
--(axis cs:34,36.46393958543)
--(axis cs:33,34.0214244817875)
--(axis cs:32,34.8934472689011)
--(axis cs:31,32.8746424194597)
--(axis cs:30,35.0848863576579)
--(axis cs:29,32.7643579470724)
--(axis cs:28,35.0053641005072)
--(axis cs:27,35.7150384589673)
--(axis cs:26,36.8516314070424)
--(axis cs:25,34.8142892588031)
--(axis cs:24,36.0593615735038)
--(axis cs:23,37.9157853002131)
--(axis cs:22,34.083898291933)
--(axis cs:21,30.0114561982496)
--(axis cs:20,28.7720702478121)
--(axis cs:19,27.6484211430984)
--(axis cs:18,26.2853597622063)
--(axis cs:17,27.5649497027579)
--(axis cs:16,28.6893537951141)
--(axis cs:15,27.7028589105593)
--(axis cs:14,25.8944903048657)
--(axis cs:13,26.3260295477488)
--(axis cs:12,27.6907036013527)
--(axis cs:11,27.7467128350242)
--(axis cs:10,27.6664743771136)
--(axis cs:9,27.0160096380587)
--(axis cs:8,27.5695953809067)
--(axis cs:7,27.2450775594667)
--(axis cs:6,27.931263616)
--(axis cs:5,26.9389128533333)
--(axis cs:4,27.8069744)
--(axis cs:3,27.1336346666667)
--(axis cs:2,27.91696)
--(axis cs:1,28.1208666666667)
--(axis cs:0,29.7676666666667)
--cycle;

\path [fill=aligncolor, fill opacity=0.2]
(axis cs:0,28.8673333333333)
--(axis cs:0,20.0996666666667)
--(axis cs:1,19.3594666666667)
--(axis cs:2,20.76724)
--(axis cs:3,20.6537253333333)
--(axis cs:4,20.5029802666667)
--(axis cs:5,20.7753175466667)
--(axis cs:6,20.9267873706667)
--(axis cs:7,20.1746298965333)
--(axis cs:8,20.4129039172267)
--(axis cs:9,18.7703231337813)
--(axis cs:10,18.4295918403584)
--(axis cs:11,18.6770068056201)
--(axis cs:12,19.281405444496)
--(axis cs:13,19.0117243555968)
--(axis cs:14,18.9892461511441)
--(axis cs:15,19.877863587582)
--(axis cs:16,19.9151575367322)
--(axis cs:17,19.7519260293858)
--(axis cs:18,19.5348074901753)
--(axis cs:19,19.4208459921402)
--(axis cs:20,19.2099434603789)
--(axis cs:21,18.6878881016364)
--(axis cs:22,18.8569104813091)
--(axis cs:23,19.4585283850473)
--(axis cs:24,19.2468227080378)
--(axis cs:25,19.0639248330969)
--(axis cs:26,18.3844731998109)
--(axis cs:27,18.3671785598487)
--(axis cs:28,18.326942847879)
--(axis cs:29,19.3614209449698)
--(axis cs:30,19.7622700893092)
--(axis cs:31,19.9430160714474)
--(axis cs:32,21.2806128571579)
--(axis cs:33,22.497556952393)
--(axis cs:34,22.2312455619144)
--(axis cs:35,21.9314631161982)
--(axis cs:36,21.9449704929585)
--(axis cs:37,22.2092430610335)
--(axis cs:38,21.7406611154935)
--(axis cs:39,21.2591955590614)
--(axis cs:40,22.0668231139158)
--(axis cs:41,22.393191824466)
--(axis cs:42,22.0477534595728)
--(axis cs:43,21.9048694343249)
--(axis cs:44,22.1967622141266)
--(axis cs:45,22.8637431046346)
--(axis cs:46,22.424127817041)
--(axis cs:47,23.1726355869661)
--(axis cs:48,23.0179751362396)
--(axis cs:49,23.0207801089917)
--(axis cs:50,22.5759574205267)
--(axis cs:51,22.227432603088)
--(axis cs:52,23.6418127491371)
--(axis cs:53,24.2067168659763)
--(axis cs:54,26.2381068261144)
--(axis cs:55,27.9431521275582)
--(axis cs:56,27.6339883687132)
--(axis cs:57,26.8737240283039)
--(axis cs:58,26.9720458893098)
--(axis cs:59,29.5642367114478)
--(axis cs:60,28.8713227024916)
--(axis cs:61,28.1297248286599)
--(axis cs:62,31.0568465295946)
--(axis cs:63,30.4115438903424)
--(axis cs:64,30.5291017789406)
--(axis cs:65,32.4566147564858)
--(axis cs:66,32.5583584718553)
--(axis cs:67,31.7992867774842)
--(axis cs:68,32.505496088654)
--(axis cs:69,32.0772635375899)
--(axis cs:70,34.3817441634053)
--(axis cs:71,33.7915286640575)
--(axis cs:72,33.3928895979127)
--(axis cs:73,34.3276450116635)
--(axis cs:74,37.2347826759975)
--(axis cs:75,37.2668928074646)
--(axis cs:76,38.4399809126384)
--(axis cs:77,40.6649847301107)
--(axis cs:78,41.1905877840885)
--(axis cs:79,40.9924035606042)
--(axis cs:80,40.7121228484833)
--(axis cs:81,39.85523161212)
--(axis cs:82,41.010785289696)
--(axis cs:83,40.6948948984235)
--(axis cs:84,40.2422492520721)
--(axis cs:85,40.6733994016577)
--(axis cs:86,40.8117861879928)
--(axis cs:87,41.5958956170609)
--(axis cs:88,45.1567164936487)
--(axis cs:89,45.218573194919)
--(axis cs:90,42.5881252226019)
--(axis cs:91,41.4837668447482)
--(axis cs:92,41.2268801424652)
--(axis cs:93,42.2941041139722)
--(axis cs:94,43.5077499578444)
--(axis cs:95,43.8993999662755)
--(axis cs:96,46.3194533063537)
--(axis cs:97,49.340762645083)
--(axis cs:98,50.5125434493997)
--(axis cs:99,53.0423680928531)
--(axis cs:100,51.8127611409492)
--(axis cs:101,49.943275579426)
--(axis cs:102,50.9076204635408)
--(axis cs:103,50.7518963708326)
--(axis cs:104,50.8208504299994)
--(axis cs:105,51.9899470106662)
--(axis cs:106,50.0918909418663)
--(axis cs:107,49.6065794201597)
--(axis cs:108,48.5977968694611)
--(axis cs:109,50.2703041622355)
--(axis cs:110,50.3758433297884)
--(axis cs:111,52.7730079971641)
--(axis cs:112,52.1114063977313)
--(axis cs:113,53.4889917848517)
--(axis cs:114,54.8761267612147)
--(axis cs:115,55.4539014089717)
--(axis cs:116,54.0496544605107)
--(axis cs:117,53.0786569017419)
--(axis cs:118,52.4961921880602)
--(axis cs:119,54.6766204171148)
--(axis cs:120,53.4872296670252)
--(axis cs:121,53.6897837336202)
--(axis cs:122,51.6712269868961)
--(axis cs:123,54.1806482561836)
--(axis cs:124,53.0638519382802)
--(axis cs:125,51.4970815506242)
--(axis cs:126,51.883331907166)
--(axis cs:127,54.5933321923995)
--(axis cs:128,52.1277990872529)
--(axis cs:129,50.208905936469)
--(axis cs:130,50.4869247491752)
--(axis cs:131,50.3354064660068)
--(axis cs:132,53.6141251728055)
--(axis cs:133,53.9569001382444)
--(axis cs:134,52.4847201105955)
--(axis cs:135,52.5796427551431)
--(axis cs:136,52.1436475374478)
--(axis cs:137,53.3549180299582)
--(axis cs:138,53.6502677572999)
--(axis cs:139,53.6663475391733)
--(axis cs:140,52.966211364672)
--(axis cs:141,50.5993024250709)
--(axis cs:142,49.30557527339)
--(axis cs:143,46.964260218712)
--(axis cs:144,48.5580081749696)
--(axis cs:145,48.492939873309)
--(axis cs:146,50.0208185653139)
--(axis cs:147,48.3498548522511)
--(axis cs:148,48.5461505484676)
--(axis cs:149,47.5227871054407)
--(axis cs:150,45.5440963510192)
--(axis cs:151,44.6818770808154)
--(axis cs:152,44.3454349979856)
--(axis cs:153,43.5086146650552)
--(axis cs:154,43.3861583987108)
--(axis cs:155,42.0687267189687)
--(axis cs:156,42.0415147085083)
--(axis cs:157,42.5126784334733)
--(axis cs:158,40.9834760801119)
--(axis cs:159,41.6465141974229)
--(axis cs:160,41.2883446912716)
--(axis cs:161,41.576942419684)
--(axis cs:162,41.8812872690805)
--(axis cs:163,42.4580298152644)
--(axis cs:164,43.6991571855449)
--(axis cs:165,45.3125924151026)
--(axis cs:166,46.5699405987487)
--(axis cs:167,46.3488858123323)
--(axis cs:168,45.5789086498658)
--(axis cs:169,41.642860253226)
--(axis cs:170,40.6004215359141)
--(axis cs:171,38.6668705620646)
--(axis cs:172,38.072429782985)
--(axis cs:173,37.584543826388)
--(axis cs:174,40.2867017277771)
--(axis cs:175,41.2357613822217)
--(axis cs:176,45.4471424391107)
--(axis cs:177,44.0706472846219)
--(axis cs:178,45.3825844943642)
--(axis cs:179,45.2248675954913)
--(axis cs:180,43.6662274097264)
--(axis cs:181,47.5995152611144)
--(axis cs:182,47.4928122088916)
--(axis cs:183,49.0937831004466)
--(axis cs:184,50.6815598136906)
--(axis cs:185,50.3649811842858)
--(axis cs:186,49.938518280762)
--(axis cs:187,48.8633479579429)
--(axis cs:188,50.029145033021)
--(axis cs:189,50.0293160264168)
--(axis cs:190,49.3563861544668)
--(axis cs:191,48.3649755902401)
--(axis cs:192,45.7384471388587)
--(axis cs:193,47.696957711087)
--(axis cs:194,47.6901661688696)
--(axis cs:195,49.6253329350957)
--(axis cs:196,49.4666663480765)
--(axis cs:197,52.5199330784612)
--(axis cs:198,51.9014797961023)
--(axis cs:199,50.5877171702152)
--(axis cs:200,47.8895737361722)
--(axis cs:201,44.5907923222711)
--(axis cs:202,46.7993005244835)
--(axis cs:203,49.5789070862535)
--(axis cs:204,52.7628590023361)
--(axis cs:205,51.0634205352022)
--(axis cs:206,52.0770030948284)
--(axis cs:207,52.5147358091961)
--(axis cs:208,51.1380553140235)
--(axis cs:209,48.8037775845522)
--(axis cs:210,51.6226887343084)
--(axis cs:211,54.0766176541134)
--(axis cs:212,54.1077607899574)
--(axis cs:213,54.1187419652992)
--(axis cs:214,54.834860238906)
--(axis cs:215,52.2675548577915)
--(axis cs:216,50.9939772195665)
--(axis cs:217,51.0417817756532)
--(axis cs:218,50.9053587538559)
--(axis cs:219,51.8635536697514)
--(axis cs:220,49.7235762691345)
--(axis cs:221,50.8651276819742)
--(axis cs:222,53.7309021455794)
--(axis cs:223,52.4377883831302)
--(axis cs:224,49.6032973731708)
--(axis cs:225,51.76257123187)
--(axis cs:226,53.9359903188293)
--(axis cs:227,52.7420589217301)
--(axis cs:228,52.8115138040508)
--(axis cs:229,55.9820777099073)
--(axis cs:230,51.9520621679258)
--(axis cs:231,53.0282497343407)
--(axis cs:232,52.9546664541392)
--(axis cs:233,53.843599829978)
--(axis cs:234,54.6076798639824)
--(axis cs:235,56.2460772245193)
--(axis cs:236,58.8095284462821)
--(axis cs:237,57.980756090359)
--(axis cs:238,57.7178048722872)
--(axis cs:239,55.0742438978298)
--(axis cs:240,53.2924617849305)
--(axis cs:241,53.1603027612777)
--(axis cs:242,53.9277755423555)
--(axis cs:243,51.9950871005511)
--(axis cs:244,52.4292696804409)
--(axis cs:245,53.816349077686)
--(axis cs:246,52.8660125954821)
--(axis cs:247,52.732343409719)
--(axis cs:248,49.4390080611086)
--(axis cs:249,46.9105397822202)
--(axis cs:250,49.1549651591095)
--(axis cs:251,48.0567054606209)
--(axis cs:252,50.1984310351634)
--(axis cs:253,50.2450114947974)
--(axis cs:254,52.3223425291713)
--(axis cs:255,49.711074023337)
--(axis cs:256,50.8015925520029)
--(axis cs:257,48.607140708269)
--(axis cs:258,49.8985125666152)
--(axis cs:259,50.6184100532922)
--(axis cs:260,47.3011947093004)
--(axis cs:261,48.1999557674403)
--(axis cs:262,47.6524312806189)
--(axis cs:263,46.7950116911618)
--(axis cs:264,49.2219426862628)
--(axis cs:265,47.8774874823436)
--(axis cs:266,48.5811899858748)
--(axis cs:267,46.1182186553665)
--(axis cs:268,41.7344415909599)
--(axis cs:269,42.5273532727679)
--(axis cs:270,43.001549284881)
--(axis cs:271,42.4405727612381)
--(axis cs:272,45.8449915423238)
--(axis cs:273,48.9485932338591)
--(axis cs:274,47.2047412537539)
--(axis cs:275,47.3303930030031)
--(axis cs:276,47.3419144024025)
--(axis cs:277,49.8517981885887)
--(axis cs:278,47.7209052175376)
--(axis cs:279,46.8561241740301)
--(axis cs:280,43.1510993392241)
--(axis cs:281,40.9675461380459)
--(axis cs:282,39.6005702437701)
--(axis cs:283,40.0598561950161)
--(axis cs:284,40.0475516226795)
--(axis cs:285,41.6887746314769)
--(axis cs:286,41.6438863718482)
--(axis cs:287,41.0547090974786)
--(axis cs:288,38.7569006113162)
--(axis cs:289,40.612120489053)
--(axis cs:290,41.4890297245757)
--(axis cs:291,41.6978904463272)
--(axis cs:292,43.8381123570618)
--(axis cs:293,44.7634898856494)
--(axis cs:294,46.1901919085195)
--(axis cs:295,45.851286860149)
--(axis cs:296,44.0398294881192)
--(axis cs:297,44.5113969238287)
--(axis cs:298,44.2623842057296)
--(axis cs:299,43.789240697917)
--(axis cs:299,75.1640379107946)
--(axis cs:299,75.1640379107946)
--(axis cs:298,76.5549640551599)
--(axis cs:297,77.8924550689499)
--(axis cs:296,77.0137355028541)
--(axis cs:295,79.9251693785676)
--(axis cs:294,82.0062950565428)
--(axis cs:293,80.4993688206785)
--(axis cs:292,80.8233776925148)
--(axis cs:291,77.1447221156435)
--(axis cs:290,76.8218193112211)
--(axis cs:289,77.4771074723597)
--(axis cs:288,74.2625510071163)
--(axis cs:287,78.3446887588953)
--(axis cs:286,78.4281942819525)
--(axis cs:285,79.8763261857739)
--(axis cs:284,76.9699077322174)
--(axis cs:283,78.0288013319385)
--(axis cs:282,79.1685849982564)
--(axis cs:281,80.9258145811539)
--(axis cs:280,80.2070182264423)
--(axis cs:279,85.3081061163862)
--(axis cs:278,87.3017159788161)
--(axis cs:277,90.3583949735202)
--(axis cs:276,87.5551603835669)
--(axis cs:275,84.8605338127919)
--(axis cs:274,86.8582505993233)
--(axis cs:273,86.1890632491541)
--(axis cs:272,82.2278290614426)
--(axis cs:271,76.4509529934699)
--(axis cs:270,77.5966912418374)
--(axis cs:269,77.7875307189634)
--(axis cs:268,76.3753300653709)
--(axis cs:267,83.0015792483803)
--(axis cs:266,85.3429740604754)
--(axis cs:265,85.6702175755943)
--(axis cs:264,87.7544386361595)
--(axis cs:263,86.1262149618661)
--(axis cs:262,85.4319353689993)
--(axis cs:261,86.3980858779157)
--(axis cs:260,85.430440680728)
--(axis cs:259,89.92130085091)
--(axis cs:258,88.9842093969709)
--(axis cs:257,86.7375117462136)
--(axis cs:256,89.987139682767)
--(axis cs:255,90.0839246034588)
--(axis cs:254,93.4955724209902)
--(axis cs:253,90.4767155262377)
--(axis cs:252,89.5624777411305)
--(axis cs:251,86.4595138430798)
--(axis cs:250,87.3491423038497)
--(axis cs:249,85.1442612131455)
--(axis cs:248,87.9049098497652)
--(axis cs:247,93.0808873122064)
--(axis cs:246,93.3501924735914)
--(axis cs:245,93.4944072586559)
--(axis cs:244,89.8511757399866)
--(axis cs:243,91.0869696749832)
--(axis cs:242,94.5335454270623)
--(axis cs:241,91.5827651171612)
--(axis cs:240,91.6355397297849)
--(axis cs:239,92.0438413288978)
--(axis cs:238,96.3961349944555)
--(axis cs:237,99.294335409736)
--(axis cs:236,96.9845025955034)
--(axis cs:235,96.7137949110459)
--(axis cs:234,93.942160305474)
--(axis cs:233,94.2352003818425)
--(axis cs:232,94.9018338106365)
--(axis cs:231,92.6759589299623)
--(axis cs:230,92.8447819957862)
--(axis cs:229,100.597227494733)
--(axis cs:228,96.2214510350827)
--(axis cs:227,94.3261471271866)
--(axis cs:226,95.03210057565)
--(axis cs:225,90.2727090528958)
--(axis cs:224,89.8648863161198)
--(axis cs:223,94.1888578951497)
--(axis cs:222,95.5356557022705)
--(axis cs:221,92.3523196278381)
--(axis cs:220,90.2530662014643)
--(axis cs:219,92.924249418497)
--(axis cs:218,90.7048117731212)
--(axis cs:217,90.8805980497349)
--(axis cs:216,89.3671642288353)
--(axis cs:215,90.7837052860441)
--(axis cs:214,94.8704649408885)
--(axis cs:213,94.0959978427773)
--(axis cs:212,93.4199973034716)
--(axis cs:211,94.6657466293395)
--(axis cs:210,90.6821832866743)
--(axis cs:209,87.0599791083429)
--(axis cs:208,92.183307218762)
--(axis cs:207,93.8273006901191)
--(axis cs:206,93.2407091959822)
--(axis cs:205,90.7493031616445)
--(axis cs:204,92.7695456187222)
--(axis cs:203,89.7200153567361)
--(axis cs:202,86.6146858625869)
--(axis cs:201,82.8849406615669)
--(axis cs:200,87.6535924936253)
--(axis cs:199,91.7499906170316)
--(axis cs:198,92.9121549379562)
--(axis cs:197,91.9785270057786)
--(axis cs:196,89.9479087572233)
--(axis cs:195,91.1428859465291)
--(axis cs:194,89.0027740998281)
--(axis cs:193,88.5700509581184)
--(axis cs:192,83.795563697648)
--(axis cs:191,83.6357879553934)
--(axis cs:190,85.8524849442417)
--(axis cs:189,88.4568561803021)
--(axis cs:188,89.9699868920443)
--(axis cs:187,86.9528169483887)
--(axis cs:186,89.9818545188192)
--(axis cs:185,88.209068148524)
--(axis cs:184,88.2589185189884)
--(axis cs:183,86.5973981487354)
--(axis cs:182,82.8958310192526)
--(axis cs:181,82.4855387740658)
--(axis cs:180,78.2984234675822)
--(axis cs:179,82.5645293344778)
--(axis cs:178,79.5885783347639)
--(axis cs:177,76.7772229184549)
--(axis cs:176,80.7711119814019)
--(axis cs:175,75.4541399767524)
--(axis cs:174,73.5675083042739)
--(axis cs:173,69.1839687136757)
--(axis cs:172,71.3295442254279)
--(axis cs:171,70.5192636151182)
--(axis cs:170,73.5238295188978)
--(axis cs:169,75.3794535652889)
--(axis cs:168,81.4492336232778)
--(axis cs:167,84.5527086957639)
--(axis cs:166,83.3472192030382)
--(axis cs:165,81.8081073371311)
--(axis cs:164,81.5681341714139)
--(axis cs:163,78.3175010476007)
--(axis cs:162,77.4382929761676)
--(axis cs:161,78.2136162202095)
--(axis cs:160,77.9166869419285)
--(axis cs:159,78.2038586774106)
--(axis cs:158,76.44549001343)
--(axis cs:157,80.3056125167874)
--(axis cs:156,79.431682312651)
--(axis cs:155,79.3715195574804)
--(axis cs:154,82.3639827801838)
--(axis cs:153,81.3630618085631)
--(axis cs:152,82.0870772607039)
--(axis cs:151,82.7828465758798)
--(axis cs:150,84.0358082198498)
--(axis cs:149,86.5775936081456)
--(axis cs:148,88.0384086768487)
--(axis cs:147,88.2299275127275)
--(axis cs:146,88.903576057576)
--(axis cs:145,89.4710534053034)
--(axis cs:144,86.1789834232959)
--(axis cs:143,84.8960626124532)
--(axis cs:142,89.1949949322331)
--(axis cs:141,90.4183269986247)
--(axis cs:140,94.3641587482809)
--(axis cs:139,96.7715317686845)
--(axis cs:138,94.803498044189)
--(axis cs:137,93.9370392219029)
--(axis cs:136,91.6286323607119)
--(axis cs:135,92.8769571175566)
--(axis cs:134,92.0531130636124)
--(axis cs:133,95.3074746628488)
--(axis cs:132,92.0160099952277)
--(axis cs:131,88.5679291607013)
--(axis cs:130,90.3931614508767)
--(axis cs:129,89.0997851469292)
--(axis cs:128,90.0497314336615)
--(axis cs:127,94.4701642920768)
--(axis cs:126,91.7867053650961)
--(axis cs:125,90.4651317063701)
--(axis cs:124,91.6723312996293)
--(axis cs:123,95.2644974578699)
--(axis cs:122,92.3806218223374)
--(axis cs:121,96.8085272779218)
--(axis cs:120,97.1674090974022)
--(axis cs:119,101.116594705086)
--(axis cs:118,95.8282433813576)
--(axis cs:117,96.816304226697)
--(axis cs:116,98.4451302833713)
--(axis cs:115,100.439079520881)
--(axis cs:114,98.8316827344343)
--(axis cs:113,96.6311867513762)
--(axis cs:112,94.4127334392203)
--(axis cs:111,95.3074167990253)
--(axis cs:110,89.940854332115)
--(axis cs:109,90.6238179151438)
--(axis cs:108,87.737605727263)
--(axis cs:107,91.1470071590788)
--(axis cs:106,90.6754256155152)
--(axis cs:105,94.459782019394)
--(axis cs:104,91.9738108575758)
--(axis cs:103,91.0991802386364)
--(axis cs:102,90.6488086316289)
--(axis cs:101,91.0693441228694)
--(axis cs:100,92.2345968202534)
--(axis cs:99,93.5261626919835)
--(axis cs:98,90.107120031646)
--(axis cs:97,89.2495667062242)
--(axis cs:96,84.3950417161136)
--(axis cs:95,80.643802145142)
--(axis cs:94,79.3879193480941)
--(axis cs:93,77.309732518451)
--(axis cs:92,75.2862489813971)
--(axis cs:91,75.1073945600797)
--(axis cs:90,76.9839932000997)
--(axis cs:89,81.7956581667912)
--(axis cs:88,82.0693227084891)
--(axis cs:87,77.2356533856113)
--(axis cs:86,74.9190667320141)
--(axis cs:85,74.7820834150177)
--(axis cs:84,76.0190209354388)
--(axis cs:83,74.2711095026318)
--(axis cs:82,73.7116368782897)
--(axis cs:81,73.6969627645288)
--(axis cs:80,75.5618701223277)
--(axis cs:79,75.7850043195763)
--(axis cs:78,74.4141720661371)
--(axis cs:77,72.2167150826713)
--(axis cs:76,70.2866438533392)
--(axis cs:75,70.2661381500073)
--(axis cs:74,68.4238393541758)
--(axis cs:73,60.8943825260531)
--(axis cs:72,60.2174781575664)
--(axis cs:71,59.754097696958)
--(axis cs:70,60.7175387878641)
--(axis cs:69,59.5960901514968)
--(axis cs:68,59.8019460227044)
--(axis cs:67,59.4523491950471)
--(axis cs:66,61.0566031604756)
--(axis cs:65,60.0525872839278)
--(axis cs:64,57.2486507715764)
--(axis cs:63,57.8355634644705)
--(axis cs:62,59.0937876639215)
--(axis cs:61,52.8078179132352)
--(axis cs:60,53.5429390582107)
--(axis cs:59,52.5453404894301)
--(axis cs:58,47.3556756117876)
--(axis cs:57,45.1194278480678)
--(axis cs:56,47.3741181434181)
--(axis cs:55,47.8088143459393)
--(axis cs:54,46.0599345990908)
--(axis cs:53,43.6566682488635)
--(axis cs:52,41.203251977746)
--(axis cs:51,39.1033983055159)
--(axis cs:50,38.2540812152282)
--(axis cs:49,39.8507681857019)
--(axis cs:48,37.954126898794)
--(axis cs:47,38.9842419568258)
--(axis cs:46,37.0803024460323)
--(axis cs:45,38.2499613908737)
--(axis cs:44,35.7119517385921)
--(axis cs:43,35.7896896732402)
--(axis cs:42,36.2360287582169)
--(axis cs:41,36.9533692811044)
--(axis cs:40,36.0161282680472)
--(axis cs:39,34.6024936683923)
--(axis cs:38,35.5697837521571)
--(axis cs:37,37.628646356863)
--(axis cs:36,36.5853079460787)
--(axis cs:35,37.2315515992651)
--(axis cs:34,38.9806894990814)
--(axis cs:33,40.0085285405184)
--(axis cs:32,39.4437440089813)
--(axis cs:31,34.6863466778933)
--(axis cs:30,35.9077666807)
--(axis cs:29,34.317708350875)
--(axis cs:28,33.1551354385937)
--(axis cs:27,34.0935026315754)
--(axis cs:26,34.008544956136)
--(axis cs:25,31.0105978618366)
--(axis cs:24,31.6624973272958)
--(axis cs:23,31.9363716591198)
--(axis cs:22,31.1699645738997)
--(axis cs:21,32.3541223840413)
--(axis cs:20,34.4923196467183)
--(axis cs:19,31.8818995583978)
--(axis cs:18,31.4094577813306)
--(axis cs:17,32.41998889333)
--(axis cs:16,32.7249027833291)
--(axis cs:15,30.7726284791614)
--(axis cs:14,28.8402022656184)
--(axis cs:13,29.125002832023)
--(axis cs:12,30.0145035400288)
--(axis cs:11,29.3346294250359)
--(axis cs:10,28.8597034479616)
--(axis cs:9,30.1412959766187)
--(axis cs:8,32.9178699707733)
--(axis cs:7,33.4386707968)
--(axis cs:6,34.989338496)
--(axis cs:5,34.5615064533333)
--(axis cs:4,31.7839664)
--(axis cs:3,32.3378746666667)
--(axis cs:2,30.91376)
--(axis cs:1,28.5005333333333)
--(axis cs:0,28.8673333333333)
--cycle;
\addplot [very thick, sourcecolor]
table {%
0 21.436
1 21.0158
2 20.5534933333333
3 19.9938613333333
4 19.1089224
5 18.75913792
6 17.912630336
7 17.3677442688
8 16.5248020817067
9 15.9969816653653
10 15.2353653322923
11 14.6524322658338
12 14.1509658126671
13 13.7973593168003
14 13.3366607867736
15 12.7897619627522
16 12.4806429035351
17 12.1138143228281
18 12.1793381249291
19 11.9342038332766
20 11.778109733288
21 11.6620677866304
22 11.5562942293043
23 11.4044687167768
24 11.4438749734214
25 11.6416866454038
26 11.7694426496564
27 12.0272607863918
28 11.8857552957801
29 11.8434842366241
30 11.8656273892993
31 11.8773419114394
32 12.0508468624849
33 12.1396974899879
34 12.152444658657
35 12.5695023935922
36 13.1383152482071
37 13.3100388652324
38 13.4442844255192
39 14.4151608737487
40 15.047248698999
41 14.0486589591992
42 13.3926605006927
43 13.3849617338875
44 13.4166627204433
45 13.5913568430213
46 13.4821988077504
47 14.194325712867
48 14.7002739036269
49 14.9335324562349
50 17.1719592983212
51 16.375467438657
52 17.7722539509256
53 24.2220764940738
54 29.436721195259
55 33.3302969562072
56 36.5011042316325
57 40.100923385306
58 42.9432787082448
59 45.1472496332625
60 45.55367970661
61 47.3096704319547
62 51.0400630122304
63 54.146157076451
64 57.3620989944941
65 62.3723325289286
66 66.2974993564762
67 69.438579485181
68 71.0258102548114
69 74.1173682038492
70 75.5320145630793
71 80.2775649837968
72 85.0123719870374
73 90.4326375896299
74 93.7837167383706
75 99.9196267240298
76 102.752048045891
77 106.963991770046
78 108.234200082703
79 106.307673399496
80 102.791665386263
81 108.144618975677
82 111.505948513875
83 114.8845188111
84 116.209081715547
85 120.813918705771
86 121.050861631283
87 123.853675971693
88 122.475660777355
89 122.15977528855
90 123.44224023084
91 124.785718851339
92 124.140201747738
93 127.14212139819
94 125.562303785219
95 123.742356361508
96 125.474351755873
97 124.931454738032
98 125.471883790426
99 124.812733699007
100 121.024000292539
101 125.624873567365
102 125.846218853892
103 126.594955083113
104 125.432637399824
105 129.618249919859
106 128.089046602554
107 128.38604394871
108 128.847988492301
109 128.104410793841
110 124.824881968406
111 129.177365574725
112 130.97733245978
113 133.303512634491
114 133.462863440926
115 132.611670752741
116 130.671583268859
117 127.762986615087
118 128.763262625403
119 128.693710100323
120 126.269021413591
121 128.608710464206
122 131.945395038032
123 135.094522697092
124 133.792891491007
125 131.620113192806
126 130.440130554245
127 132.941637776729
128 133.531723554717
129 129.167232177107
130 128.543299075019
131 128.421739260015
132 127.187304741345
133 130.829530459743
134 133.517217701128
135 133.685320827569
136 135.766423328722
137 134.011898662977
138 132.882398930382
139 130.673799144305
140 132.790412648778
141 135.576430119022
142 134.087937428551
143 132.926149942841
144 133.043673287606
145 132.118265296751
146 134.340072237401
147 135.260317789921
148 133.93098756527
149 132.443916718883
150 128.652720041773
151 127.657916033418
152 126.020726160068
153 128.017114261388
154 129.941824742443
155 129.780479793955
156 131.160077168497
157 132.321468401464
158 132.761574721172
159 131.087399776937
160 131.531206488216
161 133.034485190573
162 132.188028152459
163 130.3907758553
164 128.08596068424
165 131.664528547392
166 131.93958950458
167 133.876211603664
168 133.878862616265
169 133.094996759678
170 133.945524074409
171 132.713205926194
172 133.131451407622
173 134.472701126098
174 134.728920900878
175 135.561823387369
176 138.650985376562
177 136.577221634583
178 137.493637307666
179 137.158443179466
180 137.702587876906
181 139.848950301525
182 139.76322024122
183 139.136269526309
184 139.789948954381
185 139.928312496838
186 138.495223330804
187 135.958538664643
188 133.478990931714
189 132.469826078705
190 133.950187529631
191 136.038203357038
192 137.166576018964
193 140.669947481838
194 139.17365798547
195 138.865386388376
196 140.234629110701
197 136.089476621894
198 138.027334630849
199 133.345047704679
};
\addlegendentry{Source}
\addplot [very thick, ourcolor]
table {%
0 19.6847666666667
1 19.6316133333333
2 18.125164
3 17.9047112
4 17.6009022933333
5 17.1142218346667
6 16.7445574677333
7 16.38099930752
8 15.9944661126827
9 15.5964862234795
10 14.8002956454502
11 14.5697898496935
12 14.0753185464215
13 13.4860481704705
14 13.5212918697097
15 12.8048934957678
16 12.7938814632809
17 12.5733918372914
18 12.1939201364998
19 12.1149894425332
20 11.8309182206932
21 11.6903612432212
22 11.4910823279103
23 11.3231991956616
24 11.2355326898626
25 10.9204594852234
26 11.2236809215121
27 11.350658070543
28 11.9019597897677
29 12.5384744984808
30 13.160272932118
31 13.4515116790277
32 13.1405560098889
33 12.9225448079111
34 13.0273225129955
35 13.6892713437298
36 14.3805770749838
37 14.198121659987
38 13.9226039946563
39 14.084283195725
40 15.35420655658
41 14.9813919119307
42 14.3007535295446
43 14.4795494903023
44 14.4225595922418
45 15.7852810071268
46 16.0274381390348
47 17.0026771778945
48 18.0264084089823
49 19.9490067271858
50 22.5021520484153
51 20.6927016387322
52 20.6978479776525
53 19.940498382122
54 20.2232653723642
55 22.7436456312247
56 23.5128498383131
57 22.6894465373172
58 23.0593172298537
59 22.044533783883
60 25.3067070271064
61 22.5916322883518
62 20.6006458306814
63 21.1012099978785
64 25.5872746649694
65 30.2495263986422
66 32.3440811189138
67 36.091584895131
68 36.9349612494381
69 35.6486356662172
70 34.3853285329738
71 35.2620961597123
72 35.1324569277699
73 34.6992722088826
74 33.2270977671061
75 34.1926648803515
76 35.3424519042812
77 38.3022681900916
78 37.9309945520733
79 37.4993423083253
80 37.3997271799936
81 35.0986350773282
82 39.4090147285292
83 45.0759917828234
84 51.6585200929254
85 55.5130560743403
86 56.8179581928056
87 60.5099932209111
88 63.9919412433956
89 64.2535596613831
90 65.6018143957732
91 67.7342848499519
92 71.1207878799615
93 76.6931436373025
94 80.107514909842
95 83.2630585945403
96 85.4609002089656
97 87.3823535005058
98 86.9416894670713
99 87.3098249069904
100 86.1750932589256
101 89.0801879404738
102 93.5490303523791
103 95.0400909485699
104 96.6686660921893
105 96.9136595404181
106 98.7124342990011
107 98.6502407725342
108 98.5619126180274
109 101.331663427755
110 100.197224075538
111 100.70797926043
112 105.008396741677
113 107.487144060009
114 110.26840858134
115 113.899120198405
116 112.640429492058
117 112.907110260313
118 114.55900820825
119 115.530159899934
120 113.76636125328
121 114.407309002624
122 114.912940535433
123 117.173885761679
124 118.514801942677
125 116.315594887475
126 118.58009590998
127 121.469636727984
128 118.473096049054
129 115.281710172576
130 117.661961471394
131 116.773735843782
132 117.098355341692
133 117.443030940021
134 120.37371808535
135 119.31807446828
136 116.453579574624
137 115.478876993032
138 115.874941594426
139 113.971013275541
140 112.649517287099
141 111.930853829679
142 112.930156397077
143 113.822771784328
144 113.379777427463
145 115.43950194197
146 115.676288220243
147 115.527290576194
148 114.076979127622
149 110.143656635431
150 108.091898641678
151 113.580118913342
152 112.441908464007
153 113.984820104539
154 117.242202750298
155 120.129382200238
156 121.889619093524
157 121.214188608153
158 120.829317553189
159 119.640314042551
160 117.720304567374
161 116.770350320566
162 118.311453589786
163 117.803669538496
164 117.128722297463
165 117.361104504637
166 118.590930270376
167 114.583010882968
168 112.421402039708
169 110.609561631766
170 109.07939597208
171 109.428296777664
172 107.693524088798
173 109.238972604371
174 107.48511141683
175 107.877735800131
176 106.407648640105
177 103.930678912084
178 103.368089796334
179 103.123211837067
180 102.418282802987
181 103.710079575723
182 107.575803660578
183 106.562462928463
184 110.274603676103
185 111.897756274216
186 112.059318352706
187 112.513081348832
188 117.057805079065
189 116.284210729919
190 115.004795250602
191 113.790849533815
192 111.539039627052
193 113.646658368308
194 112.717546694647
195 118.314550689051
196 120.893027217907
197 122.639495107659
198 120.707476086127
199 123.330454202235
};
\addlegendentry{Ours}
\addplot [very thick, singlecolor]
table {%
0 23.0789333333333
1 22.5650733333333
2 22.045272
3 20.9651042666667
4 20.18971008
5 18.969208064
6 18.0195131178667
7 17.1240704942933
8 16.517929728768
9 16.2354571163477
10 15.0597123597449
11 14.8961565544625
12 14.32648524357
13 13.768868194856
14 13.5408678892182
15 12.9398543113745
16 12.8217101157663
17 12.7065014259464
18 12.0560878074238
19 12.192290245939
20 12.0120455300845
21 11.830929757401
22 11.4648104725874
23 11.34194837807
24 11.1022853691226
25 10.8908882952981
26 10.8821306362385
27 10.9953978423241
28 11.1401982738593
29 13.0066919524208
30 13.4346668952699
31 13.1653268495493
32 12.7143814796394
33 12.2902385170449
34 12.0336641469692
35 11.9115446509087
36 11.771515720727
37 11.7974259099149
38 12.1195140612653
39 12.9553445823455
40 13.8085689992098
41 14.3585085327011
42 13.4571201594943
43 12.9778227942621
44 12.6810449020763
45 12.5562825883277
46 12.5990127373288
47 11.9601235231964
48 11.9289321518905
49 11.9107257215124
50 11.9470939105432
51 12.2394417951013
52 11.9137067694143
53 11.8152920821981
54 11.5025803324252
55 11.1599709326068
56 11.2868234127521
57 11.6649453968684
58 11.373029650828
59 11.1098770539957
60 11.1131216431966
61 10.8038839812239
62 10.5424605183125
63 10.1135417479833
64 10.18994673172
65 10.6123040520427
66 12.7589965749675
67 12.7346639266406
68 13.8152711413125
69 13.6348302463833
70 13.4500508637733
71 14.0299006910187
72 14.1450072194816
73 15.1967057755853
74 15.6239712871349
75 16.4820303630412
76 16.3379709570997
77 16.1857900990131
78 16.8212787458771
79 16.9654496633684
80 16.1111463973614
81 16.7244104512224
82 16.3160216943113
83 16.8967906887823
84 16.4499925510259
85 16.4948140408207
86 16.1877578993232
87 17.8190596527919
88 18.3603943889002
89 17.9995555111202
90 18.5858510755628
91 18.9311675271169
92 18.6018006883602
93 18.6926072173548
94 20.2349857738839
95 22.0935352857738
96 24.6762548952857
97 24.9675905828952
98 25.5196457996495
99 25.9075366397196
100 26.238382645109
101 27.7248194494205
102 27.5922622262031
103 28.3982231142958
104 29.6894984914367
105 29.3992787931493
106 28.9831230345195
107 31.1500784276156
108 31.3393960754258
109 30.9663768603406
110 31.5729281549392
111 31.4805358572847
112 33.0171686858277
113 34.9427482819955
114 37.4635386255964
115 40.5692442338105
116 42.7668487203817
117 45.9069923096387
118 49.2731005143776
119 51.3530404115021
120 51.9547789958683
121 49.3651831966947
122 52.6973132240224
123 53.3927305792179
124 51.7145044633743
125 50.3427435706995
126 50.2698615232262
127 52.4301158852477
128 53.5377127081981
129 56.7946034998918
130 57.4150961332468
131 54.6064835732641
132 53.0972201919446
133 53.452329486889
134 52.2294569228446
135 54.4012322049423
136 56.6501657639539
137 58.7774526111631
138 57.2213154222638
139 58.046672337811
140 59.5562712035822
141 59.6937836295324
142 56.8405202369593
143 56.9759495229007
144 54.0498262849873
145 54.9661876946565
146 53.3315301557252
147 54.2108507912468
148 54.4904739663308
149 52.7387858397313
150 50.423628671785
151 50.699082937428
152 53.6313863499424
153 53.8268024132873
154 56.6617485972965
155 58.6881322111705
156 61.2109524356031
157 62.3643886151491
158 62.220637558786
159 62.1344767136954
160 63.0067613709564
161 63.1366957634317
162 65.0025566107454
163 66.737871955263
164 69.1496642308771
165 69.9600180513683
166 70.7823544410946
167 71.9885635528757
168 71.5280241756339
169 71.4448593405071
170 66.9871941390724
171 67.6934086445912
172 66.6471002490063
173 69.4268668658717
174 71.4292334926974
175 73.4353467941579
176 72.6657307686596
177 74.6247846149277
178 79.2114210252755
179 79.2345768202204
180 81.787668122843
181 76.7396944982744
182 76.1962422652862
183 74.7157404788956
184 77.1746857164498
185 78.3089352398265
186 78.3949148585279
187 78.721258553489
188 79.6178135094578
189 77.4230841408996
190 75.9100073127197
191 74.2156591835091
192 72.5000540134739
193 75.0893898774458
194 75.6820919019567
195 78.3975668548987
196 74.8984868172523
197 73.7907361204685
198 73.7865955630415
199 72.8355831170998
200 72.5310131603465
201 72.0278905282772
202 72.3408124226218
203 71.6430499380974
204 72.0558799504779
205 71.2093639603823
206 69.2028178349725
207 70.955774267978
208 68.5284327477158
209 70.1776661981726
210 70.0491262918714
211 70.6318210334971
212 67.9453634934644
213 63.7450574614382
214 65.7767859691505
215 66.6577221086538
216 66.6328310202563
217 65.8750781495384
218 63.2638958529641
219 62.4874100157046
220 60.8334546792303
221 58.7829304100509
222 59.1212509947074
223 60.4667874624326
224 61.5971299699461
225 60.7414039759569
226 63.5904231807655
227 62.2127452112791
228 62.0697561690233
229 64.1911982685519
230 64.5865186148416
231 63.9805282252066
232 62.1662959134986
233 64.3223100641322
234 65.7513080513058
235 64.8993464410446
236 66.3391171528357
237 67.7889803889352
238 65.1816243111482
239 64.2728861155852
240 64.2296888924682
241 66.2081111139745
242 66.2281822245129
243 68.370972446277
244 70.5006646236883
245 74.9668583656173
246 75.4447066924938
247 79.0713986873284
248 79.8709656165294
249 76.7620524932235
250 75.4095353279121
251 71.3264882623297
252 70.4845506098638
253 69.252740487891
254 74.0787390569795
255 74.0580645789169
256 73.8087116631335
257 73.6735026638402
258 74.6449621310721
259 73.770803038191
260 72.9264357638862
261 71.4720619444423
262 69.3828762222205
263 67.2973343111097
264 67.6317407822211
265 67.2633792924436
266 65.8367367672882
267 67.0004827471639
268 68.8809795310644
269 70.9615369581849
270 70.0651228998812
271 67.0655316532383
272 64.4002119892573
273 63.0010829247392
274 61.4657396731247
275 65.6332650718331
276 63.9280520574665
277 62.2083483126398
278 62.2168919834452
279 59.4129002534228
280 62.5121068694049
281 59.3421788288573
282 61.6373963964192
283 60.001883783802
284 60.4426603603749
285 63.4165949549666
286 62.3239892973066
287 63.951198104512
288 61.9917651502762
289 62.5901587868877
290 61.8364803628435
291 63.1381309569414
292 64.4528980988865
293 65.9117251457758
294 66.1839267832873
295 65.9283480932965
296 64.6605251413039
297 64.2832401130431
298 63.2246587571012
299 62.1870403390143
};
\addlegendentry{Single}
\addplot [very thick, auxcolor]
table {%
0 21.9247
1 21.4189466666667
2 19.716404
3 19.1203432
4 18.1098012266667
5 17.3881409813333
6 16.9741327850667
7 16.52919289472
8 16.383234315776
9 15.9339674526208
10 14.9520006287633
11 15.069633836344
12 14.7140937357418
13 14.0009816552601
14 13.7217453242081
15 13.2709762593665
16 13.1975676741599
17 12.9185274726612
18 12.8077886447956
19 12.8392442491699
20 12.4737820660025
21 12.307965652802
22 11.8259591889083
23 11.66124068446
24 11.587712547568
25 11.3981100380544
26 11.9107280304435
27 12.7610757576881
28 12.6729206061505
29 13.5974898182537
30 13.8646051879363
31 13.9297774836824
32 13.3054686536126
33 12.9772015895567
34 12.7724546049787
35 13.1673370173163
36 13.553609613853
37 14.3086343577491
38 14.8198074861993
39 16.0592859889594
40 16.0032487911675
41 15.600019032934
42 14.6611885596806
43 13.7266375144111
44 13.2984300115289
45 13.7162306758898
46 14.4042912073785
47 14.5135396325695
48 14.9834983727222
49 15.0317920315111
50 15.3699536252089
51 14.9239495668338
52 14.0183129868004
53 14.0339303894403
54 15.5544976448856
55 15.2128847825751
56 15.5404678260601
57 15.9924142608481
58 15.7151847420118
59 15.3525411269428
60 15.4402929015542
61 14.7236476545767
62 13.927364790328
63 13.9812651655958
64 15.5955654658099
65 15.611692372648
66 16.5962072314517
67 16.6457057851614
68 16.1861379614624
69 16.7386503691699
70 17.9689002953359
71 16.8032935696021
72 16.808828189015
73 16.6644358845453
74 17.2721087076363
75 18.5326936327757
76 18.0561882395539
77 18.6014639249764
78 19.4130378066478
79 20.9031035786516
80 22.6133961962546
81 22.5910636236703
82 22.1047108989363
83 22.782388719149
84 22.8929509753192
85 26.938087446922
86 26.3975766242043
87 27.8908146326968
88 28.4270717061574
89 30.0273773649259
90 32.6479085586074
91 31.6724601802193
92 31.4658681441754
93 31.9931945153403
94 32.1172889456056
95 32.4783778231511
96 33.5301555918542
97 34.0700311401501
98 34.3451982454534
99 37.3462385963627
100 38.5134508770902
101 36.6269340350055
102 37.4801805613377
103 38.8371444490702
104 42.0152088925895
105 43.2366204474049
106 45.2387030245906
107 47.3690024196725
108 49.3524086024046
109 48.4071668819237
110 48.7489468388723
111 46.3417174710978
112 49.0578006435449
113 50.636820514836
114 51.8708964118688
115 56.601457129495
116 60.6961190369293
117 65.3342352295435
118 68.7442148503014
119 69.9560518802411
120 72.7346281708596
121 74.1429892033543
122 75.0315313626835
123 78.9163117568134
124 78.1068360721174
125 77.8484488576939
126 77.9699457528218
127 79.2280632689241
128 78.082117281806
129 79.8062938254448
130 81.3679483936891
131 83.1706720482847
132 84.7555043052944
133 86.1775101109022
134 87.0303280887217
135 90.8466558043107
136 93.1286446434486
137 94.5132023814255
138 97.2190819051404
139 97.3364855241123
140 101.207315085957
141 98.3753854020986
142 100.645928321679
143 101.501895990676
144 101.480390125874
145 99.0253321006996
146 96.251579013893
147 97.2551632111144
148 99.4953572355582
149 99.0825924551132
150 102.667847297424
151 98.9821778379391
152 98.8059422703513
153 98.6129204829477
154 99.1594830530248
155 97.9212864424199
156 101.464289153936
157 99.7081579898154
158 98.0007397251857
159 100.443391780149
160 100.746126757452
161 99.2695347392951
162 103.247987791436
163 103.790903566482
164 104.941136186519
165 104.620755615882
166 101.935244492706
167 102.155742260831
168 103.254533808665
169 101.333207046932
170 101.742825637546
171 102.670240510036
172 100.458485741362
173 102.115501926423
174 103.133968207805
175 101.876787899578
176 100.189490319662
177 99.589625589063
178 98.9429071379171
179 101.439539043667
180 101.119931234934
181 101.40843832128
182 102.072470657024
183 103.215409858953
184 105.199094553829
185 104.764628976396
186 105.647809847784
187 104.169287878227
188 100.881456969248
189 103.219092242065
190 102.259247126986
191 102.362337701588
192 103.012703494604
193 101.109856129017
194 102.408638236547
195 98.2885905892373
196 95.0094524713898
197 95.4530686437785
198 94.1384349150228
199 91.0416479320183
200 90.7304050122813
201 91.1677773431583
202 93.2055418745267
203 92.0918334996213
204 90.7490734663637
205 95.7682454397576
206 91.5710296851394
207 89.9349970814449
208 93.7228176651559
209 93.9605807987914
210 94.5623179723664
211 85.8280610445598
212 87.1301021689812
213 88.0596217351849
214 84.6132307214813
215 83.718504577185
216 81.099483661748
217 79.8618669293984
218 80.1015468768521
219 78.090570834815
220 78.0841900011853
221 78.1187120009482
222 78.3501962674253
223 78.7935903472735
224 79.6767522778188
225 81.0827351555884
226 78.998841457804
227 77.8963198329099
228 80.1527625329946
229 83.3681500263957
230 80.0243600211165
231 79.2979346835599
232 83.2891877468479
233 84.0954435308117
234 82.7687548246493
235 83.2738305263861
236 81.2290044211089
237 81.9461035368871
238 83.100716162843
239 79.1625862636077
240 80.0145490108862
241 76.7452725420423
242 78.6231380336338
243 76.0244104269071
244 76.755961674859
245 79.1559826732205
246 83.2736861385764
247 85.7729155775278
248 84.9492524620222
249 82.7445086362845
250 83.8437002423609
251 83.9203801938887
252 83.2301374884443
253 80.8159499907554
254 85.5980333259377
255 84.9629733274168
256 83.1052319952668
257 83.9075655962134
258 85.3350391436374
259 86.7341513149099
260 85.7637610519279
261 82.5378288415423
262 80.2270097399005
263 81.4645877919204
264 83.6640635668697
265 80.5603508534957
266 82.1796340161299
267 81.4811272129039
268 79.1276684369898
269 77.3617880829252
270 78.7483971330068
271 79.9044843730721
272 79.9598941651244
273 80.6465219987661
274 76.8342575990129
275 79.2794660792103
276 77.6998661967016
277 74.6801596240279
278 75.812074365889
279 75.3733928260446
280 77.6033009275023
281 76.3897607420018
282 76.5247285936015
283 73.6090362082145
284 71.1267956332383
285 70.3520631732573
286 71.7039372052725
287 72.3199030975513
288 71.1783091447077
289 69.0524539824328
290 66.2241231859463
291 64.0693318820904
292 65.8273388390056
293 69.8212377378712
294 72.5927701902969
295 73.1681028189042
296 71.01206892179
297 73.4000684707654
298 70.1880681099456
299 69.4066544879565
};
\addlegendentry{Auxiliary}
\addplot [very thick, tunecolor]
table {%
0 24.175
1 23.0817533333333
2 22.9577826666667
3 22.2640394666667
4 22.5734049066667
5 21.8283439253333
6 22.6575151402667
7 22.0232321122133
8 22.1548323564373
9 21.8670325518165
10 22.0957793747866
11 21.9014301664959
12 21.9925241331967
13 21.0883993065574
14 20.9574061119126
15 21.7148915561967
16 21.7504265782907
17 21.1242612626326
18 20.3842756767727
19 21.3005205414182
20 21.7473564331345
21 22.6058251465076
22 23.9740801172061
23 25.6957507604315
24 25.1810872750119
25 24.6671631533429
26 26.0764305226743
27 25.6803777514728
28 25.5529088678449
29 24.5051404276092
30 25.5434656754207
31 24.3763992070032
32 26.0988926989359
33 25.5352674924821
34 27.439887327319
35 27.1433031951885
36 28.4300825561508
37 29.3156127115873
38 31.5128101692699
39 30.9896814687492
40 30.5206785083327
41 31.2189628066662
42 31.9353102453329
43 30.6322681962663
44 30.7918278903464
45 31.7147356456105
46 31.0974818498217
47 30.9506188131907
48 31.0822817172192
49 31.5681253737754
50 31.1572802990203
51 31.4752709058829
52 34.0042700580397
53 35.7214693797651
54 36.921075503812
55 37.536153736383
56 39.520309655773
57 41.2641943912851
58 40.8410088463614
59 40.4960737437558
60 41.5727456616713
61 43.0168898626704
62 44.1192652234696
63 47.089825512109
64 51.0698404096872
65 51.0570656610831
66 50.5915391955332
67 54.1302846897599
68 54.4898544184746
69 53.685476868113
70 54.4118614944904
71 51.550195862259
72 50.6014233564738
73 52.2555453518457
74 53.9967962814766
75 53.9599770251813
76 58.0332682868117
77 58.449981296116
78 60.6758717035595
79 59.7743906961809
80 59.5688925569447
81 58.9877940455558
82 59.1229552364446
83 61.785937522489
84 61.6593100179912
85 61.4740146810596
86 62.4586517448477
87 62.4685613958782
88 60.5081757833692
89 59.7255206266954
90 59.312403168023
91 57.915489201085
92 60.5629380275347
93 63.4967704220278
94 64.9371096709555
95 63.7609477367644
96 65.1206248560782
97 68.8944798848626
98 69.9626105745567
99 68.224975126312
100 69.2276467677163
101 67.121577414173
102 68.1965219313384
103 70.5644842117374
104 70.2658607027233
105 67.9885285621786
106 70.5936961830762
107 72.5996436131277
108 71.7157615571688
109 70.886649245735
110 69.386259396588
111 69.6471675172704
112 69.891080680483
113 69.7688112110531
114 69.3514823021758
115 67.7865191750739
116 66.0941553400592
117 64.8136376053807
118 65.5097700843045
119 64.4627560674436
120 64.8423515206216
121 64.7503278831639
122 66.9422089731978
123 68.9802671785582
124 68.2474670761799
125 69.6598469942773
126 69.9552375954218
127 66.7526900763375
128 64.52169206107
129 65.0518069821893
130 62.3674455857514
131 58.7636564686012
132 61.8180851748809
133 64.1465014732381
134 63.5567611785905
135 67.0416889428724
136 65.2836444876312
137 67.1851622567716
138 68.0393498054173
139 66.0031598443339
140 66.6107612088004
141 67.6097089670403
142 67.5255138402989
143 67.4365577389058
144 64.7364528577913
145 65.0536422862331
146 64.5988004956531
147 67.3256137298558
148 63.639304317218
149 60.2060367871077
150 60.4034294296862
151 55.5149568770823
152 54.3448188349992
153 58.2287684013327
154 59.6920613877328
155 61.3838291101862
156 63.0889566214823
157 61.9452119638525
158 62.202389571082
159 59.5976183235323
160 58.4290613254925
161 56.830809060394
162 56.7133205816485
163 57.7082831319855
164 58.0072798389217
165 59.665250537804
166 61.6653404302432
167 61.7478190108613
168 59.325015208689
169 58.3161988336179
170 57.4687790668943
171 58.0609432535154
172 60.5228279361457
173 58.9747690155832
174 61.8599085457999
175 62.0836401699733
176 65.4553054693119
177 62.4254243754496
178 61.027252833693
179 57.1551356002877
180 57.4613818135635
181 58.4283054508508
182 60.884657694014
183 60.0560528218778
184 60.8863555908356
185 61.4088511393352
186 62.6238742448015
187 60.6900260625078
188 60.6320675166729
189 59.755820680005
190 59.0325898773374
191 57.1740719018699
192 59.7417575214959
193 58.5534260171967
194 62.5694941470907
195 63.0718219843392
196 62.6426309208047
197 65.0073714033104
198 63.576703789315
199 59.7348896981187
200 59.0535784251616
201 57.9058627401293
202 59.9979301921034
203 62.4128108203494
204 63.0777753229462
205 60.9214869250236
206 62.0309362066856
207 62.4056822986818
208 62.4051125056121
209 60.8715366711563
210 62.4036426702584
211 60.8526074695401
212 63.121865975632
213 63.5756327805056
214 62.9925595577378
215 61.1847343128569
216 57.2775674502856
217 58.1450406268951
218 61.4450791681828
219 62.5414166678795
220 62.203366667637
221 59.0786066674429
222 58.016112000621
223 57.0121229338301
224 56.9584783470641
225 58.0952226776513
226 58.375258142121
227 58.6942265136968
228 58.3810478776241
229 55.8111783020993
230 56.8568893083461
231 56.0416181133436
232 53.6152211573415
233 50.9273035925399
234 50.1298095406986
235 48.5380342992255
236 46.3936207727137
237 47.2734499515043
238 49.1975599612035
239 51.0336079689628
240 51.2559263751702
241 51.0119744334695
242 50.1539662134423
243 49.2218129707538
244 49.7699170432697
245 48.2282403012824
246 47.5524055743593
247 47.1818444594874
248 48.4553555675899
249 49.6653777874053
250 50.6507955632576
251 50.6838631172727
252 51.5824704938182
253 51.0164763950545
254 48.545474449377
255 49.5895595595016
256 50.3553743142679
257 52.9011794514143
258 51.1748702277981
259 48.1558628489052
260 46.6036569457908
261 46.678478889966
262 47.6557431119728
263 48.3739011562449
264 50.1874809249959
265 55.0341780733301
266 55.9983757919974
267 55.2444673002646
268 54.808827173545
269 54.6995284055027
270 54.6890893910688
271 54.1297781795217
272 56.5375025436174
273 56.9639020348939
274 54.1382282945818
275 50.5977359689988
276 48.9840954418657
277 48.2698230201592
278 47.0791184161274
279 48.0879013995686
280 47.7901011196548
281 45.9430142290572
282 46.1288513832458
283 46.68967443993
284 51.687039551944
285 52.3432383082218
286 52.0632506465775
287 52.4367271839286
288 53.2817150804762
289 53.0118987310477
290 49.9756589848381
291 48.7434471878705
292 48.5904844169631
293 47.1446342002371
294 46.0502540268564
295 45.4145232214851
296 47.1758652438547
297 47.6829655284171
298 45.6891124227337
299 45.3343966048536
};
\addlegendentry{Finetune}
\addplot [very thick, aligncolor]
table {%
0 24.2569333333333
1 23.6586133333333
2 25.5525173333333
3 26.0061805333333
4 25.7363510933333
5 26.9937875413333
6 27.2575966997333
7 26.1369773597867
8 26.0970552211627
9 23.9345508435968
10 23.1785406748774
11 23.565272539902
12 24.2602980319216
13 23.7041584255372
14 23.6188200737631
15 24.8984760590105
16 25.6725608472084
17 25.4816153444334
18 24.9694989422134
19 25.1265991537707
20 25.8743193230166
21 24.6829154584133
22 24.2833657000639
23 24.8780592267178
24 24.7737073813743
25 24.4877792384327
26 24.9608167240795
27 25.0510400459303
28 24.6975787034109
29 25.9673629627287
30 26.9688370368496
31 26.612542962813
32 29.6768810369171
33 30.571398162867
34 30.0022318636269
35 29.0702454909016
36 28.7676163927212
37 29.3502664475103
38 28.1741531580083
39 27.5154358597399
40 28.720388687792
41 29.3328442835669
42 28.7727220935202
43 28.4376776748161
44 28.5597621398529
45 30.0693230452157
46 29.4006784361725
47 30.837982748938
48 30.2580061991504
49 30.887051625987
50 29.9271279674563
51 30.0365490406317
52 31.8107725658387
53 32.9274247193376
54 35.2595797754701
55 37.0751438203761
56 36.7440683896342
57 35.336741378374
58 36.2094797693659
59 40.1807104821594
60 39.8678883857275
61 39.2385240419153
62 43.8500059001989
63 42.9387447201591
64 42.8681891094606
65 45.2389512875685
66 45.9360676967215
67 44.6966674907105
68 45.4256006592351
69 45.0841871940547
70 46.9231164219104
71 46.206219804195
72 46.137475843356
73 47.0258406746848
74 51.9679925397478
75 52.7113940317983
76 53.2898618921053
77 55.4404361803509
78 56.6282356109474
79 56.8820284887579
80 56.7353027910063
81 55.4525022328051
82 56.3227751195774
83 56.2807667623286
84 57.0238067431962
85 56.5052587278903
86 56.7349403156456
87 58.3404922525165
88 62.7935471353465
89 62.6513443749439
90 59.0159688332884
91 57.5471750666307
92 57.5733600533046
93 59.1542480426437
94 60.9457051007816
95 61.7149040806253
96 64.4365832645002
97 68.1090399449335
98 69.2973986226135
99 72.1559322314241
100 70.8116791184726
101 69.2081766281114
102 69.3922679691558
103 69.553107708658
104 69.8955128335931
105 71.8113436002078
106 68.8560548801662
107 68.9125905707997
108 66.6822191233064
109 69.0392352986451
110 68.7866482389161
111 72.9392985911329
112 72.2039388729063
113 74.1196244316584
114 75.9484195453267
115 77.2239089695947
116 75.5946138423424
117 74.1364844072073
118 73.4704875257658
119 77.0467166872793
120 74.4255666831568
121 74.3514066798588
122 71.123785343887
123 73.8712016084429
124 71.6143146200877
125 70.2581116960701
126 71.0073760235228
127 73.7172074854849
128 70.1745459883879
129 68.7082501240437
130 69.4634067659016
131 68.6342054127213
132 71.9919376635104
133 73.686176797475
134 71.38184143798
135 71.8216264837173
136 70.9670878536405
137 72.6784302829124
138 73.1563708929966
139 73.984923381064
140 72.4142120381845
141 69.4811029638809
142 68.1311023711047
143 64.8889818968838
144 66.4550121841737
145 68.025089747339
146 68.6302117978712
147 67.3587761049636
148 67.2136075506375
149 65.9771127071767
150 63.7645901657414
151 62.6903921325931
152 62.2340403727411
153 61.2901589648596
154 61.6593338385543
155 59.6291270708435
156 59.7385216566748
157 60.2633839920065
158 57.7229471936052
159 58.9497844215508
160 58.7738342039073
161 58.9380340297925
162 58.695427223834
163 59.5999084457339
164 61.9358200899204
165 62.883902738603
166 64.2986955242158
167 64.7005164193726
168 62.9302131354981
169 57.7456305083985
170 56.4147110733854
171 53.7808888587084
172 53.8174577536333
173 52.4858262029067
174 55.8600009623253
175 57.4820207698603
176 62.5295699492216
177 59.9714692927106
178 62.2263087675018
179 63.4750736806681
180 60.5177922778678
181 64.5030871556276
182 64.6643230578354
183 67.534265112935
184 69.123872090348
185 68.9258576722784
186 69.217399471156
187 67.2367329102582
188 68.9931129948732
189 68.3727237292319
190 66.7097789833855
191 65.2281365200417
192 63.6586758827001
193 67.0907340394934
194 67.6627538982614
195 69.6514564519424
196 69.105205161554
197 71.7079507959098
198 71.6030539700612
199 70.1821098427156
200 66.4988612075058
201 62.368462299338
202 65.1817565061371
203 68.081658538243
204 71.489753497261
205 69.9472561311422
206 71.6933515715804
207 71.8517812572643
208 70.3221716724781
209 66.9169306713158
210 70.1811912037193
211 73.0730262963088
212 72.591001037047
213 72.731234162971
214 73.3674673303768
215 70.1219605309681
216 68.9061017581078
217 69.7494014064862
218 69.664281125189
219 71.2717582334845
220 69.1651265867876
221 70.7845946027634
222 73.9561290155441
223 72.6505832124353
224 69.1412332366149
225 70.3492332559586
226 73.7976532714335
227 72.7706426171468
228 73.7509674270508
229 77.5799139416406
230 71.7816044866458
231 72.26675692265
232 73.2682988714533
233 73.4869257638293
234 73.9966539443968
235 75.9674898221841
236 77.3383518577473
237 78.0947414861978
238 76.5671598556249
239 72.9328812178333
240 71.4407583075999
241 71.5901599794133
242 73.5176879835306
243 70.9605037201578
244 70.7801829761263
245 73.0661930475677
246 72.5452277713875
247 72.1744288837767
248 67.9107364403547
249 65.3126958189504
250 67.7223966551603
251 66.7831706574616
252 69.2002098593026
253 69.5492412207754
254 72.0762263099537
255 68.9650210479629
256 69.6602901717037
257 66.9742188040296
258 68.7846150432237
259 69.6934853679123
260 65.8186682943298
261 66.8457813021305
262 66.0151383750378
263 65.7798173666969
264 68.0614072266908
265 66.293019114686
266 66.4887286250821
267 63.987456233399
268 58.4672383200526
269 59.7111506560421
270 59.644573858167
271 58.9609257532003
272 63.7320472692269
273 67.4269044820482
274 66.4791435856385
275 65.4715348685108
276 66.7861545614753
277 69.5499036491803
278 66.9679762526775
279 65.6603276688087
280 61.2071354683803
281 60.4369550413709
282 58.6628240330967
283 58.3550925598107
284 58.1021273811819
285 60.2845819049455
286 59.3187921906231
287 58.9183070858318
288 55.6274656686655
289 58.180879201599
290 58.3406766946126
291 58.6329546890234
292 61.496937084552
293 61.8390896676416
294 63.43629840078
295 62.1579920539573
296 59.9362803098325
297 60.6782509145327
298 59.8878807316261
299 58.9589712519676
};
\addlegendentry{Time-aligned}

==> figs/subfig_cheetah.tex <==
\nextgroupplot[ 
title = {Cheetah}
]

\path [draw=sourcecolor, fill=sourcecolor, opacity=0.25]
(axis cs:0,207.902644970233)
--(axis cs:0,191.831502350144)
--(axis cs:1,492.868804727583)
--(axis cs:2,625.441181501587)
--(axis cs:3,669.529953663893)
--(axis cs:4,703.79727314691)
--(axis cs:5,724.881866761351)
--(axis cs:6,737.901576471254)
--(axis cs:7,726.850831995898)
--(axis cs:8,729.986990412421)
--(axis cs:9,771.744283134398)
--(axis cs:9,797.35861290106)
--(axis cs:9,797.35861290106)
--(axis cs:8,784.391168361048)
--(axis cs:7,770.653134139791)
--(axis cs:6,747.651307325264)
--(axis cs:5,755.926210281424)
--(axis cs:4,713.706105824865)
--(axis cs:3,700.168212600787)
--(axis cs:2,673.617267958567)
--(axis cs:1,557.991311233892)
--(axis cs:0,207.902644970233)
--cycle;

\path [draw=singlecolor, fill=singlecolor, opacity=0.25]
(axis cs:0,198.599346162565)
--(axis cs:0,179.90648532961)
--(axis cs:1,352.491600004381)
--(axis cs:2,359.113169894587)
--(axis cs:3,437.584637139243)
--(axis cs:4,386.752610030574)
--(axis cs:5,452.818534331418)
--(axis cs:6,462.105808570268)
--(axis cs:7,471.191969861788)
--(axis cs:8,453.048903454905)
--(axis cs:9,445.308119260931)
--(axis cs:9,487.638327319847)
--(axis cs:9,487.638327319847)
--(axis cs:8,497.236275536688)
--(axis cs:7,550.294100146159)
--(axis cs:6,540.011344156501)
--(axis cs:5,523.863952621867)
--(axis cs:4,482.942709818012)
--(axis cs:3,491.802205749171)
--(axis cs:2,394.895808965121)
--(axis cs:1,410.351959222161)
--(axis cs:0,198.599346162565)
--cycle;

\path [draw=ourcolor, fill=ourcolor, opacity=0.25]
(axis cs:0,194.695615934737)
--(axis cs:0,181.73516942581)
--(axis cs:1,381.591782834057)
--(axis cs:2,484.064497649354)
--(axis cs:3,529.471074610907)
--(axis cs:4,545.96857085794)
--(axis cs:5,552.831833543155)
--(axis cs:6,571.813618607036)
--(axis cs:7,590.290738588118)
--(axis cs:8,607.959134678948)
--(axis cs:9,609.654794634609)
--(axis cs:9,650.555468262409)
--(axis cs:9,650.555468262409)
--(axis cs:8,638.440856102104)
--(axis cs:7,620.590385737189)
--(axis cs:6,613.799976371042)
--(axis cs:5,599.681531704714)
--(axis cs:4,597.077679169069)
--(axis cs:3,574.954810771127)
--(axis cs:2,506.414795562167)
--(axis cs:1,409.801965262942)
--(axis cs:0,194.695615934737)
--cycle;

\path [draw=auxcolor, fill=auxcolor, opacity=0.25]
(axis cs:0,179.76384890887)
--(axis cs:0,171.541846098312)
--(axis cs:1,353.249077030134)
--(axis cs:2,400.089696733579)
--(axis cs:3,464.98596215118)
--(axis cs:4,475.899457545471)
--(axis cs:5,491.952488467856)
--(axis cs:6,520.019062792394)
--(axis cs:7,542.964427997587)
--(axis cs:8,553.56110178082)
--(axis cs:9,559.676898084762)
--(axis cs:9,602.783681967598)
--(axis cs:9,602.783681967598)
--(axis cs:8,596.508936046606)
--(axis cs:7,580.565456961485)
--(axis cs:6,571.983648514414)
--(axis cs:5,544.704383653909)
--(axis cs:4,536.089674579693)
--(axis cs:3,519.814345216449)
--(axis cs:2,418.468699548445)
--(axis cs:1,381.977559071068)
--(axis cs:0,179.76384890887)
--cycle;

\path [draw=tunecolor, fill=tunecolor, opacity=0.25]
(axis cs:0,203.892576796391)
--(axis cs:0,184.187514108616)
--(axis cs:1,384.909447632736)
--(axis cs:2,424.572008051)
--(axis cs:3,458.04122593703)
--(axis cs:4,463.658090110088)
--(axis cs:5,497.373296015004)
--(axis cs:6,510.131259629636)
--(axis cs:7,525.89085344572)
--(axis cs:8,554.496684504139)
--(axis cs:9,536.684024504506)
--(axis cs:9,603.356591580685)
--(axis cs:9,603.356591580685)
--(axis cs:8,611.549577950775)
--(axis cs:7,592.393702060146)
--(axis cs:6,574.212965662729)
--(axis cs:5,562.084659267693)
--(axis cs:4,577.500044361388)
--(axis cs:3,504.106605545737)
--(axis cs:2,480.407446928424)
--(axis cs:1,425.887864804737)
--(axis cs:0,203.892576796391)
--cycle;

\path [draw=aligncolor, fill=aligncolor, opacity=0.25]
(axis cs:0,182.041273462905)
--(axis cs:0,175.877699133955)
--(axis cs:1,318.312366426722)
--(axis cs:2,394.704002562536)
--(axis cs:3,434.674450710602)
--(axis cs:4,447.175654593568)
--(axis cs:5,450.486961511993)
--(axis cs:6,451.378458960343)
--(axis cs:7,459.322899371637)
--(axis cs:8,466.093117990537)
--(axis cs:9,471.559963321842)
--(axis cs:9,559.337017586039)
--(axis cs:9,559.337017586039)
--(axis cs:8,546.814678963202)
--(axis cs:7,539.359806817437)
--(axis cs:6,531.348091142683)
--(axis cs:5,521.783069423896)
--(axis cs:4,519.542444827647)
--(axis cs:3,504.178721909893)
--(axis cs:2,416.065233410349)
--(axis cs:1,363.253835734476)
--(axis cs:0,182.041273462905)
--cycle;

\addplot [semithick, sourcecolor]
table {%
0 200.655692826384
1 527.323075930595
2 651.178701691926
3 683.715487147097
4 708.245013827208
5 739.2891816659
6 742.452679838358
7 749.726465995097
8 758.672233885867
9 784.497096778985
};
\addlegendentry{Source}

\addplot [semithick, singlecolor]
table {%
0 188.881352921584
1 380.588011516177
2 377.571661941599
3 463.470845755998
4 434.298247272079
5 487.882063115174
6 499.00459206061
7 509.321815349304
8 475.440872186581
9 465.619134436305
};
\addlegendentry{Without Transfer}
\addplot [semithick, ourcolor]
table {%
0 188.533786432264
1 396.294870203832
2 495.348353775272
3 552.39623947499
4 572.295017352543
5 577.135093779887
6 593.466315660652
7 605.871462120734
8 623.459809100769
9 631.421007868601
};
\addlegendentry{With Transfer}
\addplot [semithick, auxcolor]
table {%
0 175.601051642895
1 365.275510941878
2 408.97268576091
3 491.615935301933
4 504.187546676194
5 517.282095880204
6 542.271566931003
7 561.404754995274
8 573.196614936404
9 581.147007512805
};
\addlegendentry{Auxiliary Tasks}
\addplot [semithick, tunecolor]
table {%
0 194.328733547028
1 404.690597848387
2 454.402345358587
3 481.630046464068
4 525.311715481507
5 528.78776446986
6 543.11126825726
7 561.528569107191
8 584.112119844749
9 568.531585324439
};
\addlegendentry{Fine-tune}
\addplot [semithick, aligncolor]
table {%
0 178.628417197807
1 340.036721283328
2 404.526601663728
3 465.04690228254
4 480.408384178008
5 484.224520196241
6 489.740666266114
7 495.70885221505
8 505.556841140709
9 514.006344102661
};
\addlegendentry{Time-aligned}
\legend{};

==> halfcheetah_ablation.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={HalfCheetah},
x grid style={white!69.0196078431373!black},
xlabel={steps},
xmajorgrids,
xmin=-4.95, xmax=103.95,
xtick style={color=black},
xtick={0,20,40,60,80,100},
xticklabels={0k,200k,400k,600k,800k,1000k},
y grid style={white!69.0196078431373!black},
ylabel={Return},
ymajorgrids,
ymin=-240.674849660313, ymax=4667.87126650874,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.25]
(axis cs:0,-4.86148704856668)
--(axis cs:0,-17.5591171071745)
--(axis cs:1,51.1807257704293)
--(axis cs:2,229.478935904115)
--(axis cs:3,448.93792198758)
--(axis cs:4,657.525204760701)
--(axis cs:5,757.207708252639)
--(axis cs:6,701.869778418762)
--(axis cs:7,759.366205411334)
--(axis cs:8,795.083782295168)
--(axis cs:9,888.796808502576)
--(axis cs:10,873.303965999891)
--(axis cs:11,965.748649024855)
--(axis cs:12,932.145979641106)
--(axis cs:13,927.466093586972)
--(axis cs:14,971.046906932384)
--(axis cs:15,1033.46308367243)
--(axis cs:16,1126.23850912815)
--(axis cs:17,1164.34520949092)
--(axis cs:18,1196.43983301424)
--(axis cs:19,1265.79933943031)
--(axis cs:20,1259.71535664198)
--(axis cs:21,1341.23107583601)
--(axis cs:22,1418.50650749061)
--(axis cs:23,1546.69437012274)
--(axis cs:24,1498.12664853701)
--(axis cs:25,1537.21567787302)
--(axis cs:26,1589.3980625322)
--(axis cs:27,1667.97544158709)
--(axis cs:28,1639.94660937953)
--(axis cs:29,1666.97281766284)
--(axis cs:30,1719.14397346101)
--(axis cs:31,1702.56248560516)
--(axis cs:32,1789.46028337378)
--(axis cs:33,1827.50605094207)
--(axis cs:34,1818.18539735303)
--(axis cs:35,1835.37310504401)
--(axis cs:36,1873.14717246469)
--(axis cs:37,1850.21121090857)
--(axis cs:38,1890.80118715084)
--(axis cs:39,1906.1778271455)
--(axis cs:40,1917.81410125555)
--(axis cs:41,1918.27077471886)
--(axis cs:42,1906.90951395059)
--(axis cs:43,1940.9378802823)
--(axis cs:44,1966.49550484835)
--(axis cs:45,1855.21963803132)
--(axis cs:46,1962.70875161607)
--(axis cs:47,1967.17871312954)
--(axis cs:48,1985.80208675596)
--(axis cs:49,1966.70145832544)
--(axis cs:50,1956.31438170074)
--(axis cs:51,2007.40005485832)
--(axis cs:52,1960.94457203168)
--(axis cs:53,2115.76406628063)
--(axis cs:54,2073.14380478075)
--(axis cs:55,2062.73894867009)
--(axis cs:56,2069.68845920919)
--(axis cs:57,2099.27344654391)
--(axis cs:58,2108.23750765726)
--(axis cs:59,2137.53995349505)
--(axis cs:60,2125.28148950372)
--(axis cs:61,2095.50566468756)
--(axis cs:62,2131.85670650373)
--(axis cs:63,2154.08177409947)
--(axis cs:64,2090.4217368938)
--(axis cs:65,2205.56467756056)
--(axis cs:66,2167.37700874322)
--(axis cs:67,2110.42398533225)
--(axis cs:68,2165.6675132361)
--(axis cs:69,2239.90314905439)
--(axis cs:70,2257.45096951806)
--(axis cs:71,2184.80701985497)
--(axis cs:72,2253.61589662606)
--(axis cs:73,2271.75713675878)
--(axis cs:74,2247.44848749397)
--(axis cs:75,2293.38808919841)
--(axis cs:76,2327.3338124809)
--(axis cs:77,2344.50823743256)
--(axis cs:78,2383.46044865038)
--(axis cs:79,2338.58097866277)
--(axis cs:80,2378.77371255312)
--(axis cs:81,2329.94024828125)
--(axis cs:82,2401.21599876009)
--(axis cs:83,2404.93176530972)
--(axis cs:84,2462.09922111143)
--(axis cs:85,2416.58321139241)
--(axis cs:86,2472.18820156346)
--(axis cs:87,2401.75734499535)
--(axis cs:88,2521.78214117514)
--(axis cs:89,2448.4385863152)
--(axis cs:90,2454.36633291909)
--(axis cs:91,2547.48116026531)
--(axis cs:92,2452.19452140337)
--(axis cs:93,2498.5337474189)
--(axis cs:94,2553.05102193357)
--(axis cs:95,2558.58855809078)
--(axis cs:96,2545.24526888484)
--(axis cs:97,2536.47260310106)
--(axis cs:98,2538.69264305889)
--(axis cs:99,2466.10031442603)
--(axis cs:99,3429.73633614058)
--(axis cs:99,3429.73633614058)
--(axis cs:98,3600.19483203576)
--(axis cs:97,3609.05898310111)
--(axis cs:96,3595.56040284393)
--(axis cs:95,3572.28024972714)
--(axis cs:94,3613.24166875524)
--(axis cs:93,3544.66762501971)
--(axis cs:92,3528.62248720776)
--(axis cs:91,3492.78707671457)
--(axis cs:90,3517.667690518)
--(axis cs:89,3488.36895708831)
--(axis cs:88,3515.97021563052)
--(axis cs:87,3408.86697033635)
--(axis cs:86,3431.67246057134)
--(axis cs:85,3405.30515463493)
--(axis cs:84,3355.36328210851)
--(axis cs:83,3367.5712022178)
--(axis cs:82,3344.26577317076)
--(axis cs:81,3331.87986626372)
--(axis cs:80,3360.95944769142)
--(axis cs:79,3192.03867513452)
--(axis cs:78,3337.41284049053)
--(axis cs:77,3334.67930968438)
--(axis cs:76,3203.52318082358)
--(axis cs:75,3165.48306262993)
--(axis cs:74,3196.9657868547)
--(axis cs:73,3170.37831381546)
--(axis cs:72,3085.88128515625)
--(axis cs:71,3135.26280986177)
--(axis cs:70,3172.04581537129)
--(axis cs:69,3042.49156585731)
--(axis cs:68,3130.95983024521)
--(axis cs:67,3006.23351914661)
--(axis cs:66,3010.36084991637)
--(axis cs:65,3061.96904802812)
--(axis cs:64,2960.86823235794)
--(axis cs:63,3021.00020237101)
--(axis cs:62,3024.30063303229)
--(axis cs:61,3006.1056918483)
--(axis cs:60,2979.47533509475)
--(axis cs:59,2989.14048143868)
--(axis cs:58,2902.36073242958)
--(axis cs:57,2964.00134115517)
--(axis cs:56,2856.08535549337)
--(axis cs:55,2897.64980906998)
--(axis cs:54,2918.53210815763)
--(axis cs:53,2907.1098009003)
--(axis cs:52,2841.92852717021)
--(axis cs:51,2842.81428213655)
--(axis cs:50,2840.14069204298)
--(axis cs:49,2809.02737598103)
--(axis cs:48,2746.34388983844)
--(axis cs:47,2803.95951577019)
--(axis cs:46,2800.78461369805)
--(axis cs:45,2685.20930384405)
--(axis cs:44,2722.30905640814)
--(axis cs:43,2686.57615406201)
--(axis cs:42,2659.9353500308)
--(axis cs:41,2660.46619329571)
--(axis cs:40,2611.91254176405)
--(axis cs:39,2641.52294218534)
--(axis cs:38,2648.59991959234)
--(axis cs:37,2551.10348217818)
--(axis cs:36,2558.98761300813)
--(axis cs:35,2513.87523127286)
--(axis cs:34,2472.57193422726)
--(axis cs:33,2485.78011361719)
--(axis cs:32,2430.33583935113)
--(axis cs:31,2351.62944426776)
--(axis cs:30,2260.16818253518)
--(axis cs:29,2271.80487765026)
--(axis cs:28,2216.17344222787)
--(axis cs:27,2274.73924856425)
--(axis cs:26,2182.78462728207)
--(axis cs:25,2105.03297091567)
--(axis cs:24,2002.76471098274)
--(axis cs:23,2063.81917319444)
--(axis cs:22,1931.4797890585)
--(axis cs:21,1893.3911672037)
--(axis cs:20,1759.62364531051)
--(axis cs:19,1840.82107672777)
--(axis cs:18,1765.11613068137)
--(axis cs:17,1708.06697480238)
--(axis cs:16,1662.18933618276)
--(axis cs:15,1590.71041692961)
--(axis cs:14,1515.01317841607)
--(axis cs:13,1430.18553005668)
--(axis cs:12,1372.34166219899)
--(axis cs:11,1429.94729091468)
--(axis cs:10,1384.97568876844)
--(axis cs:9,1309.70085830112)
--(axis cs:8,1226.24186587736)
--(axis cs:7,1132.24292067991)
--(axis cs:6,1102.01694138893)
--(axis cs:5,1074.31466392856)
--(axis cs:4,916.552807066411)
--(axis cs:3,729.373016177397)
--(axis cs:2,532.826825376399)
--(axis cs:1,155.669164879405)
--(axis cs:0,-4.86148704856668)
--cycle;

\path [draw=green!50.1960784313725!black, fill=green!50.1960784313725!black, opacity=0.25]
(axis cs:0,47.2047364255923)
--(axis cs:0,-2.65915644867213)
--(axis cs:1,7.51692988665886)
--(axis cs:2,2.38678973627775)
--(axis cs:3,160.713235021052)
--(axis cs:4,296.105999231114)
--(axis cs:5,412.613442177057)
--(axis cs:6,635.412151240929)
--(axis cs:7,847.031035859417)
--(axis cs:8,905.028610959436)
--(axis cs:9,1019.60461168053)
--(axis cs:10,1188.82108857787)
--(axis cs:11,1190.5085194263)
--(axis cs:12,1382.01572626336)
--(axis cs:13,1491.57408048096)
--(axis cs:14,1513.47939710068)
--(axis cs:15,1543.45539216917)
--(axis cs:16,1568.19165295542)
--(axis cs:17,1583.58613897989)
--(axis cs:18,1607.24387426497)
--(axis cs:19,1601.47233951863)
--(axis cs:20,1623.91883274357)
--(axis cs:21,1655.58702557294)
--(axis cs:22,1713.14309917408)
--(axis cs:23,1723.00301876539)
--(axis cs:24,1764.2096155033)
--(axis cs:25,1876.27438065925)
--(axis cs:26,1857.38824665802)
--(axis cs:27,1974.19610216807)
--(axis cs:28,1952.79070648111)
--(axis cs:29,1921.82042515931)
--(axis cs:30,2002.68321365198)
--(axis cs:31,2057.12251435356)
--(axis cs:32,2121.2093685317)
--(axis cs:33,2101.51759483253)
--(axis cs:34,2179.74512110872)
--(axis cs:35,2297.12600263884)
--(axis cs:36,2306.09183625888)
--(axis cs:37,2339.26064838504)
--(axis cs:38,2357.88333149311)
--(axis cs:39,2348.2997038981)
--(axis cs:40,2349.0747641075)
--(axis cs:41,2424.91556352374)
--(axis cs:42,2486.51169869601)
--(axis cs:43,2522.50526384538)
--(axis cs:44,2563.92261255278)
--(axis cs:45,2609.93007796049)
--(axis cs:46,2568.86027387872)
--(axis cs:47,2641.7959794716)
--(axis cs:48,2663.95433365989)
--(axis cs:49,2741.77496274705)
--(axis cs:50,2733.54374393341)
--(axis cs:51,2716.7273530754)
--(axis cs:52,2765.71454855578)
--(axis cs:53,2848.58810800324)
--(axis cs:54,2849.02752974287)
--(axis cs:55,2882.70700759689)
--(axis cs:56,3007.53995641982)
--(axis cs:57,2996.56017294282)
--(axis cs:58,3004.21225172137)
--(axis cs:59,3003.51733438876)
--(axis cs:60,3099.9347871723)
--(axis cs:61,3104.36958824834)
--(axis cs:62,3165.31179122242)
--(axis cs:63,3196.55342107074)
--(axis cs:64,3178.13704473715)
--(axis cs:65,3263.20271116445)
--(axis cs:66,3259.47401928986)
--(axis cs:67,3257.67719428826)
--(axis cs:68,3255.20514369804)
--(axis cs:69,3290.55974069051)
--(axis cs:70,3318.05896426068)
--(axis cs:71,3346.87064735074)
--(axis cs:72,3358.80013395085)
--(axis cs:73,3383.0300246677)
--(axis cs:74,3406.34251788852)
--(axis cs:75,3309.32513269053)
--(axis cs:76,3407.78613484326)
--(axis cs:77,3439.69492349899)
--(axis cs:78,3411.69985102143)
--(axis cs:79,3405.34183770809)
--(axis cs:80,3385.18551455515)
--(axis cs:81,3407.45635642855)
--(axis cs:82,3390.90773071852)
--(axis cs:83,3388.7050421717)
--(axis cs:84,3465.56636104986)
--(axis cs:85,3468.74785503741)
--(axis cs:86,3471.03384836968)
--(axis cs:87,3439.5383167058)
--(axis cs:88,3494.32319277098)
--(axis cs:89,3518.10636253971)
--(axis cs:90,3510.30273783052)
--(axis cs:91,3554.15917551649)
--(axis cs:92,3501.9608051066)
--(axis cs:93,3550.49597652156)
--(axis cs:94,3553.35712414308)
--(axis cs:95,3524.63508828543)
--(axis cs:96,3529.54277285338)
--(axis cs:97,3574.44508569631)
--(axis cs:98,3554.03049375633)
--(axis cs:99,3601.72846493995)
--(axis cs:99,4444.7555339556)
--(axis cs:99,4444.7555339556)
--(axis cs:98,4388.85883828941)
--(axis cs:97,4398.18153950046)
--(axis cs:96,4321.9731418338)
--(axis cs:95,4327.18930208247)
--(axis cs:94,4337.85993818148)
--(axis cs:93,4359.95787748152)
--(axis cs:92,4316.80835324122)
--(axis cs:91,4331.00902272161)
--(axis cs:90,4282.89867144423)
--(axis cs:89,4318.48839157845)
--(axis cs:88,4324.8436637386)
--(axis cs:87,4246.9359584758)
--(axis cs:86,4241.54341226975)
--(axis cs:85,4217.30402327563)
--(axis cs:84,4249.89359660185)
--(axis cs:83,4249.25248994419)
--(axis cs:82,4187.78229665748)
--(axis cs:81,4233.12465924577)
--(axis cs:80,4190.89527432862)
--(axis cs:79,4188.40795429288)
--(axis cs:78,4214.92979123969)
--(axis cs:77,4193.10842817833)
--(axis cs:76,4196.41483465942)
--(axis cs:75,4125.30822629123)
--(axis cs:74,4186.12066194708)
--(axis cs:73,4170.77776927206)
--(axis cs:72,4142.73417961138)
--(axis cs:71,4125.69964662831)
--(axis cs:70,4123.43803207798)
--(axis cs:69,4094.48675837182)
--(axis cs:68,4098.49135866485)
--(axis cs:67,4036.19174129836)
--(axis cs:66,4070.43356129305)
--(axis cs:65,4031.24329725839)
--(axis cs:64,3996.37822690603)
--(axis cs:63,3948.53368041693)
--(axis cs:62,3962.82804552951)
--(axis cs:61,3905.54735504158)
--(axis cs:60,3905.15212009017)
--(axis cs:59,3818.92804370427)
--(axis cs:58,3827.40755069082)
--(axis cs:57,3805.51291343862)
--(axis cs:56,3763.7490395991)
--(axis cs:55,3656.63062612847)
--(axis cs:54,3692.32688159955)
--(axis cs:53,3635.82299621915)
--(axis cs:52,3607.03792786311)
--(axis cs:51,3530.21755246871)
--(axis cs:50,3532.97674798691)
--(axis cs:49,3517.82473109009)
--(axis cs:48,3431.58852723932)
--(axis cs:47,3405.71650242836)
--(axis cs:46,3333.95638343952)
--(axis cs:45,3340.65732373052)
--(axis cs:44,3302.96718256399)
--(axis cs:43,3253.40102121344)
--(axis cs:42,3215.36042123354)
--(axis cs:41,3160.6520723303)
--(axis cs:40,3089.64384971076)
--(axis cs:39,3083.60112429254)
--(axis cs:38,2963.38567360397)
--(axis cs:37,2974.43495463525)
--(axis cs:36,2959.4095146885)
--(axis cs:35,2840.29437689475)
--(axis cs:34,2768.00431648625)
--(axis cs:33,2646.73601122411)
--(axis cs:32,2669.66266133294)
--(axis cs:31,2603.51594463333)
--(axis cs:30,2582.17809220897)
--(axis cs:29,2440.71533650271)
--(axis cs:28,2453.08094837111)
--(axis cs:27,2428.48771622382)
--(axis cs:26,2316.0640376844)
--(axis cs:25,2228.76974982929)
--(axis cs:24,2154.63570934645)
--(axis cs:23,2106.48822784136)
--(axis cs:22,2044.14205864596)
--(axis cs:21,1961.37307447775)
--(axis cs:20,1935.27033802111)
--(axis cs:19,1857.02174332084)
--(axis cs:18,1856.89258792916)
--(axis cs:17,1834.68195819241)
--(axis cs:16,1804.73038547795)
--(axis cs:15,1726.34256646555)
--(axis cs:14,1701.21377905242)
--(axis cs:13,1683.5305610349)
--(axis cs:12,1606.46156900964)
--(axis cs:11,1478.75889326971)
--(axis cs:10,1468.43846645296)
--(axis cs:9,1420.37085666422)
--(axis cs:8,1361.94347139281)
--(axis cs:7,1256.52586651271)
--(axis cs:6,987.467237824806)
--(axis cs:5,787.77945201487)
--(axis cs:4,660.78866232566)
--(axis cs:3,379.112584179643)
--(axis cs:2,52.3205714661793)
--(axis cs:1,89.3517280243388)
--(axis cs:0,47.2047364255923)
--cycle;

\addplot [semithick, blue]
table {%
0 -11.0178532331251
1 99.3175684184132
2 374.967228209651
3 585.090791596031
4 800.964306939033
5 934.525211183715
6 904.041870461718
7 932.526515873367
8 995.951482366304
9 1082.78017530664
10 1103.71862766219
11 1181.23448416646
12 1142.21670535143
13 1169.93760012654
14 1229.4609466636
15 1310.15105565182
16 1368.76614089292
17 1420.58888886806
18 1457.14276829857
19 1521.23007808936
20 1495.37800553284
21 1601.65954950899
22 1645.6470738063
23 1765.62094669983
24 1727.49279773991
25 1783.81909939981
26 1855.4503665983
27 1940.93592472679
28 1903.23239254481
29 1953.4588967603
30 1968.40063838392
31 2005.37694142948
32 2084.83037912967
33 2122.25438575824
34 2144.89859063938
35 2139.58945512007
36 2195.76515955755
37 2170.87472495984
38 2244.59102596719
39 2246.57750872989
40 2252.31598304335
41 2252.28724483783
42 2269.56049158407
43 2277.501825042
44 2316.17536571358
45 2228.7366525669
46 2359.13475520781
47 2342.27628201564
48 2344.22458243234
49 2362.62794434487
50 2344.08638351857
51 2391.18394357459
52 2398.56698372182
53 2480.62196549585
54 2445.04571237694
55 2461.2332691673
56 2440.47915931298
57 2502.26540589374
58 2468.53726169202
59 2516.5536106501
60 2525.73976777404
61 2515.37603606665
62 2566.9845403377
63 2551.93125426656
64 2496.82884571014
65 2597.01541495871
66 2537.97934238333
67 2515.8433879843
68 2631.51043121734
69 2627.83115340806
70 2698.50343368259
71 2660.21187632907
72 2665.62705678322
73 2684.98678718212
74 2702.12728072576
75 2695.26456800156
76 2736.27364572059
77 2806.457254686
78 2819.9594786753
79 2742.04967054093
80 2820.02374862494
81 2782.82777189531
82 2860.59167998306
83 2869.17329115044
84 2881.60968539021
85 2904.54788711714
86 2923.69018177732
87 2898.37483159722
88 3008.2075991589
89 2954.90484072822
90 2967.36182706912
91 2980.68918697353
92 2992.36963770973
93 2991.38658228289
94 3043.22934612388
95 3039.96004102946
96 3057.00328221454
97 3078.29853296243
98 3046.86848749743
99 2933.98292394914
};
\addlegendentry{target}
\addplot [semithick, green!50.1960784313725!black]
table {%
0 20.5696111612188
1 48.0113643633792
2 23.9326775645735
3 263.420325934951
4 476.027106488257
5 612.091855565621
6 820.264622963629
7 1076.88527759144
8 1143.11165119737
9 1233.0145525565
10 1338.98363757531
11 1343.54246053364
12 1496.68721226347
13 1584.69030107945
14 1609.07812145909
15 1634.42024212684
16 1688.4847478774
17 1709.53258183138
18 1731.02642002858
19 1728.04305525034
20 1780.68481271617
21 1823.87809333996
22 1881.86067223376
23 1918.84797041333
24 1963.82643941022
25 2050.48796699402
26 2070.58813965536
27 2196.55811221607
28 2211.61733189153
29 2187.3314845781
30 2286.4771330027
31 2343.25612995444
32 2390.5108346818
33 2385.74250485813
34 2461.21164987108
35 2566.39039359839
36 2644.75436882838
37 2667.56233731144
38 2684.52466292662
39 2728.53203686652
40 2723.13923526562
41 2787.45771765632
42 2847.64900083437
43 2886.26836516029
44 2957.07571877131
45 3004.70288232187
46 2951.65883856072
47 3031.24453900284
48 3076.07046593034
49 3117.23444074912
50 3152.695293649
51 3165.83898937797
52 3210.06977101411
53 3247.90044888395
54 3297.60036487645
55 3298.73714352346
56 3401.72861330504
57 3435.64557713235
58 3443.08621399967
59 3461.86352476213
60 3542.15915658113
61 3542.18600929014
62 3603.97529191755
63 3567.42897644656
64 3633.22451386287
65 3677.54323666284
66 3690.39776615333
67 3682.89594005184
68 3716.38003739321
69 3744.67692846559
70 3750.47809950442
71 3775.26637933617
72 3767.86672666008
73 3821.82163828324
74 3803.57926696622
75 3781.89095621824
76 3835.23769932098
77 3829.24022207784
78 3852.49464263772
79 3829.21268146349
80 3835.85044645023
81 3871.99406468128
82 3844.57924318378
83 3891.61620582388
84 3914.02310593033
85 3865.61338159537
86 3891.06175114807
87 3867.60495005668
88 3956.81581728201
89 3963.47438359381
90 3928.32375148463
91 3982.54623064233
92 3949.4440846463
93 4006.60381573548
94 3990.05268659494
95 3984.19223474651
96 3988.524651105
97 4037.14704255342
98 4033.24808371652
99 4074.3076922873
};
\addlegendentry{auxiliary}
\end{axis}

\end{tikzpicture}

